Pareto-Optimal Algorithms for Learning in Games

We study the problem of characterizing optimal learning algorithms for playing repeated games against an adversary with unknown payoffs. In this problem, the first player (called the learner) commits to a learning algorithm against a second player (called the optimizer), and the optimizer best-responds by choosing the optimal dynamic strategy for their (unknown but well-defined) payoff. Classic learning algorithms (such as no-regret algorithms) provide some counterfactual guarantees for the learner, but might perform much more poorly than other learning algorithms against particular optimizer payoffs. In this paper, we introduce the notion of asymptotically Pareto-optimal learning algorithms. Intuitively, if a learning algorithm is Pareto-optimal, then there is no other algorithm which performs asymptotically at least as well against all optimizers and performs strictly better (by at least $\Omega(T)$) against some optimizer. We show that well-known no-regret algorithms such as Multiplicative Weights and Follow The Regularized Leader are Pareto-dominated. However, while no-regret is not enough to ensure Pareto-optimality, we show that a strictly stronger property, no-swap-regret, is a sufficient condition for Pareto-optimality. Proving these results requires us to address various technical challenges specific to repeated play, including the fact that there is no simple characterization of how optimizers who are rational in the long-term best-respond against a learning algorithm over multiple rounds of play. To address this, we introduce the idea of the asymptotic menu of a learning algorithm: the convex closure of all correlated distributions over strategy profiles that are asymptotically implementable by an adversary. We show that all no-swap-regret algorithms share the same asymptotic menu, implying that all no-swap-regret algorithms are ``strategically equivalent''.

==> MB_equals_MW_main_old.tex <==
We would now like to show that for the games in question, the menu $\MB$ is not merely a subset of the asymptotic menu of a mean-based no-regret algorithm (as indicated by Lemma \ref{lem:sub-mean-based}), but actually an exact characterization of such menus. While we do not show this in full generality, we show this for a large class of mean-based algorithms, including classic algorithms like multiplicative weights and follow the regularized leader.

%\esh{Changed this to no-regret}
Call a no-regret learning algorithm $\cA$ \emph{strictly mean-based} if it satisfies the following assumptions for all finite time horizons $T$:

\begin{itemize}
\item $\A$ is $\gamma$-mean based with $\gamma(t) = o_T(1)$ and $\gamma(t) \cdot t$ is a weakly monotone function of $t$~\footnote{Recall that this without loss of generality for a mean-based algorithm}.
\item On every sequence of play, $\A$ has the absolute value of regret upper bounded by $R(T)$ with $R(T) = o(T)$.
%\item $\A$ has regret lower bounded by $-O(T^{\regret})$ on any prefix of play.
\item The moves played by $\A$ each round are entirely determined by the cumulative payoffs of the actions and are invariant to additively shifting the cumulative payoffs of all actions by the same quantity. 
\item For a fixed optimizer subsequence corresponding to a subsequence of play where one of the actions (call it A) is $f(T)$-far from being the leader, where $f(T) := \max\ \{ R(T), \gamma(T) \cdot T\} $, the (normalized) CSP of this optimzer subsequence induced by playing against algorithm $\A$ for three actions  is within $O(f(T))$ close in $\ell_1$ distance to the CSP induced by play against the same algorithm $\A$ but with action A excluded from consideration.~\esh{Is it clear what this means?}~\esh{One way to make this formal is through rejection sampling}
\end{itemize}

Note that multiplicative weights and follow-the-regularized-leader satisfies this set of assumptions ~\esh{Perhaps it might be worth explaining how these assumptions are true for MW, in detail, in the appendix; so that we make it clear what they mean}. The description of these algorithms can be found in Appendix~\ref{app:mwu_ftpl}. %\jon{perhaps we want to define these here?}

\esh{Verify the regret lower bound for MW, FTPL - DIY if possible}

\begin{lemma}
The multiplicative weights algorithm and follow-the-regularized-leader are strictly mean-based.
\end{lemma}
\begin{proof}
%\jon{INSERT PROOF / REFERENCE}
See Theorems~\ref{thm:mwu},~\ref{thm:ftpl} for the regret lower and upper bounds. The mean-based property of these algorithms has been observed by~\cite{braverman2018selling} and the last two properties are apparent from the latter and from the construction of the algorithms (See Algorithms~\ref{alg:mwu},~\ref{alg:ftpl}).
\end{proof}

\begin{theorem}
\label{thm:sbm=mb}
For the $u_L$ defined in \eqref{eq:game}, if $\cA$ is a strictly mean-based algorithm, then $\cM(\cA) = \MB$. 
\end{theorem}
\begin{proof}[Proof sketch]
We provide a sketch of the proof here, and defer the details to Appendix~\ref{app:sbm=mb}. The non-trivial part of the proof to show is to show that $\cM(\cA) \subseteq \MB$ since the other direction follows directly from $\cA$ being mean-based and Lemma~\ref{lem:sub-mean-based}. To this end, we focus on a finite time version of the trajectories used to build $\MB$. Intuitively, these trajectories guarantee that a unique action is significantly the best action in hindsight, or the historical leader, on all but a sublinear number of time steps. In other words, all mean-based algorithms behave identically, i.e induce identical CSPs,  upto subconstant factors against each such optimizer subsequence. The main idea in the proof is that we can transform any optimizer sequence inducing a CSP against $\cA$ into a sequence with the above properties, against which all mean-based algorithms (including $\cA$) induce almost identical CSPs. Clearly, the parts of the trajectory that lie in a region with a ``clear" historical leader are not an issue, and the challenge to this approach comes from parts of a trajectory that lie in a region where more than one action is close to being the leader. In such regions, different mean-based algorithms could potentially exhibit markedly different behavior. The key to addressing this issue is that in~\ref{eq:game}, there can be at most two actions in contention to be the leader at any point of time. Utilizing the last property of strict mean-based algorithms, it is as if $\cA$ is being played exclusively with two actions in such segments. The no-regret upper and lower bound guarantees, when suitably applied in such segments, automatically strengthen into a stronger guarantee, which we use in concert with the regret lower bounds to construct a local transformation of the trajectory in such a region (found in Lemma~\ref{lem:nc_replacement}). Each such transformation add a sublinear error to the generated CSP.  Thus, to bound the total drift from the original CSP, we show that we do not need a large number of transformations (the specific number balances with the asymptotics of the sublinear error that we make in each local transformation) using some properties of~\eqref{eq:game}.
    
\end{proof}

As a corollary, we can finally prove the main result of this section -- that there exist learner payoffs for which algorithms like multiplicative weights and follow-the-regularized-leader are Pareto dominated. This result follows directly from an application of Theorem~\ref{thm:pareto-optimal-characterization} to the menu of any strictly mean-based algorithm; since we have shown it is a polytopal no-regret menu and its minimum value points are a superset of the minimum value points of $\M_{NSR}$.  
%\esh{This is presumably where we want to invoke the polytope characterization result/ the more general one}



\begin{corollary}
\label{cor:coup_de_grace_mw}
For the $u_L$ defined in \eqref{eq:game}, all strictly mean-based algorithms are Pareto-dominated.
\end{corollary}

\begin{comment}
    

\esh{Theorem 4.1 makes this proof extraneous? }
\begin{proof}
    We construct an asymptotic menu that dominates the asymptotic menu of a given strictly mean-based algorithm $\A$. First, we observe that $\M(\A)$ is a polytope, since $\MB$ is a polytope (Theorem~\ref{thm:mb_is_a_polytope}) and $\M(\A) = \MB$ (Theorem~\ref{thm:sbm=mb}). Next, we observe that $\MB^{-} \not \subseteq \M_{NSR}^{-}$ (Theorem~\ref{thm:high-mb-swap-regret}), implying that $\M(A)^{-} \subseteq \M_{NSR}^{-}$. However, we also know that $\M_{NSR}$ is a polytope (by definition), $M_{NSR}$ is an asymptotic menu (Corollary~\ref{cor:nsr_asymptotic}) and $M_{NSR} \subset \M(\A)$ (Lemma~\ref{lem:nsr_within_all_nr}). Thus, let $E(\A)$ and $E_{NSR}$ be the vertices of the polytopes $\M(\A)$ and $\M_{NSR}$ respectively. These are both finite sets and we know there is a point $T \in E(\A) \setminus E_{NSR}$  with $\mu_L(T) = U^-(\M) = U_{ZS}$, i.e the extreme point $T$ has learner utility equal to the minimax value, which is the minimum learner value in any no-regret menu. We now construct a new asymptotic menu $\M$ by expanding $\M_{NSR}$ through the addition of all points in $(E(A) \setminus \{T\}) \setminus E_{NSR}$, combined with taking their convex hull (Lemma~\ref{lem:char_upwards_closed}). Since polytopes have a finite number of vertices, we can safely concluded that the new menu $\M$ is also a polytope and its set of extreme points is the set $(E(A) \setminus \{T\})$. This means that $\M^- \subseteq \M^-(\A)$ and $\M_1$ and $\M_2$ are distinct menus. Thus, Lemma~\ref{lem:non-dominance} tells us that there exists an optimizer payoff $u_O$ for which the learner does strictly better in $\M$ as compared to $\M(\A)$ (\esh{Come back and edit this once we have a stable generalization to a positive measure set of optimizer payoffs}). The lasts part of this proof is to show that the learner does at least as well in $\M$ than in $\M(\A)$ against any optimizer. Lemma~\ref{lem:menu_alg_equiv} interprets the learner's value against an optimizer as coming from the optimizer selecting a CSP from the menu with largest (optimizer) payoff value (and evaluating the learner value at this CSP). Since the optimizer tie breaks in favor of the learner, we can assume the optimizer selects an extreme point of the menu (i.e. a vertex in a polytope). Thus, the only way in which an optimizer can behave differently on the menus $\M$ and $\M(\A)$ is if it picks the point $T$ in $\M(\A)$; however, in such a scenario the learner cannot do strictly better in $\M(\A)$ since $\mu_L(T) =  U^-(\M) $.
\end{proof}
\end{comment}

We have proved a sequence of results about strictly mean-based algorithms for a single learner payoff, i.e.~\ref{eq:game}, but our results in fact hold for a positive measure set of learner payoffs in $2 \times 3$%~\footnote{We think that it should be possible to extend this result to general $m \times n$ games, and leave it, along with best-responding to FTRL like algorithm in general games, as an open problem~\esh{Should we say this? Come back to this.}}
. All the results in this section can be generalized to perturbed versions of this learner payoff (~\ref{eq:perturbed_game}), and we show how to do so in Appendix~\ref{app:mean_based_pareto_dominated}. 





%\esh{Add a proof of this}
%\esh{Change the statement for the perturbed game, explain that we have the same characterization in the appendix, and invoke those to complete the proof of Pareto Domination   }


%\esh{Leaving a note here for a couple of auxilary results}

%~\esh{Should we write more about $\M_{NR}$ not being equal to the menu of every MBNR algo? It is not on any critical path, but it's a conceptually interesting contribution}. \nat{Certainly worth putting the example in a footnote at least, and I wouldn't be opposed to adding a pointer to a lemma in the appendix.} 
  

%\nat{Note that we have a disproof that all MBNR algos have the same menu as MB. Use the guess the sequence thing, you get a point with negative regret, this isn't in MW. But MB = MW, done.}

%\esh{We're claiming this result elsewhere - Lemma~\ref{lem:nr_ne_mw}, so we can add a pointer to it, but I'm yet to write the proof, so this is one approach we could take}
%\subsection{Mean Based Algorithms and Online Environments}


%\label{sec:ftl_meanbased}
%\input{ftl_meanbased}

%\subsection{Many Mean-based Algorithms are Pareto Dominated}


%\input{mw_a_polytope}


\begin{comment}
    
\subsection{Results about Mean Based No-Regret Algorithms - Proof of Theorem~\ref{thm:mbnr_pd}}
\nat{This entire section is redundant, keeping around for reference for now while writing some conceptually related results above.}
\input{no_regret_domination}

\end{comment}


==> NSR_NR.tex <==
%{\bf Observation :} If we can identify a game where two different learner algorithms 
%induce different payoffs for a best responding learner, then we have identified a difference in the menus induced for that game's learner payoff. Specifically, the menu with the larger optimizer payoff has a point that is not in the other algorithm's menu - allowing us to translate back to the tools developed in the previous subsection



\esh{ ATTENTION : This section is mostly irrelevant now, but we should note the pareto optimality of NSR somewhere}




\esh{Results about polytopes are good enough for this entire subsection}


First, we introduce some useful notation and mathematical objects. These definitions are assuming a fixed learner payoff function.


    \begin{itemize}
        \item Let $P_{NR}$ denote the set of all points satisfying the no-regret condition.
        \item Let $P_{NSR}$ denote the set of all points satisfying the no-swap regret condition.
    \end{itemize}

Both $P_{NR}$ and $P_{NSR}$ are polytopes since the respective conditions can be written down as linear conditions (that they are polytopes rather than just polyhedrons is a result of their containment in the $m \times n$-dimensional simplex).

\esh{There is a small issue with tie-breaking here - @Jon suggested we take the closure of the menu to avoid this problem. Alternatively, the set of problem points is measure zero, so perhaps we can set up the definitions to ignore these while comparing menus?}

\begin{comment}
    

\begin{theorem}
    \label{theorem:nsr_minimal}
    All NSR algorithms (asymptotically) induce the same menu for any fixed learner payoff. Additionally, this menu is minimal (no algorithm induces a menu that is a strict subset).
\end{theorem}
\end{comment}


%\esh{Note to self: bad notation here - $T$ is usually used to denote the time horizon, replace by the macro $\brmix$}
    Fix the learner payoff to be $\mu_L$.  $P_{NSR}(\mu_L) \subseteq \mathbb{R}^{m \times n}$ is the set of all points that satisfy the no-swap regret condition under this learner payoff. Define $\brmix: = \{ \mathbbm{1}_a \times \beta \in \mathbb{R}^{m \times n} : \beta \in \Delta^{[n]} \text{ and } a \in \argmax_a \mu_L(a,\beta)\}$ and let $S = Conv(\brmix)$. In other words, $\brmix$ is the set of all empirical distributions over action pairs that are the product of a mixed strategy of the learner and a pure strategy best response of the optimizer and $S$ is the convex hull of $\brmix$. We demonstrate in our proof that $P_{NSR} = S$. %As a corollary, consider the menu $\A$ of any no-swap regret algorithm - $S \subseteq \A$ and $\A \subseteq P_{NSR}$ implying that $\A = P_{NSR}$.

    \begin{claim}
        $P_{NSR} = S$.
    \end{claim}

    \begin{proof}
        
     First, we show that $S \subseteq P_{NSR}$. It suffices to show that $\brmix \subseteq P_{NSR}$ since $P_{NSR}$ is a polytope. Consider any point of the form $\mathbbm{1}_a \times \beta  \in \brmix$. This point directly satisfies the no-swap regret condition since $a$ is by definition a best response to $\beta$ and the only operation any swap function can do in this case is to replace all appearances of $a$ with something else, implying $\brmix \subseteq P_{NSR}$ and consequently $S \subseteq P_{NSR}$. 

    To show that $P_{NSR} \subseteq S$, consider a point $X \in P_{NSR}$ - let $x_{ij}$ denote the $i,j$-th coordinate of $X$. We rewrite $X$ as a sum of product measures over action pairs. For each action $a$, let $\mathbbm{1}_a \in \delta^{[m]}$ represent the learner strategy that puts all the mass on action $a \in [m]$. Let $\beta(a)$ represent the conditional marginal strategy of the optimizer corresponding to $X$ given that the learner plays action $a$, i.e. $\beta_j(a) =\frac{X_{aj}}{\sum_{k \in [n]} X_{ak}}$ for all $j \in [n]$ (for the egde case, where all the quantities $\{X_{ak}\}_k$ are $0$, we set  $\beta_k(a) = 0$ for all $k \in [n]$). For each action $a$ of the learner, the $\beta_j(a)$s aggregate to form a probability vector $\beta \in \delta^{[n]}$. Completing the rewrite $X = \sum_{a \in [m]} (\sum_{k \in [n]} X_{ak}) \mathbbm{1}_a \times \beta(a)$. For any action $a$ of the learner, if $a \notin \argmax_b u_L(b,\beta(a))$, this would imply the existence of swap regret associated with $X$. Since $X \in P_{NSR} $, this implies that for all actions $a$, $a \in \argmax_b u_L(b,\beta(a))$. Thus, we have rewritten $X$ as a convex combination of points in $T$, implying $X \in \brmix$ and thus $P_{NSR} \subseteq S$.
    \end{proof}



Having established that $S = P_{NSR}$, we show that no asymptotic menu can be weakly contained in $P_{NSR}$.

\begin{claim}
\label{claim:nsr_polytope_is_minimal}
    There is no algorithm $\B$ with asymptotic menu $\M(\B)$ such that $\M(\B) \subseteq P_{NSR}$.
\end{claim} 

   \begin{proof}
       
Assume otherwise, for sake of contradiction. This implies the existence of a point $X = \mathbbm{1}_a \times \beta \in \brmix$ that is not present in $\M(\B)$ (since $P_{NSR}$ is the convex hull of $\brmix$). First, we deal with the case where $a$ is a unique learner best response to the optimizer distribution $\beta$. There must be at at least one point $P$ in the menu $\M(\B)$ corresponding to the optimizer playing the distribution $\beta$ in every round (the reasoning can be extended by starting at finite time menus)~\esh{Note to self: find/ write a lemma that shows menus have points corresponding to every optimizer marginal distribution}. Since $P$ is not equal to $X$ (and therefore the marginal distribution of the learner is different from $\mathbbm{1}_a$), and $a$ is a unique best response to $\beta$, $P$ must have regret associated with it, implying $P \notin P_{NSR}$, however this results in a contradiction with $\M(\B) \subseteq P_{NSR}$, invalidating our assumption. 
    
If $a$ is not a unique best-response to $\beta$, then we find a nearby point $\beta'$ such that $a$ is a unique best response to $\beta'$. To this end, we use the Farkas Lemma, from which we get that there exists a distribution $\gamma \in \Delta^n$ such that $\mu_L(a,\gamma) \ge \mu_L(a',\gamma) + \kappa$ for all actions $a' \in [m] \setminus \{a\}$ and some $\kappa > 0$. Thus, for small enough $\delta > 0$, the optimizer distribution $\beta(\delta) = (1-\delta) \beta  + \delta. \beta$ has learner action $a$ as a unique best response. If all corresponding points $\mathbbm{1}_a \times \beta(\delta) $ are in $\M(\beta)$, by closure, $X$ would also be in $\M(\beta)$, resulting in a contradiction. Thus, at least one such point is not in $\M(\beta)$, in which case we can use the prevoius case's argument to derive a contradiction, completing the proof.

    
 %If $a$ is not a unique best-response to $\beta$, then we perturb the point to find a $(a,\beta)$ pair such that $a$ is a unique best response to $\beta$ that is not in $\M(\B)$ (if all such points are in $\M(\B)$, then by closure the original point is also in $\M(\B)$ leading to a contradiction) ~\esh{Insert the Farkas Lemma argument here and use closure}. Consider an optimizer that repeatedly plays the distribution $\beta$ against a learner playing algorithm $\B$. Let $\alpha$ be the historical marginal distribution of the learner. If $\alpha \neq \mathbbm{1}_a$, then there is a point in $\M(\B)$ with non-zero swap regret, implying $\M(\B) \not\subset P_{NSR}$, leading to a contradiction. However, if $\alpha = \mathbbm{1}_a$, then $ \mathbbm{1}_a \times \beta 
% \in \M(\B)$, which is again a contradiction. Thus, $P_{NSR}$ is a minimal menu.

 
 \end{proof}





\begin{comment}
    

\esh{This claim has to be written in a finer grained form that also proves consistency}

    \begin{claim}
        For any no-swap regret algorithm $\A$, the asymptotic menu $\M(\A)$ is exactly the polytope $P_{NSR}$. Implicitly, every no-swap regret algorithm is consistent.
    \end{claim}

    \begin{proof}
        
   
    First, we observe that every point in $T$ is also in the asymptotic menu of the algorithm since if the optimizer plays some distribution $\beta$ in every round, then the learner must necessarily best respond to it all the time to obtain vanishing regret. The only problem lies in tie-breaking - i.e. there might be points $(a,\beta)$ such that $a,b$ are both best responses to $\beta$ and the algorithm never plays $a$. However we appeal to the fact that the asymptotic menus are closed sets. We use the linear nature of the utilities to observe that there is a sequence of points $(a,\beta_1), (a,\beta_2), \cdots$ such that $a$ is a unique best response to $\beta_i$ and $\{\beta_i\}_i$ converges to $\beta$. Since each point in this sequence must be part of the menu, taking the closure ensures that $(a,\beta)$ is part of the menu. Thus, $S \subset \M(\A)$ implying that $P_{NSR} \subset \M(\A)$. However, we know that $\M(\A) \subseteq P_{NSR}$ since $\A$ is a no swap-regret algorithm. This implies that $\M(\A) = P_{NSR}$. Since this analysis works for any no swap-regret algorithm, all no swap-regret algorithms must have the same menu $P_{NSR}$.
     \end{proof}

     \esh{Rewriting the above}

\end{comment}

Armed with the above results, we can now show that all no-swap regret algorithms are consistent and in fact all have the same asymptotic menu, viz. $P_{NSR}$.

\begin{lemma}
Every no-swap regret algorithm is consistent and has the polytope $P_{NSR}$ as its asymptotic menu.
        %For any no-swap regret algorithm $\A$, the asymptotic menu $\M(\A)$ is exactly the polytope $P_{NSR}$. Implicitly, every no-swap regret algorithm is consistent.
    \end{lemma}


     \begin{proof}


        
         Consider any no-swap regret learning algorithm family $\A$ where the algorithm for the time horizon $T$ is $\A_T$. Let $f(m,T)$ represent its associated swap regret upper bound. By definition, $\lim_{T \rightarrow \infty} \frac{f(m,T)}{T} \rightarrow 0$. Let $\M_T = \M(\A_T)$ represent the menu of the $T$-th algorithm in the family. %Fix any $\varepsilon < 0$, we show that there is a sufficiently large time horizon $T^*$ such that for all $T > T^*$, the Hausdorff distance $h(\M_T, P_{NSR})$ is at most $\varepsilon$. 

         We introduce another sequence of sets to aid with this proof. Let $S_T$ denote the polytope defined by the no-swap regret constraints, but where we upper bound the swap regret by $\frac{f(m,T)}{T}$ rather than 0.  $M_T \subseteq S_T$ is implied by the properties of algorithm $\A$. Further, it is not hard to see that $\lim_{T \rightarrow \infty} S_T = P_{NSR}$ (follows from $S_1 \supseteq S_2 \supseteq S_3  \cdots S_T \cdots $ and $P_{NSR}$ is the maximal set contained in $S_T$ for all $T$).
         

         Consider any convergent subsequence of the sequence $\{\M_T\}_{T=1}^\infty$, let it have limit set $\M$. Since $\M_T \subseteq S_T$ for all $T$, the property of Hausdorff spaces~\esh{insert ref} allows us to conclude that $\M \subseteq P_{NSR}$. However, since $\M$ is an asymptotic menu, Claim~\ref{claim:nsr_polytope_is_minimal} implies that $\M = P_{NSR}$. Since every convergent subsequence of the sequence $\{\M_T\}_{T=1}^\infty$ converges to the same set $P_{NSR}$, the sequence is in fact convergent and converges to $P_{NSR}$ (invoking a property of Hausdorff spaces~\esh{add ref}).
         
         %Thus, for any given $\varepsilon > 0$, there is a time horizon $T^*_1$ such that for all $T> T^*_1$, $h(S_T, P_{NSR}) < \varepsilon$.

    
         %First, we consider any point $P \in \M_T$ and show that the $\ell_2$-metric distance $d(P_{NSR},P) < \varepsilon$. Since $P$ is in $\M_T$, $P$ is also contained in $S_T$. This implies existence of a point $P' \in P_{NSR}$ such that $d(P,P') < \varepsilon$.

         %First, we consider any point $P \in \M(\A_T)$ and show that the $\ell_2$-metric distance $d(P_{NSR},P) < \varepsilon$. Let $P_{a,b}$ denote the probability weight of any action pair $a,b$ with $a \in [m]$ and $b \in [n]$. Extracting  the conditional distribution of the optimizer given that the learner played action $a$, let $\alpha_a (b') = \frac{P_{a,b'}}{\sum_{b \in [n]} P_{a,b}}$ for all $b' \in [m]$ . Introducing notation for the total probability associated with a learner action , let $w_a := \sum_{b \in [n]} P_{a,b}$. Thus, we rewrite the point $P$ as $P = \sum_{a \in [n]} w_a (\mathbbm{1}_a \times \alpha_a)$, which is a convex combination of product distributions. Using the no-swap regret property, for each learner action $a$, $a$ is a $\frac{f(m,T)}{T}$-best response to $\alpha_a$. Thus, we can always find a distribution $\alpha'_a$ over optimizer actions such that $a$ is a best-response to $\alpha'_a$ and $d(\alpha_a, \alpha'_a) \le O \left (\frac{f(m,T)}{T} \right)$~\footnote{The constant factors here are only dependent on the smallest difference between any two terms in the payoff matrix $u_L$}. Based off these observations, we consider the point $P' = \sum_{a \in [n]} w_a (\mathbbm{1}_a \times \alpha'_a)$, which by construction is a point that is present in the set $S = P_{NSR}$. Additionally, we also infer from the properties of the $\alpha'_a$s that the distance between $P$ and $P'$ is bounded, i.e., $d(P,P') \le O \left (\frac{m f(m,T)}{T} \right)$. Since $\lim_{T \rightarrow \infty} \frac{f(m,T)}{T} \rightarrow 0$, we could have always set $T^*$ such that $O \left(\frac{f(m,T)}{T} \right) \le \frac{\varepsilon}{m}$, completing this part of the proof. 

        %Next, we consider any point $Q \in P_{NSR}$ and show that there exists a point $Q' \in \M_T$ such that $d(Q,Q') < \varepsilon$. To this end, we utilize the fact that $P_{NSR} = S$.
        %Since $S $ is the convex hull of $\brmix$, the vertices of $P_{NSR}$ form a subset of $\brmix$. Thus, any point $Q \in P_{NSR}$ can be written as a convex combination of a finite number of points in $\brmix$, in fact we can rewrite it as a convex combination of at most $m$ points in $\brmix$ by combining the points based upon the learner's action. For each such point $Y_a = \mathbbm{1}_a \times \alpha_a$, we perturb $\alpha_a$ by an infinitesimal amount to ensure that $a$ is a unique best response to $\alpha_a$. We then use the no-swap regret property of $\A$ to argue that for each $Y_a$, there is corresponding point $X_a \in \M_T$ such that $d(X_a,Y_a) \le O \left(\frac{f(m,T)}{T}\right)$~\esh{Still a hiccup here - what if there are other actions that re infinitesimally close to a BR?}%~\footnote{The constants here only depend on the learner's payoff matrix and are agnostic to the specific points $X_a$ and $Y_a$}. 
        %This point $X_a$ is realized in the algorithm's menu by having the optimizer play the distribution $\alpha_a$ in every round and observing that the algorithm must best-respond most of the time. $Q$ can be written as a convex combination $\sum_{a \in [m]} w_a Y_a$, we use the same weights to write down $Q' = \sum_{a \in [m]} w_a Y_a$ %\esh{Running into a hiccup here, but will cycle back to this soon}
     \end{proof}

    

\begin{observation}
    $P_{NSR}$ contains $L_+$, the maximum value point.
\end{observation}

Putting together the above two results (minimality and containing $L_+$), we invoke Theorem~\ref{thm:L+_minimal_po} to finish the proof of pareto optimality of every no-swap regret algorithm. We critically use the fact that the menu of every no-swap regret algorithm is a polytope (i.e. $P_{NSR}$).

%\esh{To be added : Proof of consistency of every NSR algorithm }
    %\esh{Incomplete, will soon be finished and moved up}


==> ec_submission/ec_mean_based.tex <==
\section{Mean-based algorithms and menus}
\label{sec:mb_algos_and_menus}

In this section, we return to one of the main motivating questions of this work: are standard online learning algorithms (like multiplicative weights or follow-the-regularized-leader) Pareto-optimal? Specifically, are \emph{mean-based} no-regret learning algorithms, which always approximately best-respond to the historical sequence of observed losses, Pareto-optimal?

We will show that the answer to this question is \emph{no}: in particular, there exist payoffs $u_L$ where the menus of some mean-based algorithms (specifically, menus for multiplicative weights and FTRL) are not Pareto-optimal. Our characterization of Pareto-optimal no-regret menus in the previous section (Theorem \ref{thm:pareto-optimal-characterization}) does most of the heavy lifting here: it means that in order to show that a specific algorithm is not Pareto-optimal, we need only find a sequence of actions by the optimizer that both causes the learner to end up with the zero-sum utility $u_{ZS}$ and high swap-regret (i.e., at a point not belonging to $\M^{-}$). Such games (and corresponding trajectories of play by the optimizer) are relatively easy to find -- we will give one explicit example shortly that works for any mean-based algorithm.

However, there is a catch -- our characterization in Theorem \ref{thm:pareto-optimal-characterization} only applies to \emph{polytopal} menus (although we conjecture that it also applies to non-polytopal menus). So, in order to formally prove that a mean-based algorithm is not Pareto-optimal, we must additionally show that its corresponding menu is a polytope. %The majority of this section is dedicated to accomplishing this. 
Specifically, we give an example of a family of games where the asymptotic menus of all $\ftrl$ algorithms have a simple description as an explicit polytope which we can show is not Pareto-optimal. 



%\esh{If we are only going to summarize this section and move the rest to the appendix, is this a good point to stop? If so, we should define (or point to a definition of ) strictly mean-based/ FTRL-like algorithms here and write out a theorem statement }


\begin{theorem}
    \label{thm:ftrl_main}
    There exists a family of learner payoffs $u_L$ with $m=3$ actions for the learner and $n=2$ actions for the optimizer where all $\ftrl$ algorithms are Pareto-dominated. %~\footnote{We show the result for a positive measure set of $3 \times 2$ learner payoffs}
\end{theorem}

In in the interest of space, the proof of this result has been moved to Appendix~\ref{app:ftrl_main}.  In Section~\ref{sec:mean-based-menu} we introduce the concept of the ``mean-based menu'', a menu of CSPs that is achievable against any mean-based algorithm, and introduce the family of games we study. We then (in Section \ref{sec:mb-is-polytope}) show that for these games, the mean-based menu can be explicitly characterized as a polytope. Finally, in Section \ref{sec:mb-equals-mwu}, we prove that the asymptotic menu of any instantiation of FTRL must actually equal this mean-based menu (instead of merely containing it).



==> ec_submission/inlcudes_ec.tex <==
\usepackage[utf8]{inputenc}
%\usepackage[numbers]{natbib}
%\usepackage{amsmath,amssymb}
%\usepackage{bbm}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
%\usepackage{algpseudocode}
%\usepackage{algorithm}
%\usepackage[]{algorithm2e}
%\RestyleAlgo{boxruled}
 
%\usepackage[usenames,dvipsnames]{xcolor}

%\usepackage{tcolorbox}
%\tcbuselibrary{skins,breakable}
%\tcbset{enhanced jigsaw}


%\colorlet{YellowOrange}{RawSienna}


\newenvironment{proofof}[1]{\par{\noindent \bf Proof of #1:}}{$\blacksquare$ \par}
\newenvironment{oneshot}[1]{\@begintheorem{#1}{\unskip}}{\@endtheorem}
\usepackage{hyperref}
%\hypersetup{
%colorlinks=true,
%pdfnewwindow=true,
%citecolor=ForestGreen,
%linkcolor=DarkRed,
%filecolor=DarkRed,
%urlcolor=DarkBlue
%}
\usepackage{cleveref}

\newcommand{\tempcol}[1]{{\color{red}#1}}

\usepackage{amsthm}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem*{note}{Note}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}

\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{assumption}{Assumption}
%\usepackage{fullpage}

\usepackage{graphicx}

%\usepackage{xcolor}

\newcommand{\sk}[1]{\textcolor{blue}{[Sampath: #1]}}
\newcommand{\ad}[1]{\textcolor{green}{[Anindya: #1]}}


\newcommand{\ade}[1]{\textcolor{red}{#1}}
\newcommand{\hdn}{homogeneous noise model}



\newcommand{\expect}[1]{\mathbb{E}\left[#1\right]}

\usepackage{comment}
\usepackage{mathtools}

\usepackage[shortlabels]{enumitem}


\newcommand{\X}{\mathcal{X}}
\newcommand{\sst}{\text{special subtree}}
\newcommand{\fs}{\sqrt{\frac{\log n}{n}}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Mh}{\mathbf{Q}_h}

\usepackage[shortlabels]{enumitem}

\newcommand{\ignore}[1]{}
\newcommand{\fsi}{\sqrt{\frac{n}{\log n}}}
\newcommand{\ohp}{overwhelmingly high probability}
\newcommand{\hide}[1]{}


%New Commands from Edited Weights

\usepackage[shortlabels]{enumitem}
\newcommand{\NL}{\mathsf{NL}}
\newcommand{\lc}{\mathsf{lc}}
\newcommand{\rc}{\mathsf{rc}}
\newcommand{\bebetter}{b_{\text{better}}}
%\newcommand{\coloneqq}{:=}



\usepackage[shortlabels]{enumitem}

\newcommand{\p}{\widetilde{p}}
\newcommand{\h}{\widehat{h}}


\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}

\newcommand{\M}{\mathcal{M}}

\usepackage{caption}
\usepackage{xcolor}

\newcommand{\brmix}{S'}

% jon commands


\def\Rset{\mathbb{R}}
\def\Sset{\mathbb{S}}

\let\Pr\undefined
\let\P\undefined
\DeclareMathOperator*{\Pr}{\mathbb{P}}
\DeclareMathOperator*{\P}{\mathbb{P}}
% \DeclareMathOperator*{\E}{\mathbb E}
% \DeclareMathOperator*{\argmax}{argmax}
% \DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\esssup}{esssup}
\DeclareMathOperator*{\dom}{dom}
\DeclareMathOperator*{\cont}{cont}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\core}{core}
\DeclareMathOperator*{\pen}{pen}
\DeclareMathOperator{\VCdim}{VCdim}
\DeclareMathOperator{\Pdim}{Pdim}
\DeclareMathOperator{\Reg}{\mathsf{Reg}}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\diag}{diag}


\DeclareMathOperator{\Ind}{\mathbb{I}} 

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert} 
\DeclarePairedDelimiter{\bracket}{[}{]}
\DeclarePairedDelimiter{\curl}{\{}{\}}
\DeclarePairedDelimiter{\norm}{\|}{\|}
\DeclarePairedDelimiter{\paren}{(}{)}
\DeclarePairedDelimiter{\tri}{\langle}{\rangle}
\DeclarePairedDelimiter{\dtri}{\llangle}{\rrangle}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\sA}{{\mathscr A}}
\newcommand{\sB}{{\mathscr B}}
\newcommand{\sC}{{\mathscr C}}
\newcommand{\sD}{{\mathscr D}}
\newcommand{\sF}{{\mathscr F}}
\newcommand{\sG}{{\mathscr G}}
\newcommand{\sH}{{\mathscr H}}
\newcommand{\sI}{{\mathscr I}}
\newcommand{\sJ}{{\mathscr J}}
\newcommand{\sK}{{\mathscr K}}
\newcommand{\sL}{{\mathscr L}}
\newcommand{\sM}{{\mathscr M}}
\newcommand{\sP}{{\mathscr P}}
\newcommand{\sS}{{\mathscr S}}
\newcommand{\sT}{{\mathscr T}}
\newcommand{\sU}{{\mathscr U}}
\newcommand{\sX}{{\mathscr X}}
\newcommand{\sY}{{\mathscr Y}}
\newcommand{\sZ}{{\mathscr Z}}

\newcommand{\bA}{{\mathbf A}}
\newcommand{\bB}{{\mathbf B}}
\newcommand{\bD}{{\mathbf D}}
\newcommand{\bH}{{\mathbf H}}
\newcommand{\bK}{{\mathbf K}}
\newcommand{\bL}{{\mathbf L}}
\newcommand{\bM}{{\mathbf M}}
\newcommand{\bN}{{\mathbf N}}
\newcommand{\bP}{{\mathbf P}}
\newcommand{\bQ}{{\mathbf Q}}
\newcommand{\bR}{{\mathbf R}}
\newcommand{\bV}{{\mathbf V}}
\newcommand{\bW}{{\mathbf W}}
\newcommand{\bX}{{\mathbf X}}
\newcommand{\bY}{{\mathbf Y}}
\newcommand{\bZ}{{\mathbf Z}}
\newcommand{\bb}{{\mathbf b}}
\newcommand{\bl}{{\mathbf l}}
\newcommand{\bx}{{\mathbf x}}
\newcommand{\by}{{\mathbf y}}
\newcommand{\bu}{{\mathbf u}}
\newcommand{\bv}{{\mathbf v}}
\newcommand{\bw}{{\mathbf w}}
\newcommand{\bp}{{\mathbf p}}
\newcommand{\bell}{{\bm \ell}}

\newcommand{\sfp}{{\mathsf p}}
\newcommand{\sfq}{{\mathsf q}}
\newcommand{\sfr}{{\mathsf r}}
\newcommand{\sfE}{{\mathsf E}}
\newcommand{\sfB}{{\mathsf B}}
\newcommand{\sfD}{{\mathsf D}}
\newcommand{\sfS}{{\mathsf S}}
\newcommand{\sfT}{{\mathsf T}}

\newcommand{\eps}{{\varepsilon}}


\DeclareMathOperator{\Prof}{\mathsf{Prof}}
\newcommand{\MB}{\M_{\mathrm{MB}}}
\DeclareMathOperator{\BR}{\mathsf{BR}}


%Macros

\newcommand{\csp}{\varphi}
\newcommand{\gameset}{\mathcal{G}}
\newcommand{\Up}{U^{+}}
\newcommand{\Um}{U^{-}}
\newcommand{\Mp}{\M^{+}}
\newcommand{\Mm}{\M^{-}}
\newcommand{\Uzs}{U_{ZS}}
\newcommand{\ox}{\overline{x}}


\newcommand{\boundary}{T^{1-\tau}}
\newcommand{\regret}{\alpha}


\newcommand{\intersectionmb}{\mathcal{M}_{MI}}


\newcommand{\ftraj}{finite trajectory}

\newcommand{\ftrajs}{finite trajectories}



%The comment commands and their alternate forms
%\newcommand{\esh}[1]{\textcolor{red}{[Eshwar: #1]}}
\newcommand{\esh}[1]{}

%\newcommand{\nat}[1]{\textcolor{blue}{[Natalie: #1]}}
\newcommand{\nat}[1]{}
%\newcommand\jon[1]{{[\color{magenta}{\textbf{Jon:}~#1}]}}
\newcommand\jon[1]{}





%New macros for EC submission, copy into the other includes fule
% \newcommand{\ftrl}{\textsf{FTRL-fixed-convex}}
\newcommand{\ftrl}{\textsf{FTRL}}
\DeclareMathOperator{\regbound}{\rho}
\newcommand{\wtA}{\widetilde{A}}
\newcommand{\opt}{\text{opt}}
\DeclareMathOperator{\sshift}{\zeta}
\usepackage{nicematrix}





==> log.tex <==
Dec 19

Edited the boundary definitions; to be sanity checked



==> mean_based_arxiv.tex <==
\section{Mean-based algorithms and menus}
\label{sec:mb_algos_and_menus}

In this section, we return to one of the main motivating questions of this work: are standard online learning algorithms (like multiplicative weights or follow-the-regularized-leader) Pareto-optimal? Specifically, are \emph{mean-based} no-regret learning algorithms, which always approximately best-respond to the historical sequence of observed losses, Pareto-optimal?

We will show that the answer to this question is \emph{no}: in particular, there exist payoffs $u_L$ where the menus of some mean-based algorithms (specifically, menus for multiplicative weights and FTRL) are not Pareto-optimal. Our characterization of Pareto-optimal no-regret menus in the previous section (Theorem \ref{thm:pareto-optimal-characterization}) does most of the heavy lifting here: it means that in order to show that a specific algorithm is not Pareto-optimal, we need only find a sequence of actions by the optimizer that both causes the learner to end up with the zero-sum utility $u_{ZS}$ and high swap-regret (i.e., at a point not belonging to $\M^{-}$). Such games (and corresponding trajectories of play by the optimizer) are relatively easy to find -- we will give one explicit example shortly that works for any mean-based algorithm.

However, there is a catch -- our characterization in Theorem \ref{thm:pareto-optimal-characterization} only applies to \emph{polytopal} menus (although we conjecture that it also applies to non-polytopal menus). So, in order to formally prove that a mean-based algorithm is not Pareto-optimal, we must additionally show that its corresponding menu is a polytope. %The majority of this section is dedicated to accomplishing this. 
Specifically, we give an example of a family of games where the asymptotic menus of all $\ftrl$ algorithms have a simple description as an explicit polytope which we can show is not Pareto-optimal. 



%\esh{If we are only going to summarize this section and move the rest to the appendix, is this a good point to stop? If so, we should define (or point to a definition of ) strictly mean-based/ FTRL-like algorithms here and write out a theorem statement }


\begin{theorem}
    \label{thm:ftrl_main}
    There exists a $3 \times 2$ learner payoff for which all $\ftrl$ algorithms are Pareto-dominated~\footnote{We show the result for a positive measure set of $3 \times 2$ learner payoffs}.
\end{theorem}

In in the interest of space, the proof of this result has been moved to appendix~\ref{}. We outline the sequence of ideas below.

In Section~\ref{sec:mean-based-menu} we introduce the concept of the ``mean-based menu'', a menu of CSPs that is achievable against any mean-based algorithm, and introduce the family of games we study. We then (in Section \ref{sec:mb-is-polytope}) show that for this game, the mean-based menu is a polytope. Finally, in Section \ref{sec:mb-equals-mwu}, we prove that for sufficiently structured mean-based algorithms (including multiplicative weights update and FTRL) their asymptotic menu must equal this mean-based menu.

\subsection{The mean-based menu}
\label{sec:mean-based-menu}

To understand the behavior of mean-based algorithms, we will introduce an convex set that we call the \emph{mean-based menu}, consisting of exactly the correlated strategy profiles that are attainable against any mean-based learning algorithm. 

\sloppy{To define the mean-based menu, we will make use of a continuous-time reformulation of strategizing against mean-based learners presented in Section 7 of \cite{deng2019strategizing}. In this reformulation, we represent a trajectory of play by a finite non-empty list of triples $\tau = \{(x_1, t_1, b_1), (x_2, t_2, b_2), \dots, (x_k, t_k, b_k)\}$ where $x_{i} \in \Delta^m$, $t_i \in \mathbb{R}_{+}$, and $b_{i} \in [n]$. Each segment of this strategy intuitively represents a segment of time of length $t_i$ where the optimizer plays a mixed strategy $x_i$ and the learner responds with the pure strategy $b_i$.}


Let $\overline{x}_{i} = \sum_{j=1}^{i} (x_jt_j) / \sum_{j=1}^{i} t_j$ (with $\overline{x}_0 = 0$) be the time-weighted average strategy of the optimizer over the first $i$ triples. In order for this to be a valid trajectory of play for an optimizer playing against a mean-based learner, a trajectory must satisfy $b_{i} \in \BR_{L}(\overline{x}_{i-1})$ and $b_{i} \in \BR_{L}(\overline{x}_{i})$. That is, the pure strategy played by the learner during the $i$th segment must be a best-response to the the average strategy of the optimizer at the beginning and ends of this segment. We let $\cT$ represent the set of all valid trajectories (with an arbitrary finite number of segments). 

Given a trajectory $\tau$, we define $\Prof(\tau) \in \Delta_{mn}$ to equal the correlated strategy profile represented by this trajectory, namely:

$$\Prof(\tau) = \frac{\sum_{i=1}^{k} \tau_{i}(x_{i} \otimes b_{i})}{\sum_{i=1}^{k} \tau_{i}}.$$

Finally, we define the \textit{mean-based menu} $\MB$ to equal the convex closure of $\Prof(\tau)$ over all valid trajectories $\tau \in \cT$. Although $\MB$ is defined solely in terms of the continuous formulation above, it has the operational significance of being a subset of the asymptotic menu of any mean-based algorithm (the proof of Lemma \ref{lem:sub-mean-based} is similar to that of Theorem 9 in \cite{deng2019strategizing}, and is deferred to the appendix).

\begin{lemma}\label{lem:sub-mean-based}
    If $\cA$ is a mean-based learning algorithm with asymptotic menu $\M$, then $\MB \subseteq \M$. 
\end{lemma}

% \nat{Remark that the semantic meaning of $M_MB$ is different than $M_{NR}$ and $M_{NSR}$} 



Note that unlike $\M_{NR}$ and $\M_{NSR}$, which contain all no-regret/no-swap-regret menus, Lemma \ref{lem:sub-mean-based} implies that $\M_{MB}$ is \emph{contained} in all mean-based menus. Since there exist mean-based algorithms that are no-regret (e.g., multiplicative weights), Lemma \ref{lem:sub-mean-based} immediately also implies that the mean-based menu is a subset of the no-regret menu (that is, $\MB \subseteq \M_{NR}$)\footnote{It is natural to ask whether $\MB$ is in general just equal to $\M_{NR}$. In Appendix \ref{app:mb_nr_gap}, we show this is not the case.}.

To construct our counterexample, we will specifically consider games with $m=2$ actions for the optimizer and $n=3$ actions for the learner, where the learner's payoff $u_L$ is specified by the following $3 \times 2$ matrix\footnote{Although we present all the results in this section for a specific learner's payoff $u_L$, they continue to hold for a positive-measure set of perturbations of this payoff function; see Appendix~\ref{app:mean_based_pareto_dominated} for details.}:

\begin{equation}\label{eq:game}
u_L = \begin{bmatrix}
  0 & 0 \\
 -1/6 & 1/3 \\
 -1/2 & 1/2
\end{bmatrix}.
\end{equation}

For convenience, we will label the learner's three actions (in order) $A$, $B$, and $C$, and the optimizer's two actions as $N$ and $Y$ (so e.g. $u_L(Y, B) = 1/3$, and $u_L(N, 0.5A + 0.5C) = -1/4$). As mentioned in the introduction, this example originates from an application in \cite{guruganesh2024contracting} for designing dynamic strategies for principal-agent problems when an agent runs a mean-based learning algorithm (the details of this application are otherwise unimportant). %All our results about~\ref{eq:game} generalize to learner payoffs generated by adding a small perturbation to this learner payoff (See~\eqref{eq:perturbed_game}), and are therefore true for a positive measure set of learner payoffs. Where necessary, we discuss generalizing the proofs in this section in the Appendix.

An interesting property of this choice of $u_L$ is that there exist points in $\MB^{-}$ not contained within $\M_{NSR}^{-}$.

\begin{theorem}\label{thm:high-mb-swap-regret}
For the choice of $u_L$ in \eqref{eq:game}, $\MB^{-} \not \subseteq \M_{NSR}^{-}$.
\end{theorem}
\begin{proof}
Consider the continuous-time trajectory $\tau = \{(N/3 + 2Y/3, 1/2, C), (N, 1/2, B)\}$. First, note that it is indeed a valid trajectory: we can check that $\ox_1 = N/3 + 2Y/3$, $\ox_2 = 2N/3 + Y/3$, $\BR_{L}(N/3 + 2Y/3) = \{B, C\}$, and that $\BR_{L}(2N/3 + Y/3) = \{A, B\}$. For this trajectory, $\Prof(\tau) = (1/6) (N \otimes C) + (1/3) (Y \otimes C) + (1/2) (N \otimes B)$.

For this game, $U_{ZS} = 0$ (the learner can guarantee non-negative utility by playing $Y$ and the optimizer can guarantee non-positive utility for the learner by playing $N$). Note that $u_L(\Prof(\tau)) = (1/6)(-1/2) + (1/3)(1/2) + (1/2)(-1/6) = 0$, so $\Prof(\tau)$ lies in $\MB^{-}$. But the swap regret of $\Prof(\tau)$ is positive, since by swapping all weight on $B$ to $A$ increases the learner's average utility by $1/12$, so $\Prof(\tau) \not\in \M_{NSR}$. 
\end{proof}

Combined with our characterization of Pareto-optimal no-regret menus (Theorem \ref{thm:pareto-optimal-characterization}), the above theorem implies that any no-regret mean-based algorithm with a polytopal menu is Pareto-dominated. In the next two sections, we will show that for the set of games we are considering a large class of mean-based algorithms have polytopal menus.

\subsection{The mean-based menu is a polytope}
\label{sec:mb-is-polytope}

Our first goal will be to show that the mean-based menu $\MB$ for this game is a polytope. Our main technique will be to show that trajectories $\tau$ whose profiles correspond to extreme points of $\MB$ must be simple and highly structured (e.g. have a small number of segments). We can then write down explicit systems of finitely many linear inequalities to characterize these profiles (implying that their convex closure $\MB$ must be a polytope). 

%\jon{add a figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/mb_trajectory.pdf}
    \caption{A simple trajectory with five segments.}
    \label{fig:mb_trajectory}
\end{figure}

Throughout the following arguments, it will be helpful to geometrically visualize a trajectory by thinking about how the cumulative strategy taken by the optimizer evolves over time. This starts at zero and traces out a polygonal line with breakpoints $X_{i} = \sum_{j=1}^{i} x_{j}t_{j}$, with segment $i$ of the trajectory taking place between breakpoints $X_{i-1}$ and $X_{i}$ (see Figure~\ref{fig:mb_trajectory}. Since the optimizer's strategy each round belongs to $\Delta_{2}$, this trajectory always stays in the positive quadrant $\Rset_{\geq 0}^2$, and strictly increases in $\ell_{1}$-norm over time. %\jon{I just realized that there is a tiny notational collision between the pure strategy labeled $X$ and using $X_i$ to denote the cumulative strategy of the adversary (the $x$ player). If we want to handle it, I think it is probably better to relabel $X$ and $Y$ to something else than to change the notation for $X_i$ (but I also think it's fine to leave it in).}~\esh{Action name changed to N (from X)}

% \nat{what does this mean? In the trajectory space the position is about cumulative payoff not what distribution you play} \jon{sorry, I changed the state space from ``cumulative utility for the learner'' to ``cumulative strategy played by the optimizer''; they are equivalent up to a linear change of variables, but while writing I felt it was a bit easier to describe things in the cumulative strategy space. happy to switch back if it is somehow easier for the proofs}

The best-response condition on $b_i$ can also be interpreted through this diagram. The quadrant can be divided into three cones $R_{A}, R_{B}, R_{C}$, where for any $j \in \{A, B, C\}$, $R_{j}$ contains the states $X$ where pure strategy $j$ for the learner is a best response to the normalized historical strategy $X / |X|_{1}$. Separating $R_{A}$ and $R_{B}$ is a ray $r_{AB}$ (where actions 1 and 2 are both best-responses to states on this ray); similarly, separating $R_{B}$ and $R_{C}$ is a ray $r_{BC}$. Here (and throughout this section) we use the term \emph{ray} to specifically refer to a set of points that lie on the same path through the origin (i.e., a set of states $X$ with the same normalized historical strategy $X/|X|_1$). 

We begin with several simplifications of trajectories that are not specific to the payoff matrix above, but hold for any game. We first show it suffices to consider trajectories where no two consecutive segments lie in the same cone.

\begin{lemma}\label{lem:switch_regions}
For any $\tau \in \cT$, there exists a trajectory $\tau' \in \cT$ such that $\Prof(\tau') = \Prof(\tau)$, and such that there are no two consecutive segments in $\tau'$ where the learner best-responds with the same action (i.e., $b_{i} \neq b_{i+1}$ for all $i$).
\end{lemma}
\begin{proof}
Consider a trajectory $\tau$ with two consecutive segments of the form $(x_i, t_i, b)$ and $(x_{i+1}, t_{i+1}, b)$ for some $b \in \{A, B, C\}$. Note that replacing these two segments with the single segment $((x_it_{i} + x_{i+1}t_{i+1})/(t_i + t_{i+1}), t_i + t_{i+1}, b)$ does not change the profile of the trajectory (e.g., in Figure \ref{fig:basic_trajectory}, we can average the first two segments into a single segment lying along $r_{AB}$). We can form $\tau'$ by repeating this process until no two consecutive $b_i$ are equal. 
\end{proof}



We similarly show that we cannot have three consecutive segments that lie along the same ray.

\begin{lemma}\label{lem:leave_ray}
We say a segment $(x_i, \tau_i, b_i)$ of a trajectory lies along a ray $r$ if both $X_{i-1}$ and $X_{i}$ lie on $r$. For any $\tau \in \cT$, there exists a trajectory $\tau' \in \cT$ such that $\Prof(\tau') = \Prof(\tau)$ and such that there are no three consecutive segments of $\tau'$ that lie along the same ray.
\end{lemma}
\begin{proof}
Assume $\tau$ contains a sequence of three segments $(x_i, t_i, b_i)$, $(x_{i+1}, t_{i+1}, b_{i+1})$, and $(x_{i+2}, t_{i+2}, b_{i+2})$ that all lie along the same ray $r$. This means that $X_{i}$, $X_{i+1}$, and $X_{i+2}$ are all non-zero points that lie on $r$, and therefore that $\ox_i = \ox_{i+1} = \ox_{i+2}$. This means that $b_{i}$, $b_{i+1}$, and $b_{i+2}$ must all belong to $\BR_L(\ox_i)$. Note also that this means that we can arbitrarily reorder these segments without affecting $\Prof(\tau)$.

However, $\BR_L(\ox_i)$ contains at most two actions for the agent (it is a singleton unless $\ox_i$ lies along $r_{AB}$ or $r_{BC}$, in which case it equals $\{A, B\}$ or $\{B, C\}$ respectively). This means that at least two of $\{b_{i}, b_{i+1}, b_{i+2}\}$ must be equal. By rearranging these segments so they are consecutive and applying the reduction in Lemma \ref{lem:switch_regions}, we can decrease the total number of segments in our trajectory while keeping $\Prof(\tau)$ invariant. We can repeatedly do this until we achieve the desired $\tau'$. 
\end{proof}

% \esh{I'm a bit confused by the proof of this statement. While I'm convinced the result is true for the payoffs we're looking at, the first part of the proof, seemingly written for general games, is something I'm not sure about - in particular, we only seem to get $x_i = x_{i+1} = x_{i+2}$ and not the stronger result that $\ox_i = \ox_{i+1} = \ox_{i+2}$. Perhaps I'm missing some reasoning here, but it seems like there are payoffs for which the former is true but not the latter. }

Finally we show that we only need to consider trajectories that end on a best-response boundary (or single segment trajectories).

\begin{lemma}\label{lem:end_on_br}
For any $\tau \in \cT$, we can write $\Prof(\tau)$ as a convex combination of profiles $\Prof(\tau')$ of trajectories $\tau'$ that either: i. consist of a single segment, or ii. terminate on a best-response boundary (i.e., $|\BR_L(\ox_k)| \geq 2$). 
\end{lemma}
\begin{proof}
We will proceed by induction on the number of segments in $\tau$. Assume $\tau$ is a trajectory with $k \geq 2$ segments that does not terminate on a best-response boundary (so $\BR_L(\ox_k) = \{b_k\}$). Let $(x_k, t_k, b_k)$ be the last segment of this trajectory, and let $\tau_{pre}$ be the trajectory formed by the first $k-1$ segments.

There are two cases. First, if $b_k \in \BR_L(x_k)$, then the single segment $(x_k, t_k, b_k)$ is itself a valid trajectory; call this trajectory $\tau_{post}$. Then $\Prof(\tau)$ is a convex combination of $\Prof(\tau_{pre})$ and $\Prof(\tau_{post})$, which both satisfy the inductive hypothesis.

Second, if $b_k \not\in \BR_L(x_k)$, then let $\tau(t)$ be the trajectory formed by replacing $t_k$ with $t$ (so the last segment becomes $(x_k, t, b_k)$). Since $b_k \not\in \BR_L(x_k)$, there is a maximal $t$ for which $\tau(t)$ is a valid trajectory (since for large enough $t$, $\ox_k$ will converge to $x_k$ and $b_k$ will no longer be a best response to $\ox_k$). Let $t_{k}^{\max}$ be this maximal $t$ and note that $\tau(t_{k}^{\max})$ has the property that it terminates on a best-response boundary. But now note that $\Prof(\tau)$ can be written as the convex combination of $\Prof(\tau(0))$ and $\Prof(\tau(t_k^{\max}))$ both of which satisfy the constraints of the lemma (the first by the inductive hypothesis, as it has one fewer segment, and the second because it terminates on a best-response boundary).
\end{proof}

We will say a \textit{proper trajectory} is a trajectory that satisfies the conditions of Lemmas \ref{lem:switch_regions}, \ref{lem:leave_ray}, and \ref{lem:end_on_br}. A consequence of these lemmas is that  $\MB$ is also the convex closure of the profiles of all proper trajectories, so we can restrict our attention to proper trajectories from now on. 

Before we further simplify the class of proper trajectories, we introduce some additional notation to describe suffixes of valid trajectories. We define an \emph{offset trajectory} $(\tau, X_0)$ to be a pair containing a trajectory $\tau$ and a starting point $X_0 \in \Rset^{2}_{\geq 0}$. Similar to ordinary trajectories, in order for an offset trajectory to be valid, we must have that $b_{i} \in \BR(\overline{x}_{i-1}) \cap \BR(\overline{x}_{i})$; however, for offset trajectories, the definition of $\overline{x}_i$ changes to incorporate the starting point $X_{0}$ via

$$\overline{x}_i = \frac{X_{0} + \sum_{j=1}^{i}t_jx_{j}}{||X_{0}||_{1} + \sum_{j=1}^{i}t_{j}}.$$

\noindent
The profile $\Prof(\tau, X_0)$ of an offset trajectory is defined identically to $\Prof(\tau)$ (in particular, it only depends on the segments after $X_0$, and not directly on $X_0$). For offset trajectories, we define $X_i = X_0 + \sum_{j=1}^{i} x_{j}t_{j}$. We will commonly use offset trajectories to describe suffixes of proper trajectories -- for example, we can model the suffix of $\tau = \{(x_1, t_1, b_1), \dots, (x_k, t_k, b_k)\}$ starting at segment $j$ with the offset trajectory $(\tau', X_0')$, where $\tau'$ is the suffix of $\tau$ starting at segment $j$ and $X_0' = X_{j-1}$. 
% \esh{Are the $X_i$ variables also redefined to account for the offset? And does the profile take $X_0$ into consideration? -- If I understand correctly, the answer is yes and no respectively (perhaps the second point is already made in the above sentence, but the ambiguity about the $X_i$s is a bit confusing for me to reconcile); and would it make sense if we emphasized the result below to state that - "it is not clear that $\tau$ is a valid trajectory, since only the altered validity conditions are satisfied. Nonetheless; $\Prof(\tau)$ is shown to be in $\MB$." }

% \esh{Perhaps this is a good place to explicitly define the profile of a suffix? I think I understand how it ties in with offsets (the offset being the cumulative effect of the prefix), but I wonder if it'd help to state it explicitly?}

If an offset trajectory of length $k$ has the property that $X_{k} = \lambda X_{0}$ for some $\lambda > 1$, we call this trajectory a \emph{spiral}. The following lemma shows that the profile of any spiral belongs to $\MB$.

\begin{lemma}\label{lem:spiral}
Let $\psi = (\tau, X_0)$ be a spiral. Then $\Prof(\psi) \in \MB$.
\end{lemma}
\begin{proof}
Let $x_0 = X_0 / ||X_0||_1 \in \Delta_2$, and choose an arbitrary $b_0 \in \BR_L(x_0)$. Also, let $\lambda = X_k/X_0$ be the scaling factor of $\psi$. Fix any positive integer $n \geq 1$, and consider the trajectory $\pi_n$ formed by concatenating the initial segment $(x_0, ||X_0||_1, b_0)$ with the offset trajectories $(\lambda^i\tau, \lambda^iX_0)$ for each $1 \leq i \leq n$ in that order. Note that this forms a valid trajectory since the $i$th offset trajectory ends at $\lambda^{i+1}X_0$, the starting point of the next trajectory.

Let $T_n$ be the total length of trajectory $\pi_n$. Note that $\Prof(\pi_n) = (||X_0||_1 (x_0 \otimes b_0) + (T_n - ||X_0||_1) \Prof(\tau))/T_n$. As $n \rightarrow \infty$, this approaches $\Prof(\tau)$, so $\Prof(\tau) \in \MB$ (recall $\MB$ is the convex closure of all profiles of trajectories).
\end{proof}

We say a trajectory or spiral is \emph{primitive} if it has no proper suffix that is a spiral. The following lemma shows that it suffices to consider primitive trajectories and spirals when computing $\MB$. 

% \nat{It seems like all spirals are also trajectories? Maybe I am misunderstanding the definitions.}\jon{The way I've defined things spirals are offset trajectories but not (proper) trajectories... but maybe this terminology is confusing.}


\begin{lemma}\label{lem:primitive}
Let $\tau$ be a proper trajectory. Then $\Prof(\tau)$ can be written as a convex combination of the profiles of primitive trajectories and primitive spirals.
\end{lemma}
\begin{proof}
We induct on the length of the trajectory. All trajectories with one segment are primitive.

Consider a trajectory $\tau$ with length $k$. If $\tau$ is not primitive, some suffix of $\tau$ is a primitive spiral. Divide $\tau$ into its prefix trajectory $\tau_{pre}$ and this suffix spiral  $\psi_{suff}$. Now, $\Prof(\tau)$ is a convex combination (weighted by total duration) of $\Prof(\tau_{pre})$ and $\Prof(\psi_{suff})$. But $\psi_{suff}$ is a primitive cycle, and $\Prof(\tau_{pre})$ is the convex combination of profiles of primitive cycles/trajectories by the inductive hypothesis. This completes the proof.
\end{proof}

One consequence of Lemma \ref{lem:primitive} is that $\MB$ is the convex hull of the profiles of all primitive trajectories and cycles. It is here where we will finally use our specific choice of game (or more accurately, the fact that the learner only has three actions and hence there are only three regions in the state space). 

\begin{lemma}\label{lem:characterize_primitive}
Any primitive trajectory or primitive spiral for a game with $m = 2$ and $n = 3$ has at most three segments.
\end{lemma}
\begin{proof}
Consider a primitive trajectory $\tau$ with $k > 3$ segments. Since it is a proper trajectory, each of the cumulative points $X_1, X_2, \dots X_k$ must lie on a best-response boundary (one of the two rays $r_{AB}$ or $r_{BC}$). Since the trajectory is primitive, all of $X_1, X_2, \dots, X_{k-1}$ must lie on a different ray from $X_k$, and hence must all lie on the same ray. But by Lemma \ref{lem:leave_ray}, we can't have $X_0 = 0$, $X_1$, $X_2$, and $X_3$ all lie on the same ray. Therefore $k-1 \leq 2$, and $k \leq 3$. The argument for primitive spirals works in exactly the same way.
\end{proof}

It only remains to show that there are finitely many extremal profiles of primitive trajectories and spirals. To this end, call the sequence of pure actions $(b_1, b_2, \dots, b_k)$ taken by the learner in a given trajectory (or spiral) the \emph{fingerprint} of that trajectory (or spiral). 

\begin{lemma}\label{lem:fingerprint_lp}
Fix a sequence $\bb \in [n]^{k}$. Then the convex hull of $\Prof(\tau)$ over all trajectories with fingerprint $\bb$ is a polytope (the intersection of finitely many half-spaces). Similarly, the convex hull of $\Prof(\gamma)$ over all spirals with fingerprint $\bb$ is also a polytope.
\end{lemma}
\begin{proof}
First, note that by scaling any spiral or trajectory by a constant, we can normalize the total time $\sum_{i=1}^{k} t_i$ to equal $1$. If this is the case, then we can write $\Prof(\tau) = \sum_{i=1}^{k} (t_ix_i) \otimes b_i$. For a fixed fingerprint $\bb$, this is a linear transformation of the $k$ variables $y_i = t_ix_i$. We will show that the set of possible values for $(y_1, y_2, \dots, y_k)$ forms a polytope.

To do so, we will write an appropriate linear program. Our variables will be the time-weighted optimizer actions $y_1, \dots, y_k \in \Delta_{2}$, times $t_1, \dots, t_k$, and cumulative actions $X_1, X_2, \dots, X_k$ (where $X_i = y_1 + y_2 + \dots + y_i$). In the case of a spiral, $X_0$ will also be one of the variables (for trajectories, we can think of $X_0$ being fixed to $0$). The following finite set of linear constraints precisely characterizes all possible values of these variables for any valid trajectory or spiral with this fingerprint:

\begin{itemize}
    \item Time is normalized to 1: $t_1 + t_2 + \dots + t_k = 1$.
    \item Relation between $X_i$ and $y_i$: $X_i = y_1 + \dots + y_i$.
    \item Relation between $y_i$ and $t_i$: For each $y_i$, $||y_i||_{1} = y_{i, 1} + y_{i, 2} = t_i$.
    \item Best-response constraint: For each $1 \leq i \leq k$, $X_i \in R_{b_i}$ and $X_{i-1} \in R_{b_{i}}$. Here $R_{b_i}$ (in our example, one of $\{R_A, R_B, R_C\}$) is the cone of states where $b_i$ is a best-response, and is specified by finitely many linear constraints.
\end{itemize}

The set of values of $(y_1, y_2, \dots, y_k)$ is a projection of the polytope defined by the above constraints and hence is also a polytope. 
\end{proof}

We can now prove the main result of this section:

\begin{theorem}
\label{thm:mb_is_a_polytope}
The mean-based menu $\MB$ of the learner payoff defined by \eqref{eq:game} is a polytope.
\end{theorem}
\begin{proof}
By Lemma \ref{lem:characterize_primitive}, there are finitely many possible fingerprints for a primitive spiral or trajectory. By Lemma \ref{lem:fingerprint_lp}, the set of profiles for each of these fingerprints is a polytope, so $\MB$ is equal to the convex hull of finitely many polytopes (and hence itself is a polytope).
\end{proof}

As a side note, note that the proof of Lemma \ref{lem:characterize_primitive} allows the optimizer to efficiently optimize against a mean-based learner in this class of games by solving a small finite number of LPs (since the output of the LP described in the proof provides not just the extremal CSP in $\M_{MB}$, but also valid trajectory attaining that CSP). It is an interesting question whether there exists a bound on the total number of possible fingerprints in more general games (a small bound would allow for efficient optimization, but it is not clear any finite bound exists).

% \esh{Would it be worth interpreting best-responses of an optimize on this polytope, after we prove MB= MW? That they solve a LP for each of 3! = 6 fingerprints and pick the best one? This is remarkably reminiscent of the static Stackelberg strategy BR against NSR, but with fingerprints instead of single best responses? This is also related to the MB = MW proof (sine we are doing an implicit decomposition into 2-learner action games and 2-action MW = 2 action NSR) }

\subsection{The mean-based menu equals the FTRL menu}
\label{sec:mb-equals-mwu}


\input{ftrl_mean_based_sec}

%Commenting out Old version and adding in a FTRL based description
%\input{MB_equals_MW_main_old}





%\esh{Add a proof of this}
%\esh{Change the statement for the perturbed game, explain that we have the same characterization in the appendix, and invoke those to complete the proof of Pareto Domination   }


%\esh{Leaving a note here for a couple of auxilary results}

%~\esh{Should we write more about $\M_{NR}$ not being equal to the menu of every MBNR algo? It is not on any critical path, but it's a conceptually interesting contribution}. \nat{Certainly worth putting the example in a footnote at least, and I wouldn't be opposed to adding a pointer to a lemma in the appendix.} 
  

%\nat{Note that we have a disproof that all MBNR algos have the same menu as MB. Use the guess the sequence thing, you get a point with negative regret, this isn't in MW. But MB = MW, done.}

%\esh{We're claiming this result elsewhere - Lemma~\ref{lem:nr_ne_mw}, so we can add a pointer to it, but I'm yet to write the proof, so this is one approach we could take}
%\subsection{Mean Based Algorithms and Online Environments}


%\label{sec:ftl_meanbased}
%\input{ftl_meanbased}

%\subsection{Many Mean-based Algorithms are Pareto Dominated}


%\input{mw_a_polytope}


\begin{comment}
    
\subsection{Results about Mean Based No-Regret Algorithms - Proof of Theorem~\ref{thm:mbnr_pd}}
\nat{This entire section is redundant, keeping around for reference for now while writing some conceptually related results above.}
\input{no_regret_domination}

\end{comment}


==> no_regret_domination.tex <==


\begin{lemma}
For a constant measure set of learner payoffs, there exists a point which 1) has vanishing regret, 2) gets the leader within sublinear factors of their maximin value for the game, and 3) has constant swap regret. 
\end{lemma}
\begin{proof}
Consider the following set of (robust) learner payoffs, where each $\epsilon_i \in (0, \varepsilon]$ for some constant $\varepsilon \in (0, \frac{1}{100})$:

 \[
\begin{bmatrix}
 1 + \epsilon_{1} & 1 + \epsilon_{2} \\
 2+ \epsilon_{3} & -1+ \epsilon_{4} \\
 -1+ \epsilon_{5} & 2+ \epsilon_{6} \\
 \frac{1}{2} - \epsilon_{7} & -1+ \epsilon_{8} \\
 -1 + \epsilon_{9} & \frac{3}{2} - \epsilon_{10} \\
\end{bmatrix}
\]

The only constraint that we enforce is that $\varepsilon_1 < \varepsilon_2$ -- this is a reasonable constraint since it can appear with significant (constant) probability for many simple probability distributions used to draw the $\{\varepsilon_i\}$s.

The set of learner payoffs is said to be robust because the  $\{\varepsilon_i\}$s force this set to have strictly positive measure.

Let the optimizer's two (column) moves be, from left to right, X and Y. Let the learner's five (row) moves be, from top to bottom, A, B, C, D, and E. 

Fix any particular instantiation of the $\epsilon$ values, consider a nash equilibrium of the corresponding zero-sum game. Let the optimizer's minimax distribution in this NE put probability $\alpha$ on X and $1-\alpha$ on Y. 

We make a couple of observations about the minimax value $M$ of this game. 

\begin{enumerate}
    \item Since the learner can always guarantee themselves value larger than $1$ by playing action $A$, $M > 1$.
    \item If the optimizer plays distribution $(1/2 X, 1/2 Y)$, then the learner's best response is $A$ --- implying that $M < 1 + \frac{\varepsilon_1 + \varepsilon_2}{2} \le 1 + \varepsilon$.
\end{enumerate}

Using the above observations, we can infer $\frac{1}{3} - \frac{\varepsilon}{3} \le \alpha \le \frac{2}{3} + \frac{\varepsilon}{3}$ (by measuring the learner payoff obtained by responding with actions B and D).

Additionally, since we have assumed that $\varepsilon_1 < \varepsilon_2$, it must be the case that $\alpha \ge 1/2$, since otherwise the learner could best respond and get value larger than $1 + \frac{\varepsilon_1 + \varepsilon_2}{2}$.


The point of interest $X$ in the menu space has the following empirical distribution over action pairs - (D,X) w.p. $\beta$; (B,X) w.p. $\alpha - \beta$ and (E,Y) w.p. $1-\alpha$ for some $\beta \in (0, \alpha)$ which we will specify shortly.

The learner's payoff changes linearly and therefore as a continuous function of $\beta$. At $\beta = 0$, the learner's payoff at X is at least $1.74$. At $\beta = \alpha$, the learner's payoff is less than $1$. The intermediate value theorem tells us that there exists a $\beta \in (0, \alpha)$ such that the learner's payoff is exactly the maximin value $M$ -- we pick precisely this value of $\beta$.

Thus, $X$ has the following properties --

\begin{enumerate}
    \item $X$ gets the leader their maximin value for the game
    \item $X$ has vanishing regret, since the marginal distribution of the optimizer in $X$ is precisely the minimax strategy and the learners gets the maximin value (which can be obtained by best responding to the minimax)
    \item $X$ has significant (constant) swap regret -- since the action pair (E,Y) appears with probability $1-\alpha \ge 0.32$. The swap function that generates significant regret only does the operation of replacing action E with action C.
\end{enumerate}
%Now note that A must be a best response to $\beta$. 

%To see this, assume for contradiction that A is not a best response. So there is some best response $m \neq A$ which gets payoff strictly greater than playing A. If this move is B, that means that $\beta_{X} > $



%REFUTE THIS. 

%Now, we will construct our point as follows: 
\end{proof}


\begin{lemma}
\label{lemma:non_robust_nr_rps}
There exists a mean-based no-regret learning algorithm that includes a point in its menu which has non-vanishing swap regret and gives the learner their maximin value.  
\end{lemma}

\begin{proof}
Let us define the learning algorithm $\mathcal{A}$ to be as follows: begin by playing your earliest-indexed move. Then play FTL, tiebreaking towards a move that was not played in the previous round. Also run a MW update on move weights in the background. If at any point the regret of the algorithm is strictly more than the largest payoff gap in the matrix (call this $c$), defect to permanently playing according to the MW algorithm. 

Note first that this algorithm is mean-based; both FTL and MW are mean-based, and as the mean-based condition is a condition that holds on a per-round basis over the history of play, and at every round either FTL or MW is played over the same history of play, the condition continues to hold in a per-round basis in $\mathcal{A}$. 

Secondly, this algorithm is also no-regret. To prove this, let $t$ be the time step after which the algorithm defects to MW (if it never defects, $T = T$). We will consider two cases: one where $T - t = o(T)$, and one where $T - t = \Omega(T)$.
\begin{itemize}
    \item If $T - t = o(T)$, then the total regret can be upper bounded by the regret in the first $t$ rounds, $c$, plus the maximum regret that could be attained in $o(T)$ rounds, $c \cdot o(T)$. Therefore the total regret is $(c+1) \cdot o(T)$, which is vanishing in $T$.
    \item If $T - t = \Omega(T)$, then let us assume for contradiction that the regret incurred by MW in this sequence is also $\Omega(T)$. But MW is a no-regret algorithm, so this would mean that the total regret incurred in the first $t$ rounds must be a negative value on the order of $-\Omega(T) \leq -\Omega(t)$. But this implies that on the $t$-length prefix of play, multiplicative weights gets regret of $-\Omega(t)$
\end{itemize}


For the first $t$ rounds, the learner can never incur total regret more than a constant value, independent of $T$. For the final $T - t$ rounds, the learner incurs the 
After the algorithm defects, it is incurring regret exactly as much as the MW algorithm is. Therefore we can upper bound the regret of $\mathcal{A}$ by the regret of the MW algorithm, which is vanishing with T.


Now, we will show a game and an optimizer sequence such that the induced history of play against  $\mathcal{A}$ is a maximin learner value point with constant swap regret. The game is Rock Paper Scissors, with loss/tie/win payoffs of $-1$, $0$ and $1$. The optimizer sequence is as follows:

$$RPP(SSSRRRPPP)^*$$
Where the moves in parentheses can be repeated until time $T$, cutting off in the middle if necessary. 

Let us consider what $\mathcal{A}$ will play against a prefix of this sequence. We will do this by showing a table of the total payoffs of Rock, Paper and Scissors for the learner at each point in the process. As long as FTL is still being played, recall that $\mathcal{A}$ will always play the best-performing move in hindsight, tiebreaking in favor of a new best-in-hindsight move. Furthermore, note that we must keep track of the total payoff for the leader under FTL and its regret to check whether the $\mathcal{A}$ will defect from FTL. In this case, the regret boundary is the performance of MW, plus $1 - (-1) = 2$. 

Note that the payoff values at round $t$ are all computed over rounds $1$ to $t-1$; that is, they are the values that the learner uses in round $t$, not the ones resulting from round $t$. For verification, one must read this table column-by-column from left to right, reading from up to down in each column. 

\begin{center}
\begin{tabular}{ |c|c|c|c|c|c|c|c|c|c|c|c|c|c| } 
 \hline
 Time Step & 1 & 2 & 3 & 4 &  5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 \\
 In hindsight payoff for R  & 0 & 0 & -1 & -2 & -1 & 0 & 1 & 1 & 1 & 1 & 0 & -1 & -2 \\ 
 In hindsight payoff for P & 0 & 1 & 1 & 1 & 0 & -1 & -2 & -1 & 0 & 1 & 1 & 1 & 1 \\ 
 In hindsight payoff for S & 0 & -1 & 0 & 1 & 1 & 1 & 1 & 0 & -1 & -2 & -1 & 0 & 1 \\ 
 Cumulative payoff under FTL & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 Total External Regret under FTL & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\
 Defect from FTL? & N & N & N & N & N & N & N & N & N & N & N & N & N \\
Learner Move & R & P & P & S & S & S & R & R & R & P & P & P & S \\
Optimizer Move & R & P & P & S & S & S & R & R & R & P & P & P & S \\ 


 
 \hline
\end{tabular}
\end{center}
 Note that throughout this prefix of play, the learner never defects from FTL and always plays the same move as the optimizer. Note also that the state of the game before the learner moves at time step 4 is exactly the same as the state of the game before the learner moves at time step 13. Thus, if the optimizer repeatedly plays the same moves that they played from time steps 4 and 12 (as they do in our proposed sequence), the table values will continue this cycle, and the learner will continue to always play the same move as the optimizer. This means that, whatever time step $T$ the repeated game ends, the payoff for the learner will be $0$, which is also the maximin value for the game.
 
 However, the swap regret of the algorithm will be very large. This is because all the rounds that the learner played R, the optimizer played R. So the learner gets $0$ on every step of this subsequence where they play R, but would get $1$ on every step of this subsequence if they played P. The same logic holds for the subsequence where the learner plays paper, and that in which they play scissors. As the learner incurs swap regret of $1$ for every time step in every one of these subsequences, the total swap regret is $T$.
 
 Therefore we have a game, an optimizer sequence and a mean-based no-regret learner algorithm that together induce a sequence of play which gives the learner their maximin value and also has non-vanishing swap regret. 
\end{proof}


We want a stronger version of Lemma~\ref{lemma:non_robust_nr_rps}, which is to show that any mean based algorithm has similar properties for a non measure zero set of learner payoffs. To this end, we introduce the robust-RPS (robust rock, paper and scissors) game with the following payoff matrix for the learner.

 \[
\begin{bmatrix}
 & R & P & S \\
R & \varepsilon_{1} & -1 + \varepsilon_2 & 1 + \varepsilon_{3} \\
P & 1 + \varepsilon_4 &  \varepsilon_{5} & -1+ \varepsilon_{6} \\
 S & -1+ \varepsilon_{7} & 1+ \varepsilon_{8} & \varepsilon_9 
\end{bmatrix}
\]

Each $\varepsilon_i$ comes from the interval $[0,\varepsilon]$ where $\varepsilon \le 0.00001$.

We make the following observations about this (parameterized set of) learner payoff(s).

\begin{lemma}
\label{lem:unique_minimax}
The robust-RPS game always has a unique minimax distribution for which rock, paper and scissors 
all have probability at least $\frac{1}{3} - \frac{2\varepsilon}{3}$. Additionally, the learner is indifferent between the three actions as a response to the minimax distribution.
\end{lemma}
\begin{proof}
Let the minimizing player be the column player. First, we will prove that against any minimax distribution of the game $d = (d_r, d_p, d_s)$, we have that the maximization player is indifferent between $r$, $p$ and $s$. 
Assume for contradiction that this is not the case. Then, either there is one unique maximizing response, or one unique minimizing response. Let us first consider the case where there is one unique maximizing response [TODO: other case]. further assume w.l.o.g that the unique maximizing response to $d$ is $r$. Then, there exists some constant $y$ such that $$\mathbb{E}_{x \sim d}[\mu(r,x)] > \mathbb{E}_{x \sim d}[\mu(p,x)] + y$$
and 
$$\mathbb{E}_{x \sim d}[\mu(r,x)] > \mathbb{E}_{x \sim d}[\mu(s,x)] + y$$

Note that given the payoff matrix defined above, $y$ is greater than $0$ and is at most $2 + 2\varepsilon < 3$. 

Now, consider the following distribution $\hat{d} = (1 - \frac{y}{4})d + \frac{y}{4} s$. Note that this is a valid distribution given the bounds on the size of $y$. The best response to $\hat{d}$ is still rock, as
\begin{align*}
\mathbb{E}_{x \sim \hat{d}}[\mu(x,r)]  
& = (1 - \frac{y}{4})\mathbb{E}_{x \sim d}[\mu(r,x)] + \frac{y}{4} \mu(s,r) \\
& > (1 - \frac{y}{4})(\mathbb{E}_{x \sim d}[\mu(s,x)] + y) + \frac{y}{4} \mu(s,r)  \\
& = (1 - \frac{y}{4})(\mathbb{E}_{x \sim d}[\mu(s,x)]) + \frac{y}{4} \mu(r,s) + y(1 - \frac{y}{4}) \\
& = \mathbb{E}_{x \sim \hat{d}}[\mu(s,x)] + y(1 - \frac{y}{4}) \\
& > \mathbb{E}_{x \sim \hat{d}}[\mu(s,x)] + \frac{y}{4} \tag{As $y < 3$} \\
\end{align*}

An equivalent proof shows that 

$$\mathbb{E}_{x \sim \hat{d}}[\mu(r,x)] > \mathbb{E}_{x \sim \hat{d}}[\mu(p,x)] + \frac{y}{4}$$

As the best response to $\hat{d}$ is rock, the maximizing response to $\hat{d}$ gets the maximizing player a payoff of 

\begin{align*}
& (1 - \frac{y}{4})\mathbb{E}_{x \sim d}[\mu(r,x)] + \frac{y}{4} \mu(r,s) \\
& = \mathbb{E}_{x \sim d}[\mu(r,x)] + (\mu(r,s) - \mathbb{E}_{x \sim d}[\mu(r,x)]) \frac{y}{4} \\
& \leq \mathbb{E}_{x \sim d}[\mu(r,x)] \tag{By the fact that $d$ is a minimax distribution, and $r$ is a best response to $\hat{d}$ and $d$} \\
& \rightarrow (\mu(r,s) - \mathbb{E}_{x \sim d}[\mu(r,x)]) \leq 0 \\
& \rightarrow d = s
\end{align*}

So the minimax distribution is is the pure strategy $s$. This means that the maximizing player can get a payoff of $1 + \varepsilon_{3} \geq 1$ by playing $r$. However, if the minimizing player had instead played $\bar{d} = r \sim \frac{1}{3}, p \sim \frac{1}{3}, s \sim \frac{1}{3}$, the maximization player's payoff would have been at most
\begin{align*}
& \max(\frac{1}{3}\varepsilon_{1} + \frac{1}{3}(-1 + \varepsilon_{2}) + \frac{1}{3}(1 + \varepsilon_{3}), \frac{1}{3}(1 + \varepsilon_{4}) + \frac{1}{3}\varepsilon_{5} + \frac{1}{3}(-1 + \varepsilon_{6}), \frac{1}{3}(\varepsilon_{7}-1) + \frac{1}{3}(1 + \varepsilon_{8}) + \frac{1}{3} \varepsilon_{9}) \\
& \leq \max(\frac{1}{3}(-1 + \varepsilon) + \frac{1}{3}(1 + \varepsilon), \frac{1}{3}(1 + \varepsilon) + \frac{1}{3}\varepsilon + \frac{1}{3}(-1 + \varepsilon), \frac{1}{3}(\varepsilon-1) + \frac{1}{3}(1 + \varepsilon) + \frac{1}{3} \varepsilon) \\
& = \epsilon < 1
\end{align*}

$d$ is not in fact the minimax distribution of the game, derving a contradiction. Therefore, against any minmax distribution of the game $d = (d_r, d_p, d_s)$, we have that the maximization player is indifferent between $r$, $p$ and $s$. 

We are now ready to prove the lemma. As the maximization player must be indifferent between the three moves under $d$, we get that
\begin{align}
& d_{r}\varepsilon_{1} + d_{p}(-1 + \varepsilon_{2}) + d_{s}(1 + \varepsilon_{3}) - (d_{r}(1 + \varepsilon_{4}) + d_{p}\varepsilon_{5} + d_{s}(-1 + \varepsilon_{6})) =  0 \tag{By indifference between r and p} \\
& \rightarrow 2d_{s} - d_{r} - d_{p} = d_{r}(\varepsilon_{4} - \varepsilon_{1}) + d_{p}(\varepsilon_{5} - \varepsilon_{2}) + d_{s}(\varepsilon_{6}-\varepsilon_{3}) \\ 
&\rightarrow 2d_{s} - d_{r} - d_{p} \leq \varepsilon \\
& \leftrightarrow d_{s}\leq \frac{\varepsilon + d_{r} + d_{p}}{2}  \label{rp} \\
\end{align}

Using the indifference between $p$ and $s$ and between $s$ and $r$, we also get that

\begin{align}
 d_{r}\leq \frac{\varepsilon + d_{p} + d_{s}}{2} \label{ps}
\end{align}
and
\begin{align}
 d_{p}\leq \frac{\varepsilon + d_{s} + d_{r}}{2} \label{sr}
\end{align}

Finally, note that

\begin{align*}
&d_{r} + d_{p} + d_{s} = 1 \\
&\rightarrow d_{r} + d_{p} +  \frac{\varepsilon + d_{r} + d_{p}}{2} \geq 1 \tag{By~\ref{rp}}\\
& \leftrightarrow \frac{3d_{r}}{2} + \frac{3d_{p}}{2} + \frac{\varepsilon}{2} \geq 1 \\
& \leftrightarrow d_{r} + d_{p} \geq \frac{2}{3} - \frac{\epsilon}{3}
\end{align*}

One can similarly derive using~\ref{ps} and~\ref{sr} that

\begin{align*}
d_{p} + d_{s} \geq \frac{2}{3} - \frac{\epsilon}{3}
\end{align*}
and

\begin{align*}
d_{s} + d_{r} \geq \frac{2}{3} - \frac{\epsilon}{3}
\end{align*}

\end{proof}

\begin{lemma}
\label{lem:minimax_split}
For every robust-RPS game, there exist three distributions $\alpha$, $\beta$ and $\gamma$ such that $\frac{\alpha + \beta + \gamma}{3}$ is equal to the minimax distribution of the game, $\alpha_{r} \geq 0.9$,  $\beta_{p} \geq 0.9$. and  $\gamma_{s} \geq 0.9$.
\end{lemma}
\begin{proof}
We will prove this by showing an algorithm which, from any minimax distribution over rock, paper and scissors $d_r, d_p, d_s$ from the $\varepsilon$-robust game, produces $\alpha$, $\beta$ and $\gamma$ fulfilling the above specifications. 

The algorithms operates by filling in $\alpha$, $\beta$ and $\gamma$ in a step-by-step manner: first, it will select 
\end{proof}


We are ready to prove our main technical result about mean-based no-regret algorithms. 

\esh{The proof of this result has been written assuming that the learner can see the distribution played by the optimizer and we measure expected payoffs as the objective, however we think the result also works in the setting where the learner only observes realized actions, through the use of concentration}

\begin{lemma}
\label{lemma:robust_mb_sr_nr}
For the learner payoffs defined by the robust-RPS game,
every mean-based no-regret learning algorithm includes a point in its menu that has non-vanishing swap regret and gives the learner their maximin value. 
\end{lemma}

\begin{proof}
    Consider any mean-based no-regret algorithm $\A$. By definition, it is $\gamma$-mean based for some $\gamma = o(1)$. Let $\gamma T = O(T^\alpha)$ for some $ 0 \le \alpha < 1$ and let $\beta = \frac{1+\alpha}{2}$. Clearly, $\beta \in (0,1)$. 
    \esh{Is $\alpha \ge 0$ a reasonable assumption? If an algorithm is $\gamma$-mean based, then it is also $\gamma'$ mean based where $\gamma'$ is pointwise larger than $\gamma$, so we can assume WLOG that $\gamma(t) \ge \frac{1}{T}$ - Sanity check this please?}
   
    
    To show such a point in the menu of the algorithm $\A$ for every parametric instantiation of the robust-RPS game, we show a sequence that the optimizer to certify the existence of a point in the menu with the desired characteristics. Fixing the parameters, let $\delta$ be the unique minimax strategy of the optimizer (using Lemma~\ref{lem:unique_minimax}) with minimax value $V$. By Lemma~\ref{lem:minimax_split}, we know there are three distributions $\kappa, \mu, \lambda$ over optimizer actions such that $\frac{\kappa + \mu + \lambda}{3}$ is equal to the minmax distribution of the game and $\kappa_{r} \geq 0.9$,  $\mu_{p} \geq 0.9$. and  $\lambda_{s} \geq 0.9$.

    The sequence acts in $T^{1-\beta}/3$ epochs of length $3 T^\beta$. Excepting the first epoch, each epoch consists of the distribution $\kappa$ is played $T^\beta$ times, followed by the distribution  $
    \mu$ for $T^\beta$ times followed by the distribution  $
    \lambda$ for $T^\beta$ times. The epochs end at times $T_0, T_1, T_2 \cdots T_{\frac{T^{1-\beta}}{3}-1}$. 

    To help analyze the behaviour of algorithm $\A$ against this sequence, we track some information about the state of the algorithm, specifically the cumulative historical payoffs of the three actions. We compress this into two quantities, the first which measures the difference in cumulative historical payoffs between rock and scissors, and the second measuring the same difference between paper and scissors. After round $t$, this partial state is recorded as $(u_t,v_t)$ where $u_t = \sigma^R_{t+1} - \sigma^S_{t+1}$ and $v_t = \sigma^P_{t+1} - \sigma^S_{t+1}$ where $\sigma^a_t$ denotes the cumulative historical payoff of action $a$ after $t-1$ rounds. These two state variables taken together reveal the best action in hindsight. We observe that rock is the leader (best action in hindsight) after $t$ rounds when $u_t \ge 0$ and $u_t \ge v_t$, paper the leader when $u_t \le v_t$ and $v_t \ge 0$ and scissors the leader when $u_t , v_t \le 0$. The margins of leadership can also be inferred from these two numbers.

    In the first epoch, ending at time $T_0 = T^\beta$, the optimizer plays a special distribution $\upsilon$ in each round such that $(u_{T_0}, v_{T_0}) = (0,-T^\beta)$. We show that such a distribution $\upsilon$ exists by construction.
    \esh{To be filled in. We can make this easier by showing the weaker result that $v_{T_0} = -\theta(T^\beta)$, which should suffice for the rest of the proof}

   \begin{claim}
       At the end of each epoch, the state resets to $(u_{T_0},v_{T_0})$, i.e. $(u_{T_0},v_{T_0}) = (u_{T_i},v_{T_i})$.
   \end{claim}

   {\bf Proof : } The claim  is true by construction for $i =0$. For any other epoch, we observe that the average distribution played by the optimizer within the epoch is $\frac{\kappa + \mu + \lambda}{3}$, which by construction is exactly the minimax distribution. By Lemma~\ref{lem:minimax_split}, we know that the learner is indifferent between their actions against this distribution. Consequently, we have $\sigma^R_{T_i+1} - \sigma^R_{T_{i-1}+1} = \sigma^P_{T_i+1} - \sigma^P_{T_{i-1}+1} = \sigma^S_{T_i+1} - \sigma^S_{T_{i-1}+1}$. This implies $(u_{T_i},v_{T_i}) = (u_{T_{i-1}},v_{T_{i-1}})$, which allows us to prove the above claim through induction on the number of epochs. \qedsymbol{}

   Let $\chi$ be the marginal distribution of the optimizer averaged over the $T$ rounds of play.

    We show that the learner gets exactly their minimax value upto sublinear factors against this sequence. Since $\A$ is a no-regret algorithm, the cumulative payoff of the learner is at $T \cdot \max_a u_L(a,\chi) - o(T)$, which by definition of the minimax value is at least $T \cdot V - o(T)$.

    To show an upper bound on the leader's payoff, we prove the following key claim about the learner algorithm's state over the course of play.

    \begin{claim}
        For all but $o(T)$ rounds, there is a $\gamma$-unique historical leader action.
    \end{claim}

    {\bf Proof : } We ignore the first epoch, since its length is $3T^\beta = o(T)$. It suffices to show that for each $i$, that most of the $i$-th epoch consists of time steps with a $\gamma$-unique historical leader. Without loss of generality, it suffices to analyze the period from $T_0$ to $T_1$ since we have shown that the relative differences between the leader payoffs reset after each epoch. Recall that $\gamma(t)t = t^\alpha$ for any $t$. Since the time steps of interest fall in the range $[3 T^\beta, 6 T^\beta] $, let us replace them by a placeholder variable $T'$ -- the exact value does not matter for our purpose since they are all asymptotically equal.  Each epoch can be divided into three contiguous phases, the $\kappa$, $\mu$ and $\lambda$. Since $\kappa_R \ge 0.9$, each round in the $\kappa$ phase increases the first coordinate ($u_t$) of the state by a value in $[0.9, 1.1]$ and increases the second coordinate ($v_t$) of the state by a value in $[1.9, 2.1]$. At time $T_0$, rock and scissors are tied as historical leader actions. Consequently, after $2T^\alpha$ rounds starting from $T_0$, rock is well separated as the unique leader by a margin of at least $T^\alpha$. Let us call this round $k_1$. Let $k_2$ be the first round after $T_0$ where rock is no longer the leader. If $k_2$ appears before the $\kappa$ phase ends, we observe that for all rounds between $k_1$ and $k_2 - 2T^\alpha$, rock is separated as a leader by a margin of $T^\alpha$. If there are more than $2T^\alpha$ rounds left after $k_2$ in the $\kappa$ phase, we observe that after round $k_2 + 2T^\alpha$, scissors is now  separated as a leader by a margin of $T^\alpha$. If $k_2 > T_0 + T^\beta$, we observe that rock is separated as a leader by a margin of $T^\alpha$ for the rounds from $k_1$ to $T_0 + T^\beta - 2T^\alpha$. Noting that $T^\alpha = \gamma(T) \cdot T \ge \gamma(T') \cdot T'$ for all $T' < T$, we have established that there is a $\gamma$-unique leader for all but at most $6T^\alpha$ rounds in the $\kappa$-phase. A similar analysis will show comparable results in the $\mu$ and $\lambda$ phases, i.e. a $\gamma$-unique leader excepting for $8T^\alpha$ rounds in each phase. To expand on this idea, we consider the time steps corresponding to the end of each phase as well as the time steps corresponding to the changes of leader. We observe that there are exactly three each of the former as well as the latter in each epoch. Aside from an interval of size $2T^\alpha$ around each of these time steps, it can be shown that there is a $\gamma$-unique leader using similar ideas from the analysis of the $\kappa$-phase. As observed earlier, the same analysis can be used for all epochs after the first one. Therefore, there is a $\gamma$-unique leader for all but  at most $
    \frac{22}{3} T^\alpha T^{1-\beta}$ rounds. $\alpha + 1 -\beta = 1 - \frac{1+\alpha}{2} < 1$ finishing the proof of the claim. \qedsymbol{}

    Armed with this claim, we can appeal to Lemma~\ref{lemma:performance_mb_unique} to lower bound the payoff obtained by the mean-based algorithm $\A$ by $T \cdot \max_a u_L(a,\chi) + o(T) + \gamma T$. We also know that the marginal distribution of the optimizer averaged over the time steps is $\frac{T - T^\beta}{T} \delta + \frac{T^\beta}{T} \upsilon$. Upper bounding $T \cdot \max_a u_L(a,\chi)$ by $T \cdot \max_a \frac{T - T^\beta}{T} u_L(a,\delta) + T \cdot \frac{T^\beta}{T} \upsilon$ and replacing the second term by $o(T)$ allows us to upper bound the payoff of the algorithm by $T \cdot \max_a u_L(a,\delta) + o(T) + \gamma T$. But since $\delta$ is the minimax distribution, $\max_a u_L(a,\delta)$ is the minimax value $V$ and since $\A$ is mean-based, $\gamma T = o(T)$, upper bounding the payoff of the algorithm by $T \cdot V + o(T)$. Thus, the learner's cumulative payoff lies in the interval $[T.V -o(T), T.V + o(T)]$, implying that the learner picks up exactly the minimax value on average ignoring subconstant factors. 

    The last part of this proof is to show that the algorithm incurs significant swap regret. We show that the swap function that swaps rock for paper and leaves the other actions unchanged obtains $\Omega(T)$ swap regret. As before, we ignore the first epoch (justified by its sublinear length), analyze the second epoch (from $T_0$ to $T_1$) and argue that the same analysis holds true for every other epoch. Within the second epoch, let $T_\kappa = 4T^\beta$ be the end-point of the $\kappa$-phase, $T_\mu = 5 T^\beta$ be the end-point of the $\mu$-phase and let $T_\lambda = T_1 = 6T^\beta$ be the end of the $\lambda$-phase. As observed earlier, there are exactly three different changes of leader in the second phase, at time $k_1$, where the leader changes from rock to paper, at time $k_2$ where the leader changes from paper to scissors and time $T_1$ where the leader changes (or is tied) from scissors to rock. The key observations we make for demonstrating significant swap regret is that $|k_1 - T_\kappa| \le 0.05 \cdot T^\beta$ and $|k_2 - T_\mu| \le 0.1 \cdot T^\beta$. These inequalities follow from the fact that $\kappa_r \ge 0.99$, $\mu_p \ge 0.99$, $\lambda_s \ge 0.99$ and that all the offsets $\varepsilon_i \le 0.0001$. The first inequality is established first and it helps with establishing the second one. Armed with these observations, we can measure the regret achieved by the proposed swap function. We can safely ignore all rounds without a $\gamma$-unique leader, since there are only $o(T)$ many such rounds. Now, consider the rounds with rock as the $\gamma$-unique leader in the $\kappa$-phase. There are at least $0.89 T^\beta$ such rounds. In all these rounds, rock is played with probability $1-\gamma$. Thus, replacing rock with paper in these rounds builds up a positive regret of at least $0.88 * 0.8 T^\beta = 0.704 T^\beta$ (since $\varepsilon \le 0.001$ and $\kappa_r \ge 0.9$). Outside of the $\kappa$-phase, rock is a $\gamma$-unique leader for at most $0.1 T^\beta$ rounds, so the maximum negative contribution of these rounds to the swap regret can be $-0.22 T^\beta$. Where some other action is the $\gamma$-unique leader, we can ignore the effect of the swap function since rock is picked with negligble probability. Therefore the swap regret in each epoch is at least $0.484 T^\beta$ (trading off a $0.01 T^\beta$ to account for all the asymptotically vanishing factors). Nothing in the analysis is specific to this epoch. Therefore, the overall swap regret is at least $0.16 T$ (again, removing $0.001333 T$ for all the remaining sublinear factors such as the first epoch). This completes the proof of this lemma. 
    
\end{proof}

\esh{Until this point, we have not used any results from polytope menus}

As a corollary of this result, we show that no mean-based no-regret algorithm is pareto-optimal. \\
General idea: for any mean based menu $A$, identify the point which has non-vanishing regret and gives the learner their maximin value. Call this point $p$. Using lemma~\ref{lem:union}, we can construct a valid menu $A'$ which is the NSR menu plus all points in $A \backslash p$. Note that by Lemma TODO, all NR menus include the NSR menu, and by the fact that $p$ is a high swap regret point, $p$ is not in the NSR menu. Therefore, $A' = A \backslash p$. $A'$ is just $A$ with one minimax point removed. By lemma~\ref{lem:FINDIT}, $A'$ dominates $A$. Therefore $A$ is not pareto-optimal. 



\subsubsection{Proof of Theorem~\ref{thm:mbnr_pd}}

\esh{Yet to be added}

==> notes.tex <==
Dec 7

Stronger version of our result (without any further tools) - Characterization of Pareto Optimal No-regret **polytopal** menus

Add corollaries at end of PO tools ---

1. NSR is PO.
2. The big NR polytope is pareto dominated.

Lemma 18 (lem:non-dominance) directly gives a proof of Pareto Domination of MW -- in that it gives us an optimizer payoff where NSR + all non min value ext points of MW does strictly better than MW. Note that this construction still needs $M_{MW}$ to be a polytope; since these operations could end up making the menus identical.


Lemma 4 (new numbering) --- Best response Learner value at limit = Limit of best respone learner values -- Can we use this to simplify some proofs in the MW = polytope section?

Adding some discussion because of the new NSR algorithms to the introduction -- these are fundamentally different algorithms (Natalie's proof via monotonicity - true for the Costis et al paper, but experimentally not true for BM); but are strategically equivalent in the limit

Universal Games - What if the learner no longer knows anything about the game at the start - neither their payoffs or even anything about the optimizer, such as the number of actions (the likes of MW, BM still make sense in this framework). The optimizer just generates losses for the actions of the learner in each round; we'd have to come up with a payoff model for the optimizer, but the hope is that the results about NSR and MW are corollaries in this setup


Dec 12

Distinct point comparing two menus, implies maximizing direction strictly better than everything in both menus? Should we go back and find a similar lemma we proved - check whether it is true only for polytopes?

Dec 20

Something to keep in mind : The algorithm that we use to show that MW is Pareto Dominated only makes sense in the world where the learner knows their payofffs upfront. It is not obvious that MW is Pareto dominated in this world, but the proof that NSR is PO still holds; and so does the revelation result. 

We should add a section about that.

Jan 4

1. Universal game 

2. Canonical Asymptotic NSR algorithm; like FTL for NR



Jan 19 (Things to discuss):

1. Definition of PO

2. New model with multiple agents -- the proofs generalize

3. Negative regret points both inside and outside NR? Natalie has examples for both



Changes to be made to figures:

1. Add labels for the hard ans soft boundaries

2. Shorten the Y-Axis

3. Transform the entire example trajectory into one spending little time outside the soft boundaries

4. Figures in MB = polytope proof, should the boundaries be redrawn to reflect the leader regions in the optimizer marginal space?





==> old/ParetoDominated.tex <==
% TODO: merge this into the pareto-optimal menus section

\section{Pareto-Dominated Algorithms}
\begin{definition}[$L^{+}$ and $L^{-}$]
For some set of learner payoffs $u_{L}$, we define $L^{+}$ as the highest payoff possible for the learner, and we define $L^{-}$ as lowest payoff for the learner. Formally, 
$$L^{+} = \textit{max}_{(i,j) \in [m][n]}(u_{L}(i,j))$$
$$L^{-} = \textit{min}_{(i,j) \in [m][n]}(u_{L}(i,j))$$
\end{definition}
 

\begin{lemma}
Any learning algorithm $\mathcal{A}_{T}$ that excludes $L^{+}$ from its menu for a constant-measure set of learner payoffs is pareto-dominated. 
\end{lemma}
\begin{proof}
We will prove this by showing a learning algorithm $\mathcal{A}^{*}_{T}$ which pareto-dominates $\mathcal{A}_{T}$. Let $(i^{*}, j^{*})$ be a move pair such that $u_{L}(i^{*},j^{*}) = L^{+}$. Now let $\mathcal{A}^{*}_{T}$ be defined as follows: play $i^*$ as long as the optimizer plays $j^*$. If the optimizer first deviates from $j^*$ at round $t$, begin playing $\mathcal{A}_{T}$ from a memoryless state (that is, as if round $t+1$ is the very first round of interaction), and play this algorithm for the remainder of the game. 

First, we will prove that $\mathcal{A}^{*}_{T}$ always performs at least as well as $\mathcal{A}_{T}$. Consider a game where the optimizer deviates at round $t$. Then the payoff of the learner is 
$$t \cdot L^{+} + (T-t) $$

\end{proof}


\begin{lemma}
Any learning algorithm $\mathcal{A}_{T}$ that includes $L^{-}$ in its menu for a constant-measure set of learning payoffs is pareto-dominated. 
\end{lemma}
\begin{proof}
\end{proof}


\section{The search for pareto-domination}

\begin{lemma}
No constant algorithm is pareto-dominated by any no-regret algorithm with regret $o(T)$.
\end{lemma}
\begin{proof}

We will first prove this claim for a particular constant algorithm. Let $C_{1}$ be the algorithm that always plays the learner's first move for every round of the game. We will show a game where $C_{1}$ outperforms any no-regret algorithm by a constant factor. Consider the following game $G$, with the learner playing the rows and the optimizer playing the columns. Call the learner's first move $A$ and their second move $B$, and call the optimizer's first move $X$ and their second move $Y$: 
 
 \[
\begin{bmatrix}
 (4,2) & (2,1.5)\\
 (5,2) & (3,3) 
\end{bmatrix}
\]

Consider if the learner plays $C_{1}$. Then the best response of the optimizer is to always play $X$, which gets the learner a payoff of $4T$. 

Now, consider any no-regret algorithm the learner can commit to. Note that $B$ strongly dominates $A$. Thus, every time the learner plays $A$ instead of $B$, they will experience regret. Intuitively, any no regret algorithm will be forced to play $B$ most of the time, and thus the optimizer will play $Y$ most of the time, leading to a payoff close to $3T$ for the learner. 

We will now formalize this. Any learner algorithm in this game $G$ induces a best response by the optimizer (tiebreaking in favor of the learner's payoff), and consequently a distribution over transcripts of action pairs. Let us write $p_{AX}$ as the expected fraction of the time that the action pair $(A,X)$ is played over the $T$ rounds, over the distribution of transcripts. Define $p_{AY}$, $p_{BX}$ and $p_{BY}$ similarly. 

If the leader commits to any no-regret algorithm, they must play $A$ an $o(T)$ fraction of the time in expectation. Thus, for any no-regret algorithm and any response by the follower, we have that $T(p_{AX} + p_{AY}) \leq o(T)$. We will choose $T$ sufficiently large s.t. the regret term is $\leq \frac{1}{64}T$. Thus, we have $$p_{AX} + p_{AY} \leq\frac{1}{64}$$

Note that against this no regret strategy, the optimizer could choose to just play $Y$. If they did this, $p_{AX} = 0$, $p_{BX} = 0$, and the optimizer's payoff would be equal to 
$$1.5 \cdot p_{AY} + 3 \cdot p_{BY}$$
$$= 1.5 \cdot p_{AY} + 3 \cdot (1 - p_{AY})$$
$$\geq 3 \cdot (1 - p_{AY})$$
$$\geq 3 \cdot \frac{63}{64}$$

Thus, whatever the best response for the optimizer is to this no regret algorithm, the optimizer can always get at least $ 3 \cdot \frac{63}{64}$. We will use this fact to upper bound the payoff of the learner. We have, for a no-regret learner and a best-responding optimizer:

$$2p_{AX} + 1.5p_{AY} + 2p_{BX} + 3p_{BY} \geq 3 \cdot \frac{63}{64}$$

Note that, from above, $p_{AX} + p_{AY} \leq \frac{1}{64}$, so $2p_{AX} + 1.5p_{AY} \leq \frac{2}{64}$. So we have that

$$ 2p_{BX} + 3p_{BY} \geq 3 \cdot \frac{63}{64} - \frac{2}{64} \geq 2.9$$

Now, note that $p_{BX} + p_{BY} \leq 1$, so we have that $$3p_{BX} + 3p_{BY} - 0.1 \leq 2.9$$

Combining these expressions, we get that 

$$2p_{BX} + 3p_{BY} \geq 3p_{BX} + 3p_{BY} - 0.1$$
Simplifying:
$$0.1  \geq p_{BX}$$

We also have that $p_{AX} \leq \frac{1}{64}$. So, the payoff of the learner when they play any no regret algorithm is at most
$$T(0.1 \cdot 5 + \frac{1}{64} \cdot 4 + (1 - 0.1 - \frac{1}{64})3) \leq 3.3T$$

This is $\Omega(T)$ worst than their payoff when playing $C_{1}$.


We have shown a game for which $C_{1}$ outperforms any no-regret algorithm. Now consider any constant algorithm playing the $i$th action, which might be played on a game with much more than $2$ actions for the learner. Call this algorithm $C_{i}$. Select some $j$ s.t. $1 \leq j \leq n$, $j \neq i$. Consider the game matrix $G_{i}$ for which $G_{i}[i][1] = (4,2)$, $G_{1}[i][2] = (2,1.5)$, $G_{i}[j][1] = (5,2)$, and $G_{1}[j][2] = (3,3)$. In other words, embed the first row of $G$ in the first two columns of the $i$th row of $G_{i}$, and the second row of $G$ in the first two columns of some other row $G_{j}$. Let all other entries of $G_{i}$ be $-C$ for some very large constant $C$, for both players. Note that in this game, $C_{i}$ will still attain payoff $4T$. Furthermore, any no regret algorithm will still have that $p_{AX} + p_{AY} \leq \frac{1}{64}$ for some $T$, 

nat: this generalization is sort of annoying to write out, I'll come back to it. It's definitely true.


\end{proof}


==> old/app_old_mw_is_equal_to_mb.tex <==
\subsection{Proof of Theorem~\ref{thm:sbm=mb}/Theorem~\ref{thm:sbm=mb_generalized}}
\label{app:sbm=mb}


%Before we begin our proof, we will first observe some structural properties about mean-based algorithms. Unlike the no-regret property, which is an aggregate constraint on the final distribution over move pairs, the mean-based property provides constraints on a round-by-round basis. Even in the relatively simple game $\mathcal{G}$, there exist points with the no-regret property which are not achievable by any mean-based algorithm




%\esh{Might be useful to keep in mind that the leader is never tied between A and C}

\esh{The proof works in its current form, but some annoying parts can be removed by cutting out the middleman $\intersectionmb$ - To be done}


Recall that $\A$ is $\gamma$-mean based with $\gamma(t) = t^{-\gamma}$ with $\gamma \in (0,1)$. Let $\intersectionmb$ denote the intersection of the menu of all mean-based algorithms. Lemma~\ref{lem:sub-mean-based} tells us that $\MB \subseteq \intersectionmb$. Tautoligcally, we also have $\intersectionmb \subseteq \M(\A)$ implying that $\M(\A) \subseteq \MB$. 
%For this proof, we use the alternative characterization of $\MB$ derived from Lemma~\ref{lem:sub-mean-based}, which shows that $\MB$ is a subset of the asymptotic menu of every mean-based algorithm, and hence a subset of the menu of all strictly mean-based algorithms.
Thus, we only need to show that the menu $\M(\A)$ of a given strictly mean-based algorithm is contained in $\MB$ to complete the proof of the lemma. Most of our time in this section goes into proving that $\M(\A) \subseteq \intersectionmb$ and we then show how to extend the same machinery for proving $\M(\A) \subseteq \MB$.

%Let $\A$ be $\gamma$-mean based.


We do this point by point in the asymptotic menu $\M$. As our proof sketch indicated, we compare the finite time menus of $\A$ and those of every mean-based algorithm. For each point $P$ in $\M$, there is a a sequence of points $P_1, P_2 \cdots $ in the finite time menus that converge to $P$. Fix any function $\kappa(T) = T^{-\kappa}$ for some $\kappa \in (0,1)$. For each point $P_T \in \M(\A)_T$ where $\M(\A)_T$ is the finite time menu of algorithm $\A$ for time horizon $T$ and for any arbitrary $\kappa$-mean based algorithm $\B$, there is a point $Q_T \in \M(\B)_T$ where $\M(\B)_T$ is the finite time menu of algorithm $\A$ for time horizon $T$ such that $d(P_T, Q_T) \le d_T$ with $\lim_{T \rightarrow \infty} d_T = 0$. In other words, we show that $P$ is present in the asymptotic menu of every mean-based algorithm and hence present in $\intersectionmb$. A subtlety here is that not all sublinear functions are of the form $\kappa(t) = t^{-\kappa}$ for some $\kappa \in (0,1)$, for eg: $\kappa(t) = \frac{
\log t
}{t}$ and therefore one might ask if our proof truly covers all possible mean based algorithms. For ease of presenting, we demonstrate the proof for such sublinear functions and then discuss how to generalize to all mean-based algorithms.

%We partially resolve this question using the following lemma:




For ease of writing, we introduce $\beta := max(\regret, 1-\gamma, 1- \kappa)$. There exists a positive constant $K$ such that the regret of both algorithms is upper bounded by $K T^\beta$. For ease of writing, we consider $K=1$, although our proof will work for any constant $K>0$.

%\esh{One more little thing to sew up when generalizing the proof to all mean-based algos/ sublinear functions}

The rest of the proof focuses mostly on proving the existence of $Q_T$ given $P_T$. %Recall that a CSP is in the menu of an algorithm if and only if there exists an ordered sequence of optimizer moves combined with the algorithm's responses, that induces this point. 
Without loss of generality, we restrict our attention to the simpler case where $P_T$ is an extreme point of the menu $\M(\A)_T$; and find a corresponding $Q_T$. The same idea can be extended to arbitrary menu points by rewriting $P_T$ as a convex combination of $mn+1$ extreme points (invoking Caratheodory's theorem).


%~\esh{Elephant in the room (only affects writing, not the proof itself): We care about optimizer sequences, which contain all extreme points of the menu, might have other points, but do not necessarily contain the entire menu with convex closure}


We introduce some notation to aid with our proofs, and formalize the notions of boundaries and trajectories. We track the (partial) state of learning algorithms by measuring the cumulative payoffs of the three actions $A,B,C$ after $t-1$ moves, which we denote by $\sigma^A_t, \sigma^B_t, \sigma^C_t$. %Since many of the algorithms we discuss, such as Multiplicative Weights and FTPL only care about the relative differences in the payoffs,
Since strictly mean-based algorithms only care about the relative differences in the payoffs of the actions,  we track $u_t := \sigma^A_t - \sigma^C_t$ and $v_t := \sigma^B_t - \sigma^C_t$, and refer to $(u_t,v_t) \in \mathbb{R}^2$ as the state of the learner. The move $x_t$ of the optimizer takes the learner's state from $(u_t,v_t)$ to $(u_{t+1},v_{t+1})$.
Recall that a CSP is an extreme point in the menu of an algorithm only if there exists an ordered sequence of optimizer moves combined with the algorithm's responses, that induces this point. Thus, let $P_T$ be generated by a sequence of optimizer actions $x_1,x_2 \cdots x_T$, in conjunction with the responses of the stictly mean-based algorithm $\A$.
%Recalling that each point $P$ in the menu corresponds to a sequence of optimizer actions $x_1,x_2 \cdots x_T$, 
Consider the sequence of learner states induced by this optimizer sequence.
We refer to the curve generated by joining consecutive states with line segments as the trajectory associated with the point $P_T$. The part of the trajectory associated with a contiguous subsequence of time steps is referred to a sub-trajectory. It is useful to keep in mind that the trajectory is entirely a function of the optimizer's actions and the learner's payoff function, and that different learner algorithm can potentially induce significantly different CSPs for the same trajectory.
%\esh{Define hard and soft boundaries}





We divide our state space $\mathbb{R}^2$ into multiple zones, based on the historical leader action and the corresponding advantage in these zones. These zones are demarcated by the following lines-

\begin{itemize}
    \item $H_{AB}$ is the set of all points $(u,v)$ where $u=v$ and $u,v \ge 0$.
    \item $H_{BC}$ is the set of all points $(u,v)$ where $v=0$ and $u<0$.
    \item $H_{AC}$ is the set of all points $(u,v)$ where $u=0$ and $v<0$.
    \item $S_{AB}$ is the set of all points $(u,v)$ where $v-u =T^\beta$ and $u,v \ge 0$.
    \item $S_{BC}$ is the set of all points $(u,v)$ where $v = T^\beta$ and $u<0$.
    
    
\end{itemize}


We refer to $H_{AB},H_{BC}, H_{AC}$ as the ``hard" boundaries separating the three actions, and refer to $S_{AB}, S_{BC}$ as the ``soft" boundaries. %The soft boundaries intuitively correspond to the $\gamma(t)$
 %term that appears in the mean-based property of $\A$.
 The separation of $T^\beta$ between the hard and soft boudnaries is interpreted an upper bound on the regret of algorithm $\A$ and the separation in cumulative payoff corresponding to the most stringent mean-based condition among the algorithms that we analyze.



We say that the learner has a ``clear" leader action if the action with the largest cumulative payoff has an advantage of at least $T^\beta$ over the other actions. In other words, at state $(u,v)$; $A$ is a clear leader when $u > T^\beta$ and $u-v > T^\beta$, $B$ is a clear leader when $v > T^\beta$ and $v-u > T^\beta$ and $C$ is a clear leader when $u <- T^\beta$ and $v < - T^\beta$. Note that a $\gamma$-mean based learner (recall that $\gamma(t) = t^{-\gamma}$) plays a clear leader at round $t$ with probability at least $1- t^{-\gamma}$ and plays the other actions with probability at most $t^{-\gamma}$. %In terms of previous notation, the notion of a clear leader is equivalent to a $\gamma$-unique leader.


\esh{Should we have these segments end on exactly the boundaries and explain the off by one move errors separately? - Let's roll with this for now}

 Consider the original point $P$ that we begin with. For $t_1 < t_2$, we call the part of a trajectory from $(u_{t_1},v_{t_1})$ to $(u_{t_2},v_{t_2})$a segment. We break up its trajectory into the following segments - 

 \begin{itemize}
     \item (I) An initial segment starting at $(0,0)$ and continuing until the first point where either $S_{AB}$ or $S_{BC}$ is crossed.
     \item (NC1) A maximal segment that starts within a move of crossing $S_{AB}$ and returns to a point within a move of $S_{AB}$ without ever crossing $S_{BC}$.
     \item (NC2)  A maximal segment that starts within a move of crossing $S_{BC}$ and returns to a point within a move of $S_{BC}$ without ever crossing $S_{AB}$.
     \item (C1)
     A minimal segment that starts within a move of crossing $S_{AB}$ and crosses $S_{BC}$ with its last line segment.
     \item (C2)
     A segment that starts within a move of crossing $S_{BC}$ and crosses $S_{AB}$ with its last line segment.
     \item (F) The final segment is broken up into a maximal C1 or C2 segment followed by a segment starting at one of the soft boundaries and staying in the zone with a unique clear leader. 
 \end{itemize}



 It is easy to see that this decomposition is unique and can be constructed directly by splitting a trajectory into an initial segment (I) followed by alternating non-crossing (NC) and crossing (C) segments and finishing with a final (F) segment. The alternating nature of non-crossing and crossing segments implies that the number of non-crossing segments is at most the number of crossing segments plus 1. 



 Recall that our algorithm of interest $\A$ has a regret upper (and lower) bound of $O(T^\regret)$. 

~\esh{Add image for trajectory}
%Consider the following graph which tracks the total payoff over all previous rounds of moves $A$, $B$ and $C$ in two dimensions, with the vertical axis showing the difference in payoff between $A$ and $B$ and the horizontal axis showing the difference in payoff between $B$ and $C$. [actually add image]


%Given some particular $\gamma$-mean-based algorithm $A$ and some sequence $S$, we can visualize the trajectory of play from round to round, where the trajectory in a given round is determined by the play of the optimizer in that round. We will also define regions of width $\gamma$ around the boundaries. 

 
%~\esh{We have a mismatch here between $\gamma$ and $\boundary$ (See macros) - what's the best fix? }

Whenever a trajectory is outside of a boundary region, i.e., in the clear leader zone, any mean-based algorithm that is $O(t^{-\kappa} + t^{-\gamma})
$-mean based must behave similarly to every other such mean-based algorithm , and play the same move with probability that it is almost $1$. Thus, any trajectory which spends a sublinear fraction of the time within the defined boundary region will induce menu points that are identical upto sublinear shifts for all $\gamma$-mean based algorithms, as long as $\gamma$ is also sublinear.





%Let us consider the intersection of all mean-based menus, and call it MB. Note that, by definition, MB is a subset of any particular mean-based no-regret menu. Furthermore, by the logic above, every point reached by any particular mean based algorithm by a trajectory which spends a sublinear amount of time within the boundary regions is also a point in MB (in the limit). 

%Therefore, to prove that any mean-based no-regret algorithm has a limit menu equal to MB, we must simply show that, for any time horizon $T$ and for any trajectory inducing some menu point $p$, there is another trajectory which spends sublinear time near the boundary and induces some menu point that is sub-constant close to $p$. %In other words,  we take every single point in the menu of our learning algorithm of interest, and construct an alternative optimizer action sequence that, when employed against an arbitrary mean-based no-regret algorithm, induces a point that is asymptotically equivalent to the original point.

We show how to transform the trajectory corresponding to point $P_T$
into another trajectory which spends only sublinear time within the soft boundaries and induces, in concert with algorithm $\A$, some CSP that is sub-constant close to $P_T$. Once we have such a transformation, we observe that every mean-based algorithm in the subclass that we consider induces a similar CSP against this trajectory (also sub-constant close). Therefore, we show the existence of the desired CSP $Q_T$ in every  $O(t^{-\kappa} + t^{-\gamma})
$-mean based algorithm.

We outline this transformation below, through a sequence of lemmas that prove some properties about this class of games and give procedures to transform the different types of segments in our target trajectory. 





%\begin{itemize}
%    \item The trajectory will never cross the boundary region between $A$ and $C$. In other words, there is no distribution over $X$ and $Y$ such that $A$ and $C$ are jointly optimal.
%    \item The trajectory is always moving away from the origin.
%\end{itemize}

%We will also make two important observations about how a mean-based, no-regret algorithm behaves on this trajectory:

%\begin{itemize}
%    \item 
 %   \item When inside of some boundary region, any no-regret algorithms must behave similarly to every other no-regret algorithm. This is less straightforward, but we will prove this.
%\end{itemize}

%define some constraints on the induced move pair distribution by constraining what $A$ can play at each round. 



%In order to understand how this guarantee translates to a constraint on the move pair distribution, we will 




Based on the learner utilities, we observe that any single move of the optimizer shifts the state of the learner by some constant distance (in say, the $\ell_1$ norm).
\begin{observation}
\label{obs:shifts}
    Starting at state $(u,v)$ and playing optimizer distribution $\alpha(X)$ for one step changes the state to $(u+\xi_1, v +\xi_2)$ with
    \begin{itemize}
        \item  $\xi_1 = 1/2 \pm 2\varepsilon$ and $\xi_2 = 1/3 \pm 2\varepsilon$ when $\alpha(X) = 1$.
        \item  $\xi_1 = -1/2 \pm2 \varepsilon$ and $\xi_2 = -1/6 \pm 2\varepsilon$ when $\alpha(X) = 0$ .
    \end{itemize}
    where $\xi = a \pm b$ is equivalent to stating $\xi \in [a-b,a+b]$.
\end{observation}


Next, we observe that the optimizer's action space in the stage game can be partitioned into contiguous intervals corresponding to which action of the learner is a best response to it. We note that the breakpoints are close to $1/3$ and $2/3$, where we parametrize the optimizer action by the probability with which action $X$ is played.
\begin{observation}
\label{obs:br_intervals}
    For an optimizer distribution $\alpha(X)$; there are numbers $q = 1/3 \pm O(\varepsilon)$ and $p = 2/3 \pm O(\varepsilon)$ such that :
    \begin{itemize}
        \item If $\alpha(X) \in [0,p)$, $C$ is a unique best response.
        \item If $\alpha(X) \in (p,q)$, $B$ is a unique best response.
        \item If $\alpha(X) \in (q,1]$, $A$ is a unique best response.
    \end{itemize}
\end{observation}

Using these observations, we show an important result, that says that the state of the algorithm drifts away from the origin, in the $\ell_1$ distance, by $\theta(t)$ after $t$ time steps. 

\begin{lemma}
There exists a constants $C_1, C_2 > 0$ such that every sub-trajectory of length $L$ corresponds to somewhere between $C_1 \cdot L$ and $C_2 \cdot L$ moves, and a constant $B > 0$ such that after $t$ time steps, the trajectory is at least $B \cdot t$-far from the origin in the $\ell_1$ distance. \label{lem:constant_dirft}
\end{lemma}

\begin{proof}
Each time step moves the state only by a constant amount in the $\ell_1$ metric (follows directly from Observation~\ref{obs:shifts}). Thus, a segment of some length $L$ must correspond to a contiguous subsequence of at least $C_1 \cdot L$ time steps for some constant $C_1>0$. Showing the second half of the lemma statement will imply a similar upper bound on the number of time steps. To do so, we look at the offsets to the state generated by the two actions $X$ and $Y$, which are $V_1 =  (1/2 \pm 2\varepsilon, 1/3 \pm 2\varepsilon)$ and $V_2 = (-1/2 \pm 2\varepsilon, -1/6 \pm 2\varepsilon)$. The average offset caused by the action of the optimizer over any number of time steps must therefore be some convex combination of $V_1$ and $V_2$ (we use linearity to rewrite the average offset of the actions as the offset generated by the historical average optimizer action). Ignoring the $\varepsilon$ terms for the moment, the line between the points $V_1$ and $V_2$ is $y = x/2 - 1/12$. The $\ell_2$ distance from the origin $(0,0)$ to this line is $\frac{1}{6 \sqrt{5}}$, implying that every point on the line is at least  $\frac{1}{6 \sqrt{10}}$ far from the origin. With the $\epsilon$ terms included, it is easy to see that this statement is still true for the distance $\frac{1}{6 \sqrt{10}} \pm O(\varepsilon)$. Thus, after $T$ time steps, the state has $\ell_1$ distance at least $\frac{T}{24}$ from the origin, completing the proof.
    %\esh{editing}
\end{proof}

The above lemma implies a bound on the number of non-crossing segments in any trajectory.



\begin{lemma}
\label{lemma:bound_crossing}
After $\phi$ time steps, there can only be $O\left(\frac{T}{\phi}\right)$ different non-crossing segments.
\end{lemma}

\begin{proof}
    An upper bound the number of crossing segments after $\phi$ time steps implies the same asymptotic upper bound for the number of non-crossing segments. %\esh{Slightly dodgy but does not matter I think, perhaps we should just drop this sentence?} 
    We assume WLOG that $\phi > T^\beta$ since the first crossing segment can only appear after $\Omega(T^\beta)$ time steps (which is the minimum length of the initial segment). Using Lemma~\ref{lem:constant_dirft}, we see that any crossing segment is the largest side of an obtuse angled triangle whose two smallest sides have length $\Omega(\phi)$. Thus, each non-crossing segment has length $\Omega(\phi)$, and must consequently correspond to $\Omega(\phi)$ time steps (since each time step's line segment has constant length). This directly implies the desired result.
\end{proof}



\begin{comment}

We prove the asymptotic menu of some algorithm $\A$ is equal to $MB$ if $\A$ fulfills the following conditions:

\begin{itemize}
\item[1] $\A$ is $T^{\gamma}$-mean based 
\item[2] $\A$ has regret upper bounded by $O(T^{\regret})$ on any prefix of play.
\item[3] $\A$ has regret lower bounded by $-O(T^{\regret})$ on any prefix of play.
\item[4] The moves played by $\A$ each round are a function only of the cumulative payoff distribution of the actions. 
\item[5] For a fixed optimizer sequence corresponding to a segment of a trajectory that stays entirely in the region where one of three actions (WLOG A) is $T^\beta$-far from being the leader, the (normalized) CSP of this segment induced by playing against algorithm $\A$ for three actions  is sub-constant close to the CSP induced by play against the same algorithm $\A$ but with action A excluded from consideration.
\end{itemize}


    
\begin{lemma}
    The above assumptions are satisfied by the variant of MW/FTRL that have a fixed learning rate, with $\regret = \boundary = 0.5$.
\end{lemma}

\begin{proof}
We first prove the first four assumptions are true for both:

\begin{itemize}
\item ($\A$ is $T^{\gamma}$-mean based.) CITE shows this is true for $\gamma = 0.5$ for MW/FTRL with a fixed learning rate.
\item ($\A$ has regret upper bounded by $O(T^{\regret})$ on any prefix of play.) It is well-known that this is the case for any MW/FTRL algorithm \nat{cite I guess?}
\item ($\A$ has regret lower bounded by $-O(T^{\regret})$ on any prefix of play.) Cite those two papers.
\item (The moves played by $\A$ each round are a function only of the cumulative payoff distribution of the actions.) This is true by the definitions of the two algorithms, as long as they have a fixed learning rate.
\end{itemize}

Now, we tackle assumption 5. Consider any optimizer sequence in a three-action game which stays entirely in a region where action $A$ is $T^\beta$-far from being the leader. Then, each round, multiplicative weights will play $A$ with probability equal to 

For a fixed optimizer sequence corresponding to a segment of a trajectory that stays entirely in the region where one of three actions (WLOG A) is $T^\beta$-far from being the leader, the (normalized) CSP of this segment induced by playing against algorithm $\A$ for three actions  is sub-constant close to the CSP induced by play against the same algorithm $\A$ but with action A excluded from consideration.


\end{proof}


\end{comment}

    

The critical part of our proof is a method to transform non-crossing segments into a segment with identical start and end points, but one that only spends sublinear ($O(T^\beta)$) number of time steps within the soft boundaries.



\begin{lemma}
\label{lem:nc_replacement}
Every non-crossing segment can be replaced with a trajectory beginning and ending in the same place, running for the same number of time steps, inducing a CSP which differs by $O(T^{\beta})$, and spending $O(T^\beta)$ time in the boundary.
\end{lemma}

\begin{proof}

%\esh{Fixing : sums in exponents}
We will prove this for the soft boundary $S_{AB}$. A similar proof works for $S_{BC}$.

Call the segment of play by the optimizer starting at $S_{AB}$ and ending somewhere within the soft boundary of $BC$ $s = x_{t_1:t_2}$. It has a resulting CSP of $c$ (the average joint distribution over action pairs measured over this sequence). To circumvent comparing the length of the segment with the total length, we unnormalize the CSP by multiplying it with $T$ for the sake of this proof.



Instead of analyzing algorithm $\A$'s induced CSP $c$ on the trajectory; we instead analyze the (unnormalized) CSP $c'$ generated by the action of $\A_{2}$, a learning algorithm which is equivalent to $\A$ except that it only considers actions $A$ and $B$, on the same trajectory. As a consequence of the properties of strictly mean-based algorithms; the CSPs $c$ and $c'$ are sublinearly close, i.e., $||c-c'||_1 \le O(T^{1-\gamma}) = O(T^\beta)$.




%Note that, because of assumption \ref{}$???$, $c$ is within $T^{\beta}$ of the CSP of $s$ against $\A_{2}$, a learning algorithm which is equivalent to $\A$ except that it only considers actions $A$ and $B$. Call this CSP $c'$. 



Now, we will describe a new trajectory that approximates $c'$. Recall that $x_t$ is the distribution played by the optimizer at round $t$. Let $(\alpha_A^t,\alpha_B^t)$ be the distribution played by the learning algorithm $\A_2$ at round $t$. Define $D_A := \frac{1}{\alpha_A} \sum_{t=t_1}^{t_2} \alpha_A^t x_t$  and $D_B := \frac{1}{\alpha_B} \sum_{t=t_1}^{t_2} \alpha_B^t x_t$ where $\alpha_A := \sum_{t=t_1}^{t_2} \alpha_A^t$ and $\alpha_B := \sum_{t=t_1}^{t_2} \alpha_B^t$. In other words, $D_{A}$ and $D_{B}$ are the average distributions of the optimizer conditioned upon the learner playing $A$ and $B$ respectively, while $\alpha_{A}$ and $\alpha_{B}$ be the sum of the probabilities over all the rounds in this segment that the optimizer plays $A$ and $B$ respectively. 

Since the segment $s$ starts and ends at the soft boundary $S_{AB}$, we know that $A$ and $B$ are both within a cumulative value of $O(T^\beta)$ to a best response to the distribution $d' = \frac{\alpha_{A}D_{A}+\alpha_{B}D_{B}}{\alpha_{B} +\alpha_{B}}$, i.e the average distribution of the optimizer over the segment of interest, played $\alpha_A+ \alpha_B$ times.

%\nat{This is clear from the start and end point of the trajectory but have to write the two lines of math that prove it.}



We argue that algorithm $\A_2$ has an upper and lower bound on regret of $O(T^\beta)$ and $-O(T^\beta)$ respectively in this segment. To see this, we imagine a prefix to this segment that starts at the hard boundary $H_{AB}$ and moves to the soft boundary $S_{AB}$ by playing $K'T^\beta$ steps of $Y$ for some constant $K'$~\footnote{We employ this argument since regret upper bounds are typically only guarantees for starting at time $t=0$.}. Now, since this extended sequence begins at the hard boundary, it is as if we started running $\A_2$ at $t=0$ at the start of this sequence. Thus, we get the regret guaranteed to be in the interval $[-O(T^\beta), O(T^\beta)]$ for the extended sequence (from the properties of strictly mean-based algorithms), and observe that the regret for the ``true" segment is therefore guaranteed to be in $[- H T^\beta, H T^\beta]$ for some constant $H> 0$.


First, we observe that the no-regret property with two actions implies no-swap regret. Quantitatively, that gives us:

\[\alpha_B (\mu_{\mathcal{L}}(D_B,A) - \mu_{\mathcal{L}}(D_B,B)) \le H T^\beta \qquad \text{(based on regret bounds against $A$)}\]
\[\alpha_A (\mu_{\mathcal{L}}(D_B,B) - \mu_{\mathcal{L}}(D_B,A)) \le -H T^\beta  \qquad \text{(based on regret bounds against $B$)}\]


We show the stronger property that $A$ and $B$ are both close to a best response to both $D_{A}$ and $D_{B}$ (the observation above only shows that $A$ is a near best response to $D_A$ and $B$ is a near best response to $D_B$). Assume for contradiction that $\alpha_A(\mu_{\mathcal{L}}(D_B,A) - \mu_{\mathcal{L}}(D_B,B)) > 2 H T^\beta$.
%We will prove that either $A$ and $B$ are both $T^{\regret}$-close to a best response to both $D_{A}$ and $D_{B}$, or that one of $\alpha_{A}$ and $\alpha_{B}$ is very small, in which case we can ignore it. To see this, assume for contradiction that $\alpha_{A} \geq T^{\beta}$, and $\mu_{\mathcal{L}}(D_{A},A) - \mu_{\mathcal{L}}(D_{A},B) > T^{\regret-1}$. Then, we write down the unnormalized payoff of the leader for this segment :
\begin{align*}
\mu_{\mathcal{L}}(c') & = \alpha_{A}\mu_{\mathcal{L}}(D_{A},A) + \alpha_{B}\mu_{\mathcal{L}}(D_{B},B) \\
& > \alpha_{A}\mu_{\mathcal{L}}(D_{A},B) + \alpha_{B}\mu_{\mathcal{L}}(D_{B},B) + 2H T^\beta \qquad \text{(by assumption)}\\
& = (\alpha_A+\alpha_B)\mu_{\mathcal{L}}(d',B) + 2H T^\beta \qquad \text{(using linearity of the payoffs)} \\
& \geq \max_{S \in \{A,B\}}(\alpha_A+\alpha_B)\mu_{\mathcal{L}}(d',s) - H T^{\beta} +  2HT^{\beta} \text{(by the fact that $B$ is close to a best response to $d'$)}\\  
\end{align*}

%\esh{Is there a problem here?}
%\nat{Add note that we can pretend this is a prefix because we are starting at the hard boundary}

%\esh{Add a multiplier of 2}

This is a contradiction for sufficiently large $T$, as $\A_{2}$ has an average regret lower bound of $-H T^\beta$. A similar argument can be made with $A$ and $B$ exchanged. Thus, we have :

\[\alpha_A(\mu_{\mathcal{L}}(D_B,A) - \mu_{\mathcal{L}}(D_B,B)) \le 2 H T^\beta\]
\[\alpha_B(\mu_{\mathcal{L}}(D_A,B) - \mu_{\mathcal{L}}(D_A,A)) \le 2 H T^\beta\]



These inequalities are key to constructing our transformation. We split our analysis into four cases, depending on whether or not actions $A$ and $B$ are both played for a significant amount of time in this segment.

%\esh{Maybe we don't need these cases}

We start by assuming that $\alpha_{A} \geq 8 K_1 T^{\beta}$, $\alpha_{B} \geq 8 K_2T^{\beta}$ for some positive constants $K_1$ and $K_2$ that we shortly define. This is the most important case in the analysis, and the other cases (where this assumption is not true) simply follow by exploiting sublinear differences in the construction.


The new sequence is as follows: from the hard boundary, play $X$ until $u_{t} - v_t = 3HT^{\beta}$. By Observation~\ref{obs:br_intervals}, this will take $K T^{\beta}$ rounds for some constant $K>0$. Then, play $D_{A}$ for $\alpha_{A} - 8K T^{\beta}$ rounds. Then, play $Y$ until $u_{t} - v_t = -3HT^{\beta}$. We claim that takes only $K_{2}T^{\beta}$ rounds for some constant $K_{2} > 0$ - this is so because the cumulative effect of playing $D_A$ for $\alpha_A$ rounds causes a difference of at most $2HT^\beta$ in the payoffs of actions $A$ and $B$ over these rounds. Therefore, at the time step $t$ at the end of playing $D_A$, $u_t - v_t \le 5HT^\beta$. Then, play $D_{B}$ for $\alpha_{B} - 8K_{2} T^{\beta}$ rounds.

Let $D_{A}(Y)$ be the fraction of the time that $Y$ is played in $D_{A}$, and define $D_{A}(X)$, $D_{B}(Y)$, and $D_{B}(X)$ accordingly. Then, let us consider the number obtained by adding up the probability of playing $X$ in all the rounds described so far. This number $n_X$ is upper bounded by $D_{A}(X)(\alpha_{A} - 8K T^{\beta}) + D_{B}(X)(\alpha_{B} - 8K_{2} T^{\beta}) + K T^{\beta}$.  Likewise, the number of times $n_Y$ we have played $y$ so far is upper bounded by $D_{A}(Y)(\alpha_{A} - 8K T^{\beta}) + D_{B}(Y)(\alpha_{B} - 8K_{2} T^{\beta}) + K_{2} T^{\beta}$.

To finish our sequence, we will play $X$ for $n'_X := d'(X) (\alpha_A + \alpha_B) - n_X$ times, which is lower bounded by  $d'(X) (\alpha_A + \alpha_B)- (D_{A}(X)(\alpha_{A} - 8K T^{\beta}) + D_{B}(X)(\alpha_{B} - 8K_{2} T^{\beta}) + K T^{\beta})$ and then play $y$ for $n'_Y:= d'(Y)(\alpha_A + \alpha_B) - n_Y$ rounds, which is lower bounded by  $d'(Y)(\alpha_A + \alpha_B) - (D_{A}(Y)(\alpha_{A} - 8K T^{\beta}) + D_{B}(Y)(\alpha_{B} - 8K_{2} T^{\beta}) + K_{2} T^{\beta})$ rounds. We show that this is a legal operation by proving that $n'_X, n'_Y \ge 0$. It suffices to show their lower bounds are non-negative.

Note that by the fact that $A$ and $B$ are near best responses for both $D_{A}$ and $D_B$ and using Observation~\ref{obs:br_intervals}, $D_{A}(X), D_B(X), D_A(Y), D_B(Y) > \frac{1}{4}$.
\begin{align*}
%& d'(X)(\alpha_{A} + \alpha_{B}) - (D_{A}(X)(\alpha_{A} - 8K T^{\beta}) + D_{B}(X)(\alpha_{B} - 8K_{2} T^{\beta}) + K T^{\beta}) \\
n'_X &= D_{A}(X)\alpha_{A} + D_{B}(X)\alpha_{B} - D_{A}(X)(\alpha_{A} - 8K T^{\beta}) - D_{B}(X)(\alpha_{B} - 8K_{2} T^{\beta}) - K T^{\beta} \\
& =  D_{A}(X)8K T^{\beta} + D_{B}(X)8K_{2} T^{\beta} - K T^{\beta}  \\
& \geq 2K T^{\beta} +2K_{2} T^{\beta} - K T^{\beta} \\
& = K T^{\beta} +2K_2 T^{\beta} > 0 \\
\end{align*}
A similar analysis for $Y$ show
\begin{align*}
%& d'(Y)(\alpha_{A} + \alpha_{B}) - (D_{A}(Y)(\alpha_{A} - 8K T^{\beta}) + D_{B}(Y)(\alpha_{B} - 8K_{2} T^{\beta}) + K_{2} T^{\beta}) \\
n'_Y & = D_{A}(Y)\alpha_{A} + D_{B}(Y)\alpha_{B} - D_{A}(Y)(\alpha_{A} - 8K T^{\beta}) - D_{B}(Y)(\alpha_{B} - 8K_{2} T^{\beta}) - K_{2} T^{\beta}  \\
& =  D_{A}(Y)8K T^{\beta} + D_{B}(Y)8K_{2} T^{\beta} + 8K_{2} - K_{2} T^{\beta}  \\
& \geq 2K T^{\beta} +2K_{2} T^{\beta} - K_{2} T^{\beta} \\
& = 2K T^{\beta} + K_{2} T^{\beta} > 0\\
\end{align*}


A similar analysis can also be used to upper bound $n'_X$ and $n'_Y$ by $8(K_1+K_2)T^\beta$.
%Note that summing together all the rounds together gives us $\alpha_{A} + \alpha_{B}$. 


%A fine grained inspection of the play in our transformed segment reveals that the marginal distribution of play of the learner is identical to that in the original segment, which implies that the segment ends at the same point as the original segment.

Since $n'_X, n'_Y \ge 0$, our construction is valid, and we have played $X$ and $Y$ the same total frequency across the rounds as compared to the original segment. Therefore the endpoint of the new segment will be exactly the same~\footnote{The state at the end of $t$ rounds only depends on the average marginal distribution of the optimizer and is invariant to reordering of the optimizer's play.} and the number of rounds will be as well. Further, we argue that the CSP of this segment is very close to the CSP of the original segment. In the new segment, because we have moved $3HT^{\beta}$ away from the hard boundary and because we can only move back by $2HT^{\beta}$ as we play $D_{A}$, the learner will play $A$ the whole time against this (except for a sublinear fraction of the rounds), since we are in the clear leader zone for action $A$~\footnote{Here, we critically use the fact that $T^\beta > t^\beta$ for all time steps $t$}. For the same reason, the learner plays $B$ against $D_{B}$ when we play it (except for a sublinear fraction of the rounds). The other drivers of change in the CSP is the $KT^\beta$ rounds of $\alpha_A$ that we do not play $D_A$ (similar for $D_B$), the $K_2 T^\beta$ rounds of playing $Y$ that are required to go from the region where $A$ is the clear leader to where $B$ is the clear leader and the $8(K_1+K_2)(T^\beta)$ rounds of play at the end to reach the same end point as the original segment. Even if all these changes go in the same direction, the net effect on the CSP is at most $O(T^{\beta})$ deviation in the 
$\ell_1$ distance (each round can only effect a change of $O(1)$), which is sublinear $O(T^\beta)$ (the constants do not depend on $T$ and are entirely determined by the learner values in the game).

Although we have assumed that $\alpha_{A} \geq 8 K_1 T^{\beta}$, $\alpha_{B} \geq 8 K_2T^{\beta}$, the same analysis can still be done if this assumption is not true. We simply do not play $D_A$/$D_B$ in the construction if the corresponding frequency $\alpha_A$/ $\alpha_B$ is very small. With minor modifications, the same guarantees can be achieved without this assumption.


\end{proof}


Armed with these tools, we focus now on generating $Q_T$ from $P_T$ for a finite time horizon $T$. The procedure starts by decomposing the trajectory of the point $P$ in the state space defined above into I,C1,C2,NC1,NC2 and F segments. Each segment is then replaced with another segment (by a suitable modification of the optimizer actions)  with the same start and end point so that the new trajectory has the property that only sublinear time is spent outside the regions with a clear leader. We maintain the invariant that the unnormalized CSP induced by this new sequence/ trajectory against algorithm $\A$ is only sublinearly different (i.e $o(T)$ distant in the $\ell_1$ metric) from $P_T$. However, since all MBNR algorithms in our comparison class behave identically, upto a sub-constant factor, in a zone with a clear leader, the (unnormalized) CSP $Q_T$ induced by this optimizer sequence against any of these MBNR algorithm is identical to $P_T$, upto sublinear shift. %For ease of analysis, we multiply the CSP by a factor of $T$ in this proof, and thus maintain the invariant that the CSP is shifted by a sublinear factor $o(T)$.

Dealing with the Crossing segments of the type C1 or C2 is the easiest part of the transformation - these segments already spend their entire duration  in a region with a single clear leader, so we can leave them untouched. To deal with non-crossing segments (C1/C2); we make use of Lemma~\ref{lem:nc_replacement} to replace them one by one with a segment that has the same start and end point, operates for eaxtly the same time duration and results in a trajectory that spends time at most $O(T^\beta)$ outside the clear leader region and generates a CSP shifted by only $O(T^\beta)$ from the starting trajectory's CSP. A concern with this sequence of transformations is that sufficiently large number of crossing segments can result in linear drift from the original CSP/ linear time spent outside the clear leader zone. To address this issue, we split the analysis into two parts. Set $\psi = (1+\beta)/2$ implying that $\psi \in (\beta,1)$. We split the time horizon $T$ into the first $T^\psi$ time steps and the remaining time steps. The play in the first part can only affect the CSP by $O(T^\psi)$, further the total time spent outside the clear leader zone in the first part is also upper bounded by $T^\kappa$. Using Lemma~\ref{lemma:bound_crossing}, there are at most $O(T^{1-\kappa})$ crossing segments in the second half. Therefore, the total drift (in $\ell_1$ distance) from the original CSP is upper bounded by $O(T^\psi +T^{1-\psi}) =   o(T)$. Similarly, in the time steps corresponding to the crossing segments, the final trajectory spend time at most $o(T)$ away from the boundary. 

A similar analysis can be done for the initial (I) and final (F) segment, by only replacing the non-crossing part of their trajectories using Lemma~\ref{lem:nc_replacement} and contributing an additional $o(T)$ drift away from the original CSP, and $o(T)$ additional time spent away from the clear leader zone. %To finish with exactly the same number of time steps, we simply truncate/ extend the trajectory by the required number of steps. Since this number is $o(T)$, the other properties remain true.




The final part of our proof is to extend our argument to all mean-based algorithms and not just $\kappa$-sublinear algorithms where $\kappa(t) = T^{-\kappa}$ for some constant $\kappa \in (0,1)$. We argue that a similar proof works where $T^\beta$ is instead replaced by $B(T) = \max \{ T^\alpha, T^{1-\gamma}, T \kappa(T)\}$ and $T^\psi$ is replaced by $\sqrt{T\cdot B(T)}$. Clearly, $B(T)$ is also a sublinear function of $T$, and hence, so is $\sqrt{T\cdot B(T)}$. To make sure the same proof works, we need the following two properties:

\begin{itemize}
    \item $\gamma(T)$ and $T \kappa(T)$ are monotone decreasing and increasing in $T$ respectively
    \item $\sum_{t=1}^T \gamma(t) = o(T)$.
\end{itemize}
 

We use the first property to claim that any action with a disadvantage of $B(T)$ is played with probability at most $\gamma(t)$; specifically we use $B(T) \ge T \cdot \kappa(T)$ and then use the inequality $\frac{T \cdot \kappa(T)}{t} \ge \kappa(t) $, i.e. the monotonicity property. The second property is used to show that we can ignore the effect (on the CSP) of actions which lag the leader by at least $\kappa(t)$ in average value, since their cumulative effect is sublinear.

While the second property  follows directly from the sub-constant property of $\gamma(t)$, the first property requires that $\kappa(t) = \omega(\frac{1}{t})$. To take care of functions that do not satisfy this property, we prove the following lemma.

\begin{lemma}
    Let $S_1$ and $S_2$ respectively denote the set of all $\gamma_1$-mean based and $\gamma_2$-mean based algorithms. If $\gamma_1(t) = o(\gamma_2(t))$, then $\cup_{\B \in S_1} \M(\B) \subseteq \cup_{\B \in S_2} \M(\B)$ 
\end{lemma}



\begin{proof}
    The proof of this lemma is based on the observation that every mean-based algorithm in the set $S_1$ can be rewritten as a mean-based algorithm in the set $S_2$, this follows directly from $\gamma_1(t) = o(\gamma_2(t))$, implying that algorithms in $S_2$ have a greater degree of freedom (for large enough $T$).
    \esh{Enough detail?}
\end{proof}

Since we know our proof works for $\kappa(t) = t^{-0.1}$ and all functions that are $O\left(\frac{1}{t}\right)$ are also asymptotically $o\left( t^{-0.1}\right)$; which means that we can safely ignore all such functions (and the associated set of mean-based algorithms) for proving $\M_{\A} \subseteq \intersectionmb$. \esh{Sanity check please}

In proving that every extreme point $P \in \M(\A)$ is contained in $\intersectionmb$; we came up with a sequence of trajectories $\tau_1, \tau_2 \cdots $ such that:

\begin{enumerate}
    \item Let $P'_T$ be the CSP induced by $\tau_T$ against $\A$; then $P'_T$ (unnormalized) is sublinearly close to $P$ and the sequence $\{P'_T\}$ converges to $P$.
    \item Each trajectory $\tau_T$ spends sublinear time within the soft boundaries. 
\end{enumerate}

Based on the trajectory $\tau_T$, we can construct a valid trajectory $\tau'_T$ in the continuous time formulation referred to in Section~\ref{sec:mb_algos_and_menus}~\esh{Might want to use different words to refer to the two kinds of trajectories}. We do this by taking the trajectory $\tau_T$, breaking it up whenever it crosses a hard boundary separating two learner actions, and replacing each segment by the time average action repeated for the length of the trajectory. We also attach the corresponding learner best response action to each segment of this trajectory to complete the triple. Since $\tau_T$ spends only sublinear time near the soft boundaries, it is easy to see that the CSP $P''_T := \Prof(\tau'_T)$ is sublinearly close to $P'_T$ and hence to $P_T$. Thus, we have a sequence of valid trajectories $\{\tau'_T\}$ whose images under the continuous function $\Prof$ are converging to $P$. Since $\MB$ is a closed and bounded set (by virtue of being a polytope, see Theorem~\ref{thm:mb_is_a_polytope}), the point $P$ is contained in $\MB$, completing the proof.




%\esh{editing}








%\esh{The proof is straightforward and can be added in when we're sure this helps; still wondering the best way to argue this covers all mean-based algorithms}

%\esh{Come back to this later - the intricacy here is for broad boundaries, such as $\frac{1}{\log t}$}

%\esh{Fix ideas -  use the geometric mean, and rewrite the above lemma for $t.\kappa(t)$ to be monotone increasing WLOG}








%Old stuff below, commented out

\begin{comment}
    

This is a contradiction for sufficiently large $T$, as $\A_{2}$ has an average regret lower bound of $-T^{\alpha-1}$.
%Next, assume for contradiction that $\alpha_{A} \geq T^{\beta}$ and $\mu_{\mathcal{L}}(D_{A},B) - \mu_{\mathcal{L}}(D_{A},A) > T^{\regret-1}$. Then, 

\begin{align*}
\mu_{\mathcal{L}}(c') & = \alpha_{A}\mu_{\mathcal{L}}(D_{A},A) + \alpha_{B}\mu_{\mathcal{L}}(D_{B},B) \\
& < \alpha_{A}\mu_{\mathcal{L}}(D_{A},B) + \alpha_{B}\mu_{\mathcal{L}}(D_{B},B) - \alpha_{A}T^{\regret-1} \\
& = \mu_{\mathcal{L}}(d',B) - \alpha_{A}T^{\regret-1} \\
& \leq \mu_{\mathcal{L}}(d',\textit{best fixed}) -  T^{\beta + \regret-1} + T^{\alpha-1}  \tag{By the fact that $B$ is close to a best response to $d'$}\\  
\end{align*}
This is also a contradiction for sufficiently large $T$, as $\A_{2}$ has a regret upper bound of $T^{\alpha-1}$.

Symmetric proofs to those above show contradictions for the case where $\alpha_{B} \geq T^{\beta}$, $\mu_{\mathcal{L}}(D_{B},B) - \mu_{\mathcal{L}}(D_{B},A) > T^{\regret}$, as well as the case where $\alpha_{B} \geq T^{\beta}$, $\mu_{\mathcal{L}}(D_{B},A) - \mu_{\mathcal{L}}(D_{B},B) > T^{\regret}$. 





\breakpointsign{Take care henceforth }


Now, we can analyze four cases: 
\begin{itemize}
\item Case 1: $\alpha_{A} \geq T^{\beta}$, $\alpha_{B} \geq T^{\beta}$. Then we have both $|\mu_{\mathcal{L}}(D_{A},A) - \mu_{\mathcal{L}}(D_{A},B)| \leq T^{\regret-1}$ and $|\mu_{\mathcal{L}}(D_{B},B) - \mu_{\mathcal{L}}(D_{B},A)| \leq T^{\regret-1}$. The new sequence we will construct is as follows: from the hard boundary, play $X$ until $u_{t} = 2T^{\beta}$. By Observation~\ref{obs:br_intervals}, this will take $K T^{\beta}$ rounds for some constant $K$. Then, play $D_{A}$ for $\alpha_{A} - 8K T^{\beta}$ rounds. Then, play $Y$ until $u_{t} = -2T^{\beta}$, which will take $K_{2}T^{\beta}$ rounds for some $K_{2}$%~\esh{ Explain with drift bound} 
-- this is because both $A$ and $B$ are within a $O(T^{\beta-1})$-additive best response to $D_A$, implying that at the state $(u,v)$ after playing $D_A$, $|u-v| = O(T^\beta)$, thus using Lemma~\ref{lem:constant_dirft}, we only need $I=O(T^\beta)$ to cross over into the $B$ clear leader region. Then play $D_{B}$ for $\alpha_{B} - 8K_{2} T^{\beta}$ rounds.

Let $D_{A}(Y)$ be the fraction of the time that $Y$ is played in $D_{A}$, and define $D_{A}(X)$, $D_{B}(Y)$, and $D_{B}(X)$ accordingly. 

Then, let us consider the number obtained by adding up the probability of playing $X$ in all the rounds described so far. This number $n_X$ is upper bounded by $D_{A}(X)(\alpha_{A} - 8K T^{\beta}) + D_{B}(X)(\alpha_{B} - 8K_{2} T^{\beta}) + K T^{\beta}$. 

Likewise, the number of times $n_Y$ we have played $y$ so far is upper bounded
$D_{A}(Y)(\alpha_{A} - 8K T^{\beta}) + D_{B}(Y)(\alpha_{B} - 8K_{2} T^{\beta}) + K_{2} T^{\beta}$.

To finish our sequence, we will play $X$ for $d'(X) (\alpha_A + \alpha_B) - n_X$ times, which is lower bounded by  $d'(X) (\alpha_A + \alpha_B)- (D_{A}(X)(\alpha_{A} - 8K T^{\beta}) + D_{B}(X)(\alpha_{B} - 8K_{2} T^{\beta}) + K T^{\beta})$ and then play $y$ for $d'(Y)(\alpha_A + \alpha_B) - n_Y$ rounds, which is lower bounded by  $d'(Y)(\alpha_A + \alpha_B) - (D_{A}(Y)(\alpha_{A} - 8K T^{\beta}) + D_{B}(Y)(\alpha_{B} - 8K_{2} T^{\beta}) + K_{2} T^{\beta})$ rounds. Note that summing together all the rounds together gives us $\alpha_{A} + \alpha_{B}$. 


We must prove that these numbers are both non-negative, which we do by showing their lower bounds are non-negative.

Note that by the fact that $A$ and $B$ are near best responses for both $D_{A}$ and $D_B$ and using Observation~\label{obs:br_intervals},  $D_{A}(X), D_B(X), D_A(Y), D_B(Y) > \frac{1}{4}$.

\begin{align*}
& d'(X)(\alpha_{A} + \alpha_{B}) - (D_{A}(X)(\alpha_{A} - 8K T^{\beta}) + D_{B}(X)(\alpha_{B} - 8K_{2} T^{\beta}) + K T^{\beta}) \\
& = D_{A}(X)\alpha_{A} + D_{B}(X)\alpha_{B} - D_{A}(X)(\alpha_{A} - 8K T^{\beta}) - D_{B}(X)(\alpha_{B} - 8K_{2} T^{\beta}) - K T^{\beta} \\
& =  D_{A}(X)8K T^{\beta} + D_{B}(X)8K_{2} T^{\beta} - K T^{\beta}  \\
& \geq 2K T^{\beta} +2K_{2} T^{\beta} - K T^{\beta} \\
& = K T^{\beta} +2K_2 T^{\beta} > 0 \\
\end{align*}

Next, for Y:

\begin{align*}
& d'(Y)(\alpha_{A} + \alpha_{B}) - (D_{A}(Y)(\alpha_{A} - 8K T^{\beta}) + D_{B}(Y)(\alpha_{B} - 8K_{2} T^{\beta}) + K_{2} T^{\beta}) \\
& = D_{A}(Y)\alpha_{A} + D_{B}(Y)\alpha_{B} - D_{A}(Y)(\alpha_{A} - 8K T^{\beta}) - D_{B}(Y)(\alpha_{B} - 8K_{2} T^{\beta}) - K_{2} T^{\beta}  \\
& =  D_{A}(Y)8K T^{\beta} + D_{B}(Y)8K_{2} T^{\beta} + 8K_{2} - K_{2} T^{\beta}  \\
& \geq 2K T^{\beta} +2K_{2} T^{\beta} - K_{2} T^{\beta} \\
& = 2K T^{\beta} + K_{2} T^{\beta} > 0\\
\end{align*}


Thus, this is a valid construction, and note that by construction we have played $X$ and $Y$ the same total frequency across the rounds, and therefore the endpoint will be exactly the same and the number of rounds will be as well. Furthermore, we will now show that the CSP of this segment is very close to the CSP of the original segment. In the new segment, because we have moved $2T^{\beta}$ away from the hard boundary and because we can only move back by $T^{\regret}$ as we play $D_{A}$, the learner will play $A$ the whole time against this (except for a sublinear fraction of the rounds). Furthermore, for the same reason, the learner plays $B$ against $D_{B}$ when we play it (except for a sublinear fraction of the rounds). The other drivers of change in the CSP is the $O(T^\beta)$ rounds of $\alpha_A$ that we do not play $D_A$ (similar for $D_B$
), the $O(T^\beta)$ rounds of playing $Y$ that are required to go from the region where $A$ is the clear leader to where $B$ is the clear leader and the $O(T^\beta)$ rounds of play at the end to reach the same end point as the original segment. Even if all these changes go in the same direction, the net effect on the CSP is at most $O(T^{\beta})$ deviation in the 
$\ell_1$ distance (each round can only effect a change of $O(1)$), which is sublinear.

%just $D_{A}$, in region $A$ (making sure we start like $T^{\regret}$ away from the boundary). This will only be $T^{\alpha}$-far from $c'$. Also, because $|\mu_{\mathcal{L}}(D_{A},A) - \mu_{\mathcal{L}}(D_{A},B)| \leq T^{\regret-1}$, we end up in a pretty similar place; cut off early to travel back if need be, it will only cut off early by $T^{\regret}$.

\item Case 2: $\alpha_{A} \geq T^{\beta}$, $\alpha_{B} \leq T^{\beta}$. Then we have that $|\mu_{\mathcal{L}}(D_{A},A) - \mu_{\mathcal{L}}(D_{A},B)| \leq T^{\regret-1}$. The new sequence we will construct is as follows: from the hard boundary, play $X$ until $u_{t} = T^{\alpha + \gamma}$. By Observation~\ref{obs:shifts}, this will take $K T^{\alpha + \gamma}$ rounds for some constant $K$. Then, play $D_{A}$ for $\alpha_{A} + \alpha_{B} - 8K T^{\alpha + \gamma}$ rounds. Then, let us consider the number of times we have played $x$ so far. It is $D_{A}(X)(\alpha_{A} + \alpha_{B} - 8K T^{\alpha + \gamma}) + K T^{\alpha + \gamma}$. 


Let $D_{A}(Y)$ be the fraction of the time that $Y$ is played in $D_{A}$, and define $D_{A}(X)$, $D_{B}(Y)$, and $D_{B}(X)$ accordingly. Then the number of times we have played $Y$ so far is upper bounded by $D_{A}(Y)(\alpha_{A} + \alpha_{B} - 8K T^{\alpha + \gamma})$. So we will play $Y$ the suitable number of times to reach the same endpoint, this number is lower bounded by $d'(Y) (\alpha_{A} + \alpha_{B}) - D_{A}(Y)(\alpha_{A} + \alpha_{B} - 8K T^{\alpha + \gamma})$, and similarly $X$ a suitable number of times, lower bounded by  $d'(X)(\alpha_{A} + \alpha_{B})  - D_{A}(X)(\alpha_{A} + \alpha_{B} - 8K T^{\alpha + \gamma}) - K T^{\alpha + \gamma}$ times. Once again , we show that these are both non-negative values to show this is a valid construction.

%Note that by the fact that $D_{A}$ approximately equalizes between $A$ and $B$, $D_{A}(X) > \frac{1}{4}$ (EZ to prove but must prove I guess). 



\begin{align*}
& d'(X) - D_{A}(X)(\alpha_{A} + \alpha_{B} - 8K T^{\alpha + \gamma}) - K T^{\alpha + \gamma} \\
& = D_{A}(X)\alpha_{A} + D_{B}(X)\alpha_{B} - D_{A}(X)(\alpha_{A} + \alpha_{B} - 8K T^{\alpha + \gamma}) - K T^{\alpha + \gamma} \\
& = D_{B}(X)\alpha_{B} - D_{A}(X)\alpha_{B} + 8D_{A}(X)K T^{\alpha + \gamma} - K T^{\alpha + \gamma} \\
& > \alpha_{B}(D_{B}(X) - D_{A}(X)) + K T^{\alpha + \gamma} \\
& \geq  -\alpha_{B} + K T^{\alpha + \gamma} \\
& \geq KT^{\alpha + \gamma} - T^{\beta} \\
& > 0 \tag{For sufficiently large T}
\end{align*}

Next, for Y:

\begin{align*}
& d'(Y) - D_{A}(Y)(\alpha_{A} + \alpha_{B} - 8K T^{\alpha + \gamma}) \\
& = D_{A}(Y)\alpha_{A} + D_{B}(Y)\alpha_{B} - D_{A}(Y)(\alpha_{A} + \alpha_{B} - 8K T^{\alpha + \gamma}) \\
& = D_{B}(Y)\alpha_{B} - D_{A}(Y)(\alpha_{B} - 8K T^{\alpha + \gamma}) \\
& = \alpha_{B}(D_{B}(Y) - D_{A}(Y)) + 8K T^{\alpha + \gamma} \\
& \geq  -\alpha_{B} + 8K T^{\alpha + \gamma} \\
& \geq  -T^{\alpha+\gamma} + 8K T^{\alpha + \gamma} \\
& > 0 \tag{For sufficiently large T}
\end{align*}


Thus, this is a valid construction, and note that by construction we have played $X$ and $Y$ the same total frequency across the rounds, and therefore the endpoint will be exactly the same. The proof showing that the CSP of this segment is very close to the CSP of the original segment is similar to that of Case 1. The main difference is in additionally using the fact that $\alpha_B \le T^\beta$, since we discard that many rounds of play of $D_B$ and add a similar number of rounds of $D_A$.


\item Case 3: $\alpha_{A} \leq T^{\beta}$, $\alpha_{B} \geq T^{\beta}$. This follows by a symmetric argument to the case above.


\item Case 4: $\alpha_{A} \leq T^{\beta}$, $\alpha_{B} \leq T^{\beta}$. Then, we do not need to modify this segment at all--we are not changing the CSP at all, and as the entire segment is of length at most $2T^{\beta}$, we are not spending more than $2T^{\beta}$ time within the soft boundary.
\end{itemize}




%\esh{Add note about ensuring finish at the same end pt., at the cost of $O(T^\regret + \boundary)$ extratime steps}




\begin{lemma}

Every non-crossing segment can be replaced with a segment that :
\begin{itemize}
    \item Has the same start and end points, and runs for the same time period as the original segment. \nat{Change to runs for a very close to same time period?}\esh{Yes, and likewise for the prev . lemma}
    \item Spends only $O(T^{\regret} + T^{\boundary})$ rounds outside the clear leader zone
    \item Induces a CSP which is different by at most $O(T^{\regret - 1} + T^{\boundary - 1})$ from the CSP before replacement.
\end{itemize}
 
\end{lemma}

\begin{proof}
We will
    \esh{Outline - Offset to the hard boundary, come back and rejoin - not too much diff in CSP, then use the previous lemma}
\end{proof}




%\begin{lemma}
%\label{lem:different_lengths}
%Let there be some segment $s_{1}$ with start point $(u_{s1},v_{s1})$, end point $(u_{e1},v_{e1})$ which runs for $t$ rounds. Let there also be some segment $s_{2}$ with the same start point, and an end point $(u_{e2},v_{e2})$ which runs for $t + t'$ rounds. If $|CSP(s_{1})- CSP(s_{2})| = F$ and $|u_{e1} + v_{e1} - u_{e_{2}} - v_{e2}| < G$, then there exists a segment $s_{3}$ such that $|CSP(s_{3}) - CSP(s_{2})| \leq F + G$, $(u_{s1},v_{s1}) = (u_{s3},v_{s3})$, $(u_{e1}, v_{e1}) = (u_{e_{2}} - v_{e2})$, and $|t_{1} - t_{2}| < H + G$.
%\end{lemma}




\begin{lemma}
Over all of $\mathcal{G}$, the limit menu $\M$ of any mean-based no-regret algorithm $\A$ satisfying Assumptions~\esh{add refs} is equal to MB. \label{lem:MWMB}
\end{lemma}
\begin{proof}
%Combines lemmas~\ref{lem:smallnumber} and~\ref{lem:badcases}. 
By definition of $MB$, $MB \subseteq \M$. The non-trivial direction to prove is $\M \subseteq MB$. To this end, we pick up any point $P \in \M_T$ (the menu of algorithm $\A$ for time horizon $T$), study the corresponding optimizer sequence $x_1, x_2 \cdots x_T$ and the induced trajectory, and come up with an optimizer sequence, that when played against an arbitrary MBNR algorithm $\B$, induces a CSP $P'$ that is sub-constant close to $P$. We know that every point in the asymptotic menu $\M$ has a sequence of points $P_1,P_2 \cdots$ converging to it with $P_T \in \M_T$. Using the above transformation, we get a sequence of points $P'_1,P'_2 \cdots$ that also converge to $P$ with $P'_T$ in the menu of an arbitrary MBNR algorithm for time horizon $T$.Thus, we show that $\M$ is contained in the menu of all MBNR algorithms, i.e. $\M \subseteq MB$. %\esh{Add the modification for no. of time steps}


We focus now on generating $P'$ from $P$ for a finite time horizon $T$. The procedure starts by decomposing the trajectory of the point $P$ in the state space defined above into I,C1,C2,NC1,NC2 and F segments. Each segment is then replaced with another segment (by a suitable modification of the optimizer actions)  with the same start and end point so that the new trajectory has the property that only sublinear time is spent outside the regions with a clear leader. We maintain the invariant that the CSP induced by this new sequence/ trajectory against algorithm $\A$ is only sub-constant different from $P$. However, since all MBNR algorithms behave identically, upto a sub-constant factor, in a zone with a clear leader, the CSP  induced by this optimizer sequence against any MBNR algorithm is identical to $P$, upto sub-constant shift. For ease of analysis, we multiply the CSP by a factor of $T$ in this proof, and thus maintain the invariant that the CSP is shifted by a sublinear factor $o(T)$.

Dealing with the Crossing segments of the type C1 or C2 is the easiest part of the transformation - these segments already spend their entire duration (except possibly their first and last moves) in a region with a single clear leader, so we can leave them untouched. To deal with non-crossing segments (C1/C2); we make use of Lemma~\ref{lem:nc_replacement} to replace them one by one with a segment that has the same start and end point, operates for roughly the same time duration ($\pm O(T^\beta))$), results in a trajectory that spends time at most $O(T^\regret + \boundary)$ outside the clear leader region and generates a CSP shifted by only $O(T\alpha + \boundary)$ from the starting trajectory's CSP. A concern with this sequence of transformations is that sufficiently large number of crossing segments can result in linear drift from the original CSP/ linear time spent outside the clear leader zone. To address this issue, we split the analysis into two parts. Let $\beta = max(\regret, \boundary)$ and set $\kappa = (1+\beta)/2$ - since $\regret, \boundary < 1$ (regret bounds and mean-based property), $\kappa \in (\beta,1)$. We split the time horizon $T$ into the first $T^\kappa$ time steps and the remaining time steps. The play in the first part can only affect the CSP by $O(T^\kappa)$, further the total time spent outside the clear leader zone in the first part is also upper bounded by $T^\kappa$. Using Lemma~\ref{lemma:bound_crossing}, there are at most $T^{1-\kappa}$ crossing segments in the second half. Therefore, the total drift (or distance) from the original CSP is upper bounded by $T^{1-\kappa + \beta} = o(T)$. Similarly, in the time steps corresponding to the crossing segments, the final trajectory spend time at most $o(T)$ away from the boundary. The change in the total number of time steps is also $o(T)$
for the same reason. 

A similar analysis can be done for the initial (I) and final (F) segment, by only replacing the non-crossing part of their trajectories using Lemma~\ref{lem:nc_replacement} and contributing an additional $o(T)$ drift away from the original CSP, and $o(T)$ additional time spent away from the clear leader zone. To finish with exactly the same number of time steps, we simply truncate/ extend the trajectory by the required number of steps. Since this number is $o(T)$, the other properties remain true.



%\esh{working}
\end{proof}
\end{comment}



\begin{comment}
    


\begin{lemma}
MB is a polytope on $\mathcal{G}$. \label{lem:MBpolytope}
\end{lemma}
\begin{proof}
TODO
\end{proof}


\begin{lemma}
The limit menus for all mean-based no-regret algorithms are polytopes on $\mathcal{G}$. \label{lem:mwpolytope}
\end{lemma}
\begin{proof}
Combines lemma~\ref{lem:MBpolytope} and lemma~\ref{lem:MWMB}. 
\end{proof}



\begin{lemma}
\label{lem:sr   meanbased}
For all $\gamma$ mean-based algorithms and all learner payoffs $\mathcal{G}$%, if the asymptptic menu of this algorithm is a polytope
, there is some vertex in any asymptotic menu with maximin learner value which has significant  swap regret (at least $\frac{T}{1000}$). 
\end{lemma}

\esh{Have to be careful about whether this implies the existence of an {\bf extreme} point of the menu with the same properties- regret/swap-regret is non-linear}
\esh{Added in the fix, the proof seems to work beyond polytope menus}



The proof of this lemma can be found in Section~\ref{sec:proof_srmeanbased}.




\begin{theorem}
All mean-based no-regret algorithms satisfying Assumptions~\ref{} are pareto-dominated.
\end{theorem}
\begin{proof}
Combines lemma~\ref{lem:srmeanbased} and lemma~\ref{lem:mwpolytope} to say that we can remove a minmax point from any mean-based no-regret algorithm.
\end{proof}
\end{comment}



\begin{comment}
    


\subsection{Redundant Lemmas}


\begin{lemma}
Any trajectory can be replaced by a distributionally-equivalent trajectory starting and ending at the same points which has at most $4$ boundary segments for every crossing between the CB boundary and the AB boundary.  \label{lem:shifting} 
\end{lemma}


\begin{proof}
For any algorithm with mean-based parameter $T^{\alpha}$ and an upper bound on regret of $T^{\beta}$ where $\alpha,\beta < 1$, any subsequence of a trajectory of play which begins within a boundary and ends within the same boundary while only passing through adjacent regions in the interim can be replaced by a trajectory which begins and ends in the same places, induces the same move pair distributions throughout, and has at most 4 contiguous segments within a boundary. Then you just have to match up the boundary shifts with the different times spent at each line.
\end{proof}





\esh{Useful in the following way - only the CB or AB difference matters when small, since the third action is always much much worse}

\esh{SW implies regret between the soft boundaries}
%MB = Intersection of all mean based algorithms' menus

%MW = Menu of multiplicative weights

%Jon's proof - MB is a polytope for all 3x2 games (based upon characterization for trajectories corresponding to extreme points of the menu)

%Is MW = MB?

%Proof Idea -- Continuous Induction

%Base Case - Consider any trajectory for MW that is either exactly on the boundary or is well away from the boundary for most of the time - we can simulate the effect of such a trajectory using a generic MB algorithm

%Induction case - Start with a menu point of MW (correspondingly a trajectory that shows MW reaching this point) and a generic MB trajectory that also achieves this point. Make a small change to the trajectory of MW (and consequently a small change to the menu point)- then we need to show that there exists a small change to the generic MB trajectory achieving the new point.

%Some constraints - this induction step must critically use the fact that MW has a continuous mapping from trajectories to menu points, otherwise this proof is bogus because it would be possible to show FTL=MB resulting in a contradiction. 

%Can we split the sublinear region into multiple sections and average the moves of the learner? Using continuity? 






%\begin{lemma}
%Any trajectory which spends $o(T)$ time within the boundaries can be approximated to within $o(T)$ by any mean-based learning algorithm.
%\label{lem:smallsum}
%\end{lemma}

\begin{lemma}
Every trajectory on this set of games can be represented by a distributionally equivalent trajectory which has at most $T^{1-\alpha-\gamma}$ contiguous segments within a boundary.
\label{lem:badcases}
\end{lemma}
\begin{proof}
Using lemma ~\ref{lem:shifting}, we can get to a point where each boundary segment is associated with a crossing. Let us assume that there are at least $T^{1-\alpha}$ segments within a boundary. Using~\ref{lem:constant}, after $T^{\alpha + 0.1}$ rounds, the trajectory must be at least $B \cdot T^{\alpha + 0.1}$-far from the boundary. We can ignore this whole segment. Every time after this that the line is leaving a boundary to cross, it must be at least $o(B \cdot T^{\alpha + 0.1})$-far along this line. Since there are at least $T^{1-\alpha}$ different segments, there are at least $\frac{T^{1-\alpha}}{4}$ different crossings, and thus the total time steps spent crossing is at least $\frac{BT^{1.1}}{4}$. For some choice of $T$ this is impossible, and thus this derives a contradiction. 
\end{proof}

\begin{lemma}
Any trajectory which has at most $T^{1-\alpha - \gamma}$ contiguous segments within a boundary can be approximation to within $o(T)$ by any $T^{\alpha}$ mean-based no-regret learning algorithm, for any constant $\gamma > 0$. \label{lem:smallnumber}
\end{lemma}

\begin{proof}

Let us consider all trajectories which lie within a particular boundary in the same region. If these trajectories together have sublinear length, we can ignore them. Otherwise, they have length at least $d \cdot T$. Let us compute the joint move distribution over all these trajectories. If this distribution is large, then



If they have length $d \cdot T$ for some constant $d$, then the best response to 


Use the no-regret property to compute the distributions along each boundary, every time you get back to the boundary, go left then right in this way. If you don't have enough time to do such a thing, just take the L and stay on one side. Each segment you get an approximation error of $o(T^{\alpha})$, and there are $T^{1 - \alpha - \gamma}$ of them, so the total approximation error induced by this is at most $T^{1 - \gamma}$, which is $o(T)$. 
\end{proof}

\end{comment}

==> old/ftpl_ftl.tex <==
\begin{lemma}
There exists a game $G$ where FTL outperforms FTPL and MW by an $\Omega(T)$ additive factor. A fortiori, FTL is not pareto dominated by either FTPL or MW.
\end{lemma}

\begin{proof}
The game $G$ of interest is defined by the matrix below. The learner is the row player and has actions A and B (first and second row respectively) whereas the optimizer is the column player and has actions X and Y respectively.
 \[
\begin{bmatrix}
 (2,-3) & (1,1)\\
 (2,1) & (1,0) 
\end{bmatrix}
\]

We define Follow the Leader (FTL) as playing the best action in hindsight with ties broken in favour of the second action (B).

Regardless of the action chosen by the column player in any round, the row player gets equal payoffs from both actions, and thus historically both actions always have the same payoff at any round of play. Thus, the learner when playing FTPL or MW, picks each action with equal probability in every round, and when playing FTL, picks action B in every round due to the tie breaking rule. Consequently, the best response of the optimizer in the case of FTL is to always play action X and in the case of FTPL / MW to always play action Y. This leads to the FTPL/ MW learner obtaining an average payoff of 1 while the FTL learner receives an average payoff of 2.


This example game can be embedded into a game where the first player has $n \ge 2$ actions, while preserving the same result (FTL does $\Omega(T)$ better than FTPL/MW). The payoff for any pair involving the learner playing any action except for the first two actions is 0 for both the learner and optimizer. The idea that FTPL/ MW plays action A and action B with equal probability in each rounds remains invariant in this extended game. Further, FTL always plays action B, while the no regret property of FTPL/ MW ensures that the historical time average probability of the learner playing actions other than A or B is $o(T)$. Putting together these observations gives the same result.
\end{proof}



==> old/notes.tex <==
Questions/ Issues about the Model :

1. Computable Functions , Finite input, etc.?

2. No more correlated randomness, is this alright?

3. Learner payoff $u_L$ not included in most notation, even thought it is implicitly there

4. Should we discuss the optimizer being oblivious (since there is no more scope for correlated play)?


5. Reference for converging subsequence for algorithms that are not consistent?

6. Notion of domination in context of multiplicity of menus for inconsistent algorithms - should we make the domination def strong or weak? Stronger makes it easier to prove things, but weaker seems better because it strengthens the notion of pareto optimality. Natalie correctly points out that weaker definitions can admit absurdities, such as both algorithms dominating each other. An alternative is to restrict our discussion to consistent families, but some of our results apply more broadly.


After Prelims:

1. Characterize Menus

2. Provide intuition with simplest pareto-domination result ( do this in the intro)

3. Think about menus rather than algorithms


Other Issues:

1. Can we drop dominated actions from the learner's action space? It can simplify at least one proof (NSR convergence), but might be useful to illustrate examples


Extras:

1. Might be worth pointing out somewhere that MW and NSR are incomparable (if the relevant example can be robustfied)





\subsection{Meeting 3/27 Notes} 

Ways to make the notion of Pareto dominance stronger:
Should dominate for a positive measure set of games. "Robustly" Pareto-dominant. 

Original hope:
Partially fix the game by keeping the learner's payoffs fixed. Game between learner and optimizer, learner has a fixed number of actions. Now we just vary the optimizer’s payoffs and show there’s some setting where algorithm 2 does better than algorithm 1.

The idea of menus: You can condense a transcript down to the the distribution over joint strategies, fraction of times that an action pair turns up a certain way. The menu is the set of joint strategy distributions that the learner's algorithm can induce given this set of payoffs for the learner. The optimizer can choose between one of these strategies. Any extreme point in this set (from the perspective of the optimizer) is also one for which there is some game where they will choose to pick that point.


Mechanism design problem:
The optimizer has private info
Learner: I am running this learning algorithm. It restricts the type of outcome you can get to this set. You can choose.
Is there every two menus you can show where one is always better than the other? One special case of this, for fixed learner payoffs, there is a point maximizing the learner's payoff over all possible joint strategy profiles (corresponding to a single action pair). If the menu does not contain this point, then we can construct a second algorithm that contains this point (maybe only this point?) and therefore guarantees pareto dominance


Look at limits as T goes to infinity in general 
Fix some o(T) function—allow the follower to respond up to a o(T) factor in favor of the leader






Two questions that don’t seem resolved:

1. Fix a “generic” $U_{L}$. What we do from now should be true for all but a measure 0 set of $U_{L}$. Is multiplicative weights ever Pareto-dominated? We know that some things are, like the constant action algorithm. \\
2. For generic $U_L$ and $U_O$, is any algorithm “robustly” Pareto-dominated?  For this, we need to replace menus with something else.\\

Also: 
3. Robustify lemma 2. Is the menu you can get in FTL a strict superset of the things you can get in FTPL? Is this actually ever useful from the learner’s perspective? 


You can construct learning algorithms where you let the optimizer reach any CCE when playing against them


% \input{ftpl_ftl}

% NOTE: the above instance can also be used to show that there exist a NSR algorithm which is dominated by another algorithm (also NSR). NSR algo A: blum aggregation~\cite{blum2007external} of MW, NSR algo B: play move B until payoff is below 2 (assume here payoffs upper bounded by 2) and then switch to playing A from clean slate. B should always do as well as A. On the instance above, B should strictly outperform.  \\
% NOTE ON THIS NOTE AFTER 3/27 MEETING: this is no longer the case if we require robust pareto domination. the fact that the payoffs for the learner are exactly the same regardless of the optimizer's actions is a measure 0 event and slightly perturbing this negates this example. 

% \section{Conjectures/ Ideas}

% NSR - Limit menu a polytope?


\begin{comment}
    

\subsection{Observations/ Questions}
\begin{itemize}
    \item Any algorithm that dominates a NR algorithm must:
    \begin{itemize}
        \item contain L+ in its menu
        \item have its menu exclusively containing points that provide at least the maximin value to the leader
        \item contain all responses to a dominant strategy in its menu, if a dominant strategy exists for the leader (and all payoffs are unique)
    \end{itemize}
    \item Does a NR algorithm dominate the algorithm that plays the maximin value all the time?
    \begin{itemize}
        \item Games of perfect cooperation (max value aligns) contain examples where NR does better than the above algorithm 
        \item Do NSR algorithms dominate? Answering this boils down to the following question - comparing A and B
        \begin{enumerate}
            \item A= Learner payoff for the optimizer BR to the learner maximin strategy
            \item B = Learner BR payoff against the follower's static Stackleberg strategy
        \end{enumerate}
        \item For zero sum games, A=B=V
        \item for games with a dominant strategy for the learner, B=A
        \item In games of perfect cooperation, B $>$ A
    \end{itemize}

    We tried coming up with a 2x2 game example where B $\leq$ A but have not yet had success.
\end{itemize}
\end{comment}



\subsection{Notes on some difficulties}

Some concerns Eshwar and I have about the model: 
For a couple of our proofs, we need this condition: (1) when a learner moves from some strategy to a "default" algorithm, the time-averaged payoff for the learner against a best-responding optimizer for the remainder of the game is sublinearly close to her time-averaged payoff if she had just played the default algorithm all along. For a finite horizon setting, the following would get us there: for large enough $T$ and any $T' \geq T$, the learner's time-averaged payoff for $A_{T}$ is very close to her time-averaged payoff for $A_{T'}$ for a fixed game $G$ and a best-responding optimizer. We attempted to ensure this by giving a seemingly stronger condition: for any fixed learner payoffs $u_{L}$, the entire menu of $A_{T}$ is very close to the entire menu of $A_{T'}$. However, this is not actually a strictly stronger condition. 

It is in fact not enough to say that the menu induced at $T$ vs a larger $T'$ is very close to the same (even if the distance is sublinear). This is because, even if the points are all very similar, any tiny shift could lead to a new point being the best point for the optimizer, and this point could lead to a completely different value for the learner. So the menus themselves being "consistent" does not give us the fact that $A_{T}$ and $A_{T'}$ on the same game $G$ will garner similar payoffs for the learner. We have to be very, very precise about what a consistent family of learning algorithms is. One idea is to only allow algorithms for which, for large enough $T$, the $\frac{T}{c}$-length prefix of play induced by a best-responding follower has a very similar (sublinearly different) distribution to the $T$-length total transcript of play induced by a best-responding follower, for any constant $c$. 
\nat{eshwar: we encountered more problems with following this approach but I am not remembering now, do you remember?}

Another approach is to only consider infinite-horizon games and algorithms that can play them. This immediately gets us condition (1). But it introduces some more complexities into our modeling. It is not clear that menus are well-defined anymore. Even if we constrain the learner to playing algorithms with well-defined limit averages (i.e., we exclude algorithms like "play move 1 for 2 rounds, play move 2 for 4 rounds, play move 1 for 8 rounds... etc), the optimizer can still employ such an algorithm in response. This may not be a best-response, but the menu is supposed to include all things the optimizer could play, not just best-responses. What is the menu point induced by the optimizer playing this geometric series?


\begin{note}
    Here is one additional property for consistent families that would suffice for our purpose -- for every learner payoff and for every optimizer payoff, the induced distribution (over action pairs) of the best response play converges. Does MW have this property?
\end{note}


\begin{definition}
    Associated with any learning algorithm $\A_T$, for every learner payoff $u_L$, we define a menu $S_T \subseteq \Delta^{mn}$ in the following manner:

    
    \begin{align*}  
    S_T (u_l) &= \text{Conv}\Bigg\{p \in \Delta^{mn} : \exists \text{ optimizer sequence } (y_1,y_2,\cdots y_T) \\
    &\qquad\qquad\qquad\quad\; \text{ where } y_t \in \Delta^n \text{ such that } p = \frac{1}{T} \sum_{t=1}^T x_t \otimes y_t \\
    &\qquad\qquad\qquad\quad\; \text{ and } x_1,x_2,\cdots x_t \text{ is the sequence played by algorithm $\A_T$ against this optimizer sequence}  \Bigg\}
\end{align*}
\end{definition}

Because the optimizer can play any sequence and knows the expected payoff that this sequence will receive against the learner's algorithm, we can think of the optimizer as being able to pick their favorite element in the menu. 

\begin{definition}
For any learning algorithm $\mathcal{A}_{T}$ with an associated menu $S_{T}$, a best response by the optimizer (induces
\end{definition}

\begin{definition}
    A family $\{\A_T\}_T$ of learning algorithms with the associated menus $\{S_T\}_T$ is said to be consistent if there exists a set $S \subseteq \Delta^{mn}$ s.t.
    \begin{enumerate}
        \item $
        \lim_{T \rightarrow \infty} S_T \rightarrow S$
        under some suitable distance metric
        \item $\cup_{T=1}^\infty S_T  = S$
    \end{enumerate}
\end{definition}

\nat{proposal: A family $\{\A_T\}_T$ of learning algorithms is said to be consistent if there exists a $T$ such that, for all $T' \geq T$, the $T$-length prefix of the }

\begin{definition}
    We say that learning algorithm $\A$ dominates learning algorithm $\B$ 
\end{definition}



==> old/nr_nsr_backup.tex <==
\section{No-regret and no-swap-regret menus}
\label{sec:NSR}

Another nice property of working with asymptotic menus is that no-regret and no-swap-regret properties of algorithms translate directly to similar properties on these algorithms' asymptotic menus (the situation for mean-based algorithms is a little bit more complex, and we discuss it in Section~\ref{sec:mean_based_pareto_dominated}). 


To elaborate, say that the CSP $\csp$ is \emph{no-regret} if it satisfies the no-regret constraint

$$\sum_{i\in[m]}\sum_{j\in[n]} \csp_{ij}u_{L}(i, j) \geq \max_{j^{*} \in [n]}\sum_{i\in[m]}\sum_{j\in[n]} \csp_{ij}u_{L}(i, j^*).$$


\noindent
Similarly, say that the CSP $\csp$ is \emph{no-swap-regret} if, for each $i \in [m]$, it satisfies

$$\sum_{j \in [n]} \csp_{ij}u_{L}(i, j) \geq \max_{j^* \in [n]} \sum_{j \in [n]} \csp_{ij}u_{L}(i, j^*).$$


We will define the \emph{no-regret menu} $\M_{NR}$ to be the convex hull of all no-regret CSPs, and the \emph{no-swap-regret menu} $\M_{NSR}$ to be the convex hull of all no-swap-regret CSPs. In the following theorem we show that the asymptotic menu of any no-(swap-)regret algorithm is contained in the no-(swap-)regret menu.

\begin{theorem}
\label{thm:nr_nsr_containment}
If learning algorithm $\cA$ is no-regret, then $\M(\cA) \subseteq \M_{NR}$. If $\cA$ is no-swap-regret, then $\M(\cA) \subseteq \M_{NSR}$.
\end{theorem}
\begin{proof}

We introduce two families of sets to aid with this proof. Let $\M_{NR}(\varepsilon)$ denote the relaxation of the set $\M_{NR}$ where the no-regret constraint is relaxed to :

$$\sum_{i\in[m]}\sum_{j\in[n]} \csp_{ij}u_{L}(i, j) \geq \max_{j^{*} \in [n]}\sum_{i\in[m]}\sum_{j\in[n]} \csp_{ij}u_{L}(i, j^*) - \varepsilon.$$

Similarly, $\M_{NSR}(\varepsilon)$ denotes the relaxation of the set $\M_{NSR}$ where the no-swap-regret constraint is relaxed to :

$$\sum_{j \in [n]} \csp_{ij}u_{L}(i, j) \geq \max_{j^* \in [n]} \sum_{j \in [n]} \csp_{ij}u_{L}(i, j^*) - \varepsilon.$$

    Let $\A$ be a no-regret algorithm. Then, its average total regret over $T$ rounds is upper bounded by some function $f(T,n)$ such that $\lim_{T \rightarrow \infty} \frac{f(T,n)}{T} = 0$. WLOG, let $f(T_1,n) < f(T_2,n)$ if $T_1 < T_2$. For each time horizon $T$, we define the set $S_T := M_{NR}\left( \varepsilon_T \right)$ where $\varepsilon_T = \frac{f(T,n)}{T}$. Let $\M_T$ denote the menu corresponding to the algorithm $\A$ run for $T$ steps. It follows from the no-regret constraint that $\M_T \subseteq S_T$. It is easy to see that $S_1 \supseteq S_2 \supseteq \cdots S_T \cdots$ and $\M_{NR} \subseteq S_T$ for all time horizons $T$.Thus we note that $\lim_{T \rightarrow \infty} S_T = \M_{NR}$ since $\lim_{T \rightarrow \infty}  \varepsilon_T = 0$ (which implies that $\M_{NR}$ is the maximal set contained in all the $\{S_T\}$ sets). (~\esh{Citation/ proof needed for this step or the next one?}). Thus, $\M(\A) \subseteq \M_{NR}$.

A similar argument works for no-swap-regret through the use of the corresponding relaxation.
\end{proof}

Note that both $\M_{NR}$ and $\M_{NSR}$ themselves are valid asymptotic menus, since for any $x \in \Delta_{m}$, they will contain some point of the form $x \otimes y$ for some $y \in \BR_{L}(x)$. In fact, we can say something much stronger about the no-swap-regret menu: it is exactly the convex hull of all such points.

\begin{lemma}\label{lem:nsr_characterization}
The no-swap-regret menu $\M_{NSR}$ is the convex hull of all CSPs of the form $x \otimes y$, with $x \in \Delta_{m}$ and $y \in \BR_{L}(x)$.
\end{lemma}
\begin{proof}
%\jon{INSERT. Maybe should also mention this is the same as the ``half-correlated-equilibrium'' $(\emptyset, \mathcal{I})$ polytope defined in Brown-Schneider-Vodrahalli.}



First, we see that every CSP of the form $x \otimes y$, with $x \in \Delta_{m}$ and $y \in \BR_{L}(x)$ is contained in $\M_{NSR}$. This follows directly follows from the fact that this CSP satisfies the no-swap-regret constraint, since no action can be a better response than $y$ to $x$.~\footnote{The no-regret property is sufficient.}

For the other direction, consider a point $X \in P_{NSR}$ - let $x_{ij}$ denote the $i,j$-th coordinate of $X$. We rewrite $X$ as a convex conbination of product measures over action pairs. For each pure learner strategy $a$, let $\beta(a)$ represent the conditional marginal strategy of the optimizer corresponding to $X$ given that the learner plays action $a$, i.e. $\beta_j(a) =\frac{X_{ja}}{\sum_{k \in [m]} X_{ka}}$ for all $j \in [m]$. For the case where all the quantities $\{X_{ka}\}_k$ are $0$, we set  $\beta_k(a) = 0$ for all $k \in [m]$. For each action $a$ of the learner, the $\beta_j(a)$s aggregate to form a probability vector $\beta(a) \in \Delta_{m}$. Completing the rewrite $X = \sum_{a \in [m]} (\sum_{k \in [m]} X_{ka}) \beta(a) \otimes a$. For any action $a$ of the learner, if $a \notin \argmax_{b} u_L(\beta(a), b)$, this would imply the existence of swap regret associated with $X$. Since $X \in P_{NSR} $, this implies that for all pure strategies $a$ of the learner, $a \in \argmax_b u_L(\beta(a), b)$. Thus, we have rewritten $X$ as a convex combination of CSPs of the desired form, completing the proof.
   % To show that $P_{NSR} \subseteq S$, consider a point $X \in P_{NSR}$ - let $x_{ij}$ denote the $i,j$-th coordinate of $X$. We rewrite $X$ as a sum of product measures over action pairs. For each action $a$, let $\mathbbm{1}_a \in \delta^{[m]}$ represent the learner strategy that puts all the mass on action $a \in [m]$. Let $\beta(a)$ represent the conditional marginal strategy of the optimizer corresponding to $X$ given that the learner plays action $a$, i.e. $\beta_j(a) =\frac{X_{aj}}{\sum_{k \in [n]} X_{ak}}$ for all $j \in [n]$ (for the egde case, where all the quantities $\{X_{ak}\}_k$ are $0$, we set  $\beta_k(a) = 0$ for all $k \in [n]$). For each action $a$ of the learner, the $\beta_j(a)$s aggregate to form a probability vector $\beta \in \delta^{[n]}$. Completing the rewrite $X = \sum_{a \in [m]} (\sum_{k \in [n]} X_{ak}) \mathbbm{1}_a \times \beta(a)$. For any action $a$ of the learner, if $a \notin \argmax_b u_L(b,\beta(a))$, this would imply the existence of swap regret associated with $X$. Since $X \in P_{NSR} $, this implies that for all actions $a$, $a \in \argmax_b u_L(b,\beta(a))$. Thus, we have rewritten $X$ as a convex combination of points in $T$, implying $X \in \brmix$ and thus $P_{NSR} \subseteq S$.




\end{proof}


An immediate corollary of the above result, along with Theorem~\ref{thm:characterization}, is that $M_{NSR}$ is an asymptotic menu of some algorithm.
\begin{corollary}
\label{cor:nsr_asymptotic}
    $M_{NSR}$ is an asymptotic menu.
\end{corollary}





This characterization of $\M_{NSR}$ allows us to prove our first main result: that all consistent no-swap-regret algorithms have the same asymptotic menu (namely, $\M_{NSR}$). Notably, this is not generically the case for no-regret algorithms (for example, in general games $\M_{NR}$ and $\M_{NSR}$ can differ, and they are both asymptotic menus for different no-regret algorithms)~\esh{Should we show details in the appendix?}. 

Before stating and proving this result, we prove a key technical property of menus:



\begin{lemma}\label{lem:farkas}
Consider some algorithm $\B$ with asymptotic menu $\M(\B)$ with the property that, for some distribution $x$, all points of the form $x \otimes y$ in $\M(\B)$ must be such that $y$ is a best response to $x$. Then, $\M(\B)$ must include all points of the form $x \otimes y$, for all $y \in \BR_{L}(x)$.
\end{lemma}

\begin{proof}
First, we deal with the case where $y$ is a unique learner best response to $x$. There must be at at least one point $P$ in the menu $\M$ corresponding to the optimizer playing the distribution $x$ in every round. Since $P$ is not equal to $X$ (and therefore the marginal distribution of the learner is different from $x$), and $y$ is a unique best response to $x$, $P$ must not be a best response, leading to a contradiction.

If $y$ is not a unique best-response to $x$, then we find a point $x'$ close to $x$ such that $y$ is a unique best response to $x'$. To this end, we use the Farkas Lemma, from which we get that there exists a distribution $\gamma \in \Delta^m$ such that $\mu_L(\gamma, y) \ge \mu_L(\gamma, y') + \kappa$ for all actions $y' \in [n] \setminus \{y\}$ and some $\kappa > 0$. In this step, we critically use the fact that $y$ is not a weakly dominated strategy (since we discard all learner payoffs with such strategies from consideration). Thus, for small enough $\delta > 0$, the optimizer distribution $x(\delta) =(1-\delta) x  + \delta. \gamma$ has learner action $y$ as a unique best response. If all corresponding points $x(\delta) \times y $ are in $\M$, by closure, $X$ is also in $\M$, resulting in a contradiction. 
\end{proof}


\begin{lemma}
All menus with $U^{-}(M) = U_{ZS}$ must contain all points in $M^{-}$ of the form $x \otimes y$, with $x \in \Delta_{m}$, $y \in \BR_{L}(x)$ (where $y$ is a pure strategy).  \label{lem:minimal_min}
\end{lemma}

\begin{proof}
Assume otherwise, for sake of contradiction. Then there is some menu $\M$ with a point $X =  x \otimes y$ such that $y \in \BR_{L}(x)$ that is not present in $\M$. %Since $\M$ is convex, without loss of generality, $y$ is a pure strategy of the learner. 

Note that for all points in $M^{-}$ of the form $x \otimes y$, with $x \in \Delta_{m}$, $y \in \BR_{L}(x)$, $x$ must be a minmax distribution. Therefore, it is sufficient to prove that all menus with $U^{-}(M) = U_{ZS}$ must contain all points of the form $x_{mm} \otimes y$, where $x_{mm}$ is a minmax distribution and $y \in \BR_{L}(x)$.

By the fact that $U^{-}(M) = U_{ZS}$, if $x_{mm}$ is a minmax distribution, then any point of the form $x_{mm} \otimes y$ in $\M$ must have that $y$ is a best response to $x_{mm}$. By Lemma~\ref{lem:farkas}, for all such $x_{mm}$, $\M$ must include all points of the form $x_{mm} \otimes y$, with $y \in \BR_{L}(x_{mm})$. 

Thus, at least one such point is not in $\M$, in which case we can use the previous case's argument to derive a contradiction, completing the proof.

\end{proof}



\begin{lemma}
\label{lemma:nsr_polytope_is_minimal}
    There is no algorithm $\B$ with asymptotic menu $\M(\B)$ such that $\M(\B) \subset \M_{NSR}$.
\end{lemma} 

\begin{proof}

%\esh{Working}

Let us consider two cases:

\begin{itemize}
\item $\M(\B)$ has points with swap regret. Then, by the fact that $\M_{NSR}$ has no points with swap regret, $\M(\B) \nsubseteq \M_{NSR}$.
\item $\M(\B)$ is a no swap regret menu. Then, $\M(\B)$ has the property that, for all distributions $x$, all points of the form $x \otimes y$ must be such that $y$ is a best response to $x$. By Lemma~\ref{lem:farkas}, $\M(\B)$ must include all points of the form $x \otimes y$, for all $x \in \Delta_m$ and $y \in \BR_{L}(x)$. By Lemma~\ref{lem:nsr_characterization}, the no-swap-regret menu $\M_{NSR}$ is exactly the convex hull of all CSPs of this form. Therefore, $\M_{NSR} \subseteq \M(\B)$.
\end{itemize}

%(the reasoning can be extended by starting at finite time menus and analyzing the limit point of the sequence)%~\esh{Note to self: find/ write a lemma that shows menus have points corresponding to every optimizer marginal distribution}.
%Since $P$ is not equal to $X$ (and therefore the marginal distribution of the learner is different from $\mathbbm{1}_a$), and $a$ is a unique best response to $\beta$, $P$ must have regret associated with it, implying $P \notin P_{NSR}$, however this results in a contradiction with $\M(\B) \subseteq P_{NSR}$, invalidating our assumption.
       
%Assume otherwise, for sake of contradiction. This implies the existence of a point $X = \mathbbm{1}_a \times \beta \in \brmix$ that is not present in $\M(\B)$ (since $P_{NSR}$ is the convex hull of $\brmix$). First, we deal with the case where $a$ is a unique learner best response to the optimizer distribution $\beta$. There must be at at least one point $P$ in the menu $\M(\B)$ corresponding to the optimizer playing the distribution $\beta$ in every round (the reasoning can be extended by starting at finite time menus)~\esh{Note to self: find/ write a lemma that shows menus have points corresponding to every optimizer marginal distribution}. Since $P$ is not equal to $X$ (and therefore the marginal distribution of the learner is different from $\mathbbm{1}_a$), and $a$ is a unique best response to $\beta$, $P$ must have regret associated with it, implying $P \notin P_{NSR}$, however this results in a contradiction with $\M(\B) \subseteq P_{NSR}$, invalidating our assumption. 
    


    
 %If $a$ is not a unique best-response to $\beta$, then we perturb the point to find a $(a,\beta)$ pair such that $a$ is a unique best response to $\beta$ that is not in $\M(\B)$ (if all such points are in $\M(\B)$, then by closure the original point is also in $\M(\B)$ leading to a contradiction) ~\esh{Insert the Farkas Lemma argument here and use closure}. Consider an optimizer that repeatedly plays the distribution $\beta$ against a learner playing algorithm $\B$. Let $\alpha$ be the historical marginal distribution of the learner. If $\alpha \neq \mathbbm{1}_a$, then there is a point in $\M(\B)$ with non-zero swap regret, implying $\M(\B) \not\subset P_{NSR}$, leading to a contradiction. However, if $\alpha = \mathbbm{1}_a$, then $ \mathbbm{1}_a \times \beta 
% \in \M(\B)$, which is again a contradiction. Thus, $P_{NSR}$ is a minimal menu.

 
 \end{proof}


\begin{theorem}\label{thm:unique_nsr_menu}
If $\cA$ is a consistent no-swap-regret algorithm, then $\M(\cA) = \M_{NSR}$.
\end{theorem}
\begin{proof}
Using Theorem~\ref{thm:nr_nsr_containment}, $\M(A) \subseteq \M_{NSR}$. However, Lemma~\ref{lemma:nsr_polytope_is_minimal} rules out the possibility of strict containment, i.e. $\M(\A) \subset \M_{NSR}$ which leaves $\M(\cA) = \M_{NSR}$ as the only possibility.
\end{proof}



Note that in the proof of Theorem \ref{thm:unique_nsr_menu}, we have appealed to Lemma~\ref{lemma:nsr_polytope_is_minimal} which uses the fact that $u_L$ has no weakly dominated actions. This is necessary: consider, for example, a game with two identical actions for the learner, $a$ and $a'$ (i.e. $u_L(\cdot, a) = u_L(\cdot, a')$). We can consider two no-swap-regret algorithms for the learner, one which only plays $a$ and never plays $a'$, and the other which only plays $a'$ and never plays $a$. These two algorithms will have different asymptotic menus, both of which containing only no-swap-regret CSPs. But as mentioned earlier, this is in some sense a degeneracy -- the set of learner payoffs $u_L$ with weakly dominated actions is zero measure (i.e., any small perturbation to $u_L$ will prevent this from taking place). 


\begin{lemma}\label{lem:menu-min-value}
If $\M$ is a no-regret asymptotic menu, then $\Um(\M) = \Uzs$.
\end{lemma}
\begin{proof}
\nat{Theorem \ref{thm:nr_nsr_containment} shows one direction; Lemma~\ref{lem:menu-min-UB} shows the other}
\end{proof}


Unlike $\M^{+}$ which is always equal to $\{\csp^{+}\}$ for Pareto-optimal menus, the minimizing set $\M^{-}$ is not uniquely defined and may contain many CSPs. However, there is a ``minimal'' minimizing set $\M^{-}$ for no-regret menus: for any such menu $\M^{-}$ must contain $\M_{NSR}^{-}$. In fact, this is true for the slightly larger class of menus with $\Um(\M) = \Uzs$. 

\begin{lemma}\label{lem:menu-min-set}
Let $\M$ be an asymptotic menu with $\Um(\M) = \Uzs$. Then $\M_{NSR}^{-} \subseteq \M^{-}$.
\end{lemma}
\begin{proof}


By Lemma~\ref{lem:nsr_characterization}, all extreme points of $\M_{NSR}^{-}$ must be of the form $x \otimes y$, with $x \in \Delta_{m}$ and $y \in \BR_{L}(x)$. Furthermore, by definition, for all points in $\M^{-}$, $u_{L}(x \otimes y) = \Uzs$. By Lemma~\ref{lem:minimal_min}, $\M^{-}$ must also contain all these points. Therefore, $\M_{NSR}^{-} \subseteq \M^{-}$.



\end{proof}



%\begin{lemma}
%If $\M$ is an asymptotic menu of a no-regret learning algorithm, then $\cM \subseteq \cM_{NR}$. If $\M$ is an asymptotic menu of a no-swap-regret learning algorithm, then $\cM \subseteq \cM_{NSR}$.
%\end{lemma}












A careful reading of the first part of the proof of Lemma~\ref{lem:nsr_characterization} highlights that we only the no-regret property in showing that all CSPs of the form $x \otimes y$, with $x \in \Delta_{m}$ and $y \in \BR_{L}(x)$ are contained in $\M_{NSR}$, thus; all such points are contained in $\M_{NR}$. We show below that a more fine grained result is true, where $\M_{NR}$ is replaced by the menu of any no-regret algorithm.

\begin{lemma}
\label{lem:nsr_within_all_nr}
    For any no-regret algorithm $\A$, $\M_{NSR} \subseteq \M(\A)$.
\end{lemma}

\begin{proof}
    We use the characterization provided by Lemma~\ref{lem:nsr_characterization}, which rewrites $\M_{NSR}$ as the convex hull of all CSPs of the form $x \otimes y$, with $x \in \Delta_{m}$ and $y \in \BR_{L}(x)$. Consider any such CSP $x \otimes y$ - our proof is complete if we prove its inclusion in $\M(\A)$.Consider CSPs of the form $x \otimes y'$ in the menu $\M(\A)$ (Theorem~\ref{thm:nr_nsr_containment} tells us that there is at least one such point). Since $\M(\A) \subseteq \M_{NR}$, $y' \in \BR_{L}(x)$ is necessarily true. This satisfies the preconditions of Lemma~\ref{lem:farkas}, which allows us to conclude  that $x \otimes y'' \in \M(\A)$ for all $y'' \in \BR_{L}(x)$; thus $x \otimes y \in \M(\A)$, completing the proof of the lemma.
\end{proof}

A natural question for the reader to ask at this point is whether no-regret algorithms all have $\M_{NR}$ as their asymptotic menu, along the lines of all no-swp regret algorithms having $\M_{NSR}$ as their asymptotic menu. We demonstrate, by counterexample, that this is not the case.

\begin{lemma}
\label{lem:nr_ne_mw}
    There exists a learner payoff where no mean-based no-regret algorithm $\A$ has $\M(\A) = \M_{NR}$. In particular, the menu of the MWU algorithm (See Appendix~\ref{app:mwu_ftpl}) is a strict subset of $\M_{NR}$.
\end{lemma}

\begin{proof}
proof sketch: show a game with a point that is no regret but which can't be reached by any mean based algorithm.



\end{proof}

\esh{Add proof in the appendix, there is an email thread/ piece of python code with the counterex}


\subsection{Characterization of Pareto-Optimal No Regret Algorithms} 
A no-regret algorithm is pareto-optimal if and only if, over most games, its menu has the same set of minimum value points as some no-swap regret algorithm.

Proof of Theorem~\ref{thm:pareto_optimal_nr_char}:
\begin{proof}
First, we will prove that every no-regret menu $\M$ that has the same set of minimum value points as $P_{NSR}$ is pareto-optimal. To do so, we will consider any other menu $\bar{\M}$ and show that $\bar{\M}$ does not pareto-dominate $\M$, considering three cases:

\begin{itemize}
\item $U^{-}(\bar{\M}) < U^{-}(\M)$. Let $u_{O} = -u_{L}$. Then, 
\begin{align*}
& V_{L}(\bar{\M}, u_{O}) = \max\{u_{L}(\varphi)| \varphi \in \argmax_{\varphi \in \bar{\M}} -u_{L}(\varphi)\} \\
& = \max\{u_{L}(\varphi)| \varphi \in \argmin_{\varphi \in \bar{\M}} u_{L}(\varphi)\} \\
& = U^{-}(\bar{\M}) \\
\end{align*}

By the same logic,  $V_{L}(\M, -u_{L}) = U^{-}(\M)$. Therefore, this implies that $V_{L}(\bar{\M}, -u_{L}) < V_{L}(\M, -u_{L})$, so $\bar{M}$ does not dominate $\M$.

\item $U^{-}(\bar{\M}) > U^{-}(\M)$. This is not possible, as the Leader cannot guarantee a value above their maxmin distribution.

\item $U^{-}(\bar{\M}) = U^{-}(\M)$. Then, by Lemma~\ref{lem:menu-min-set}, $\M^{-} \subseteq \bar{\M}^{-}$. Recall also that $\M$ and $\bar{M}$ are distinct. Therefore, by Lemma~\ref{lem:non-dominance}, $\bar{\M}$ does not dominate $\M$.
\end{itemize}

Now, we will show that if a no-regret menu $M$ does not have same set of minimum value points as some no-swap regret menu, it is pareto-dominated by some other menu. Note that, by Lemma~\ref{lem:menu-min-value}, $U(\M)^{-} = U_{ZS}$. Furthermore, by the minimality of $U_{NSR}^{-}$ shown in Lemma~\ref{lem:menu-min-set}, $U_{NSR}^{-} \subseteq U(\M)^{-}$. Therefore, if $U_{NSR}^{-} \neq U(\M)^{-}$, then $U_{NSR}^{-} \subsetneq U(\M)^{-}$. Thus, there exists some extreme point $p \in \M^{-}$ which is not in $\M_{NSR}^{-}$. 

Now, let us consider the following menu $\bar{M}$: it is the convex hull of all extreme points in $\M_{NSR}$ and all extreme points in $\M$, excluding $p$. By Lemma INSERT, this is a valid menu. Note that $\bar{\M}$ has all the same extreme points of $\M$ except for $p$.

We will show that $\bar{\M}$ pareto-dominates $\M$. To see this, note first that, by Lemma~\ref{lem:non-dominance}, there is some $u_{L}$ value such that $V_{L}(U_{\M},u_{L}) < V_{L}(U_{\bar{\M}},u_{L})$. Furthermore, for all other values of $u_{L}$, $V_{L}(U_{\M},u_{L}) \leq V_{L}(U_{\bar{\M}},u_{L})$. Also note that the set of extreme points that $\bar{\M}$ has is equal to those in $\M$ for all non-min-valued extreme points, and it has a strict subset of the min-valued points. 

For all possible $u_{L}$, there is some extreme point in $U_{\M}$ which the optimizer will choose. There are two cases:

\begin{itemize}
\item This extreme point is min-valued. Then $\bar{\M}$ can only be better.
\item This extreme point is not min-valued. Then $\bar{\M}$ also contains this point. If some point is the maximizing point on some menu $M$, it is also the maximizing point on any subset of this menu (which still contains that maximizing point). So then the menus both give the same value.
\end{itemize}

Therefore, $\bar{\M}$ pareto-dominates $\M$. This concludes our proof.
\end{proof}

Theorem~\ref{theorem:all_about_nsr} follows directly from Theorem~\ref{thm:pareto_optimal_nr_char}. 


==> old/pareto_optimal_menus_old.tex <==
\section{Pareto-Optimal Asymptotic Menus}
\label{sec:pareto-optimal-menus}

In this section we shift our attention to understanding which asymptotic menus are Pareto-optimal and which are Pareto-dominated by other asymptotic menus. Our main goal will be a characterization of all Pareto-optimal no-regret asymptotic menus (which will set up the framework for proving that multiplicative weights is sometimes Pareto-dominated in Section \ref{sec:mean_based_pareto_dominated}). 

\subsection{Constraints on learner utilities}

We begin with some simple observations on the possible utilities of the learner under Pareto-optimal menus and no-regret menus. For any menu $\M$, let $\Up(\M) = \max_{\csp \in \M} u_{L}(\csp)$ denote the maximum learner payoff of any CSP in $\M$; likewise, define $\Um(\M) = \min_{\csp \in \M} u_{L}(\csp)$. We will also let $\M^{+} = \argmax_{\csp \in \M} u_{L}(\csp)$ and $\M^{-} = \argmin_{\csp \in \M} u_{L}(\csp)$ be the subsets of $\M$ that attain this maximum and minimum.

We first consider $\M^{+}$. Recall that, by assumption, there is a unique pure strategy profile $(i^{*}, j^{*})$ that maximizes the learner's reward. Let $\csp^{+}$ be the CSP corresponding to this strategy profile (so $\csp^{+}$ maximizes $u_{L}(\csp)$ over all CSPs in $\Delta_{mn}$). We claim that any Pareto-optimal menu must contain $\csp^{+}$.

\begin{lemma}\label{lem:has_max_point}
If $\M$ is a Pareto-optimal asymptotic menu, then $\M^{+} = \{\csp^{+}\}$.
\end{lemma}
\begin{proof}
\jon{if $\csp^{+} \not\in \M$, add it}
\end{proof}

We now consider $\M^{-}$. Unlike for $\M^{+}$, it is no longer the case that all Pareto-optimal menus share the same set $\M^{-}$. It is not even the case (as we shall see in Section \ref{sec:other-pareto}, that all Pareto-optimal menus have the same minimum learner utility $\Um(\M)$. 

However, it is the case that all \emph{no-regret} algorithms share the same value for the minimum learner utility $\Um(\M)$, namely $\Uzs = \Um(\M_{NR})$. The reason for this is that $\Uzs$ is also the largest utility the learner can guarantee when playing a zero-sum game (i.e., when the optimizer has payoffs $u_{O} = -u_{L}$), and thus it is impossible to obtain a higher value of $\Um(\M)$. This is formalized in the following lemma.

\begin{lemma}\label{lem:menu-min-value}
If $\M$ is a no-regret asymptotic menu, then $\Um(\M) = \Uzs$. Moreover, every asymptotic menu must have $\Um(\M) \leq \Uzs$.  
\end{lemma}
\begin{proof}
\jon{Theorem \ref{thm:nr_nsr_containment} shows one direction; thinking about the NE of the ZSG shows the other.}
\end{proof}

Unlike $\M^{+}$ which is always equal to $\{\csp^{+}\}$ for Pareto-optimal menus, the minimizing set $\M^{-}$ is not uniquely defined and may contain many CSPs. However, there is a ``minimal'' minimizing set $\M^{-}$ for no-regret menus: for any such menu $\M^{-}$ must contain $\M_{NSR}^{-}$. In fact, this is true for the slightly larger class of menus with $\Um(\M) = \Uzs$. 

\begin{lemma}\label{lem:menu-min-set}
Let $\M$ be an asymptotic menu with $\Um(\M) = \Uzs$. Then $\M_{NSR}^{-} \subseteq \M^{-}$.
\end{lemma}
\begin{proof}
\jon{look at what extreme points lie in $\M^{-}$}

Let $D_{m}$ be the set of distributions $x \in \Delta_{m}$ such that $u_{L}(x,\BR_{L}(x)) = \Uzs$. In other words, $D_{m}$ is the set of minmax distributions. First, we claim that all points of the form $u_{L}(x,\BR_{L}(x))$ where $x \in D_{m}$ must be in $\M^{-}$. Assume for contradiction that this is not the case. Then, if an optimizer chooses to play the distribution $x \in D_{m}$ in each round for the entire game, then the


By Lemma~\ref{lem:nsr_characterization}, all extreme points of $\M_{NSR}^{-}$ must be of the form $x \otimes y$, with $x \in \Delta_{m}$ and $y \in \BR_{L}(x)$. Furthermore, by definition, for all points in $\M^{-}$, $u_{L}(x \otimes y) = \Uzs$. 

Thus, to prove this lemma, we must simply show that 

\end{proof}

\subsection{Characterizing Pareto-optimal no-regret menus}

In this section, we provide a complete characterization of all Pareto-optimal no-regret menus. We state this characterization below.

\begin{theorem}\label{thm:characterization}
A no-regret asymptotic menu $\M$ is Pareto-optimal iff it satisfies the following two conditions:

\begin{enumerate}
    \item $\M^{+} = \{\csp^{+}\}$. \nat{This is already true based on the algoritm being no-regret}
    \item $\M$ cannot be written as a convex combination $\M = \conv(\M', Z)$ where $\M' \subset \M$ is an asymptotic menu strictly contained within $\M$, and $Z \subseteq \Delta_{mn}$ is any convex set of CSPs that satisfies $u_L(\csp) = \Uzs$ for any $\csp \in Z$.
\end{enumerate}
\end{theorem}

An asymptotic menu $\M$ is a \emph{polytopal menu} if the set $\M$ is a polytope (i.e., can be written as the convex hull of finitely many vertices). For example, note that $\M_{NSR}$ and $\M_{NR}$ are both polytopal menus as they are defined by finitely many linear constraints. For polytopal menus, the characterization of Theorem \ref{thm:characterization} simplifies considerably: a polytopal menu is Pareto-optimal iff it has the same maximal and minimal sets as the no-swap-regret menu $\M_{NSR}$.

\begin{theorem}\label{thm:characterization_polytope}
A no-regret polytopal menu $\M$ is Pareto-optimal iff $\M^{+} = \M_{NSR}^{+}$ ($= \{\csp^{+}\}$) and $\M^{-} = \M^{-}_{NSR}$.
\end{theorem}

We will prove Theorems \ref{thm:characterization} and \ref{thm:characterization_polytope} through a sequence of lemmas describing under what conditions a menu $\M_1$ can Pareto-dominate a menu $\M_2$. The most significant piece of the proof is the following lemma, which states that a menu cannot be Pareto-dominated by a menu with a larger minimal set $\M^{-}$.

\begin{lemma}\label{lem:non-dominance}
Let $\M_1$ and $\M_2$ be two distinct asymptotic menus where $\M_{1}^{+} = \M_{2}^{+}$, and $\M_{1}^{-} \subseteq \M_{2}^{-}$. Then there exists a $u_O$ for which $V_{L}(\M_1, u_O) > V_{L}(\M_2, u_O)$ (i.e., $\M_2$ does not Pareto-dominate $\M_1$).
\end{lemma}

Note that Lemma \ref{lem:non-dominance} holds even in the case where $\M_{1}^{-} = \M_{2}^{-}$. One important consequence of this is that all menus with the same value of $\M^{-}$ and $\M^{+}$ are incomparable to each other under the Pareto-dominance order.

The key technical ingredient for proving Lemma \ref{lem:non-dominance} is the following lemma, which establishes a ``two-dimensional'' variant of the above claim.

\begin{lemma}\label{lem:geometry}
Let $f, g: [a, b] \rightarrow \mathbb{R}$ be two distinct concave functions satisfying $f(a) \leq g(a)$ and $f(b) = g(b)$. For $\theta \in [0, \pi]$, let $\hat{f}(\theta) = \argmax_{x \in [0, 1]} (x\cos\theta + f(x)\sin\theta)$ (if the argmax is not unique, then $\hat{f}(\theta)$ is undefined). Define $\hat{g}(\theta)$ symmetrically. Then there exists a $\theta$ for which $\hat{f}(\theta) > \hat{g}(\theta)$.
\end{lemma}
\begin{proof}
Since $f(x)$ is a concave curve, it has a (weakly) monotonically decreasing derivative $f'(x)$. This derivative is not necessarily defined for all $x \in [a, b]$, but since $f$ is concave it is defined almost everywhere. At points $c$ where it is not defined, $f$ still has a well-defined left derivative $f'_L(x) = \lim_{h \rightarrow 0} (f(x) - f(x - h))/h$ and right derivative $f'_R(x) = \lim_{h \rightarrow 0} (f(x + h) - f(x))/h$. We will abuse notation and let $f'(x)$ to denote the interval $[f'_L(x), f'_R(x)]$ (at the boundaries defining $f'(a) = (-\infty, f_{R}(a)]$ and $f'(b) = [f_{L}(b), \infty)$. Similarly, the interval-valued inverse function $(f')^{-1}(y)$ is also well-defined, decreasing in $y$, and uniquely-defined for almost all values of $y$ in $(-\infty, \infty)$. 

Note that since $\hat{f}(\theta)$ is the $x$ coordinate of the point on the curve $f(x)$ that maximizes the inner product with the unit vector $(\cos\theta, \sin\theta)$, $f'(\hat{f}(\theta))$ must contain the value $-\cos\theta / \sin\theta = -\cot \theta$. In particular, if $\hat{f}(\theta)$ is uniquely defined, $\hat{f}(\theta) = (f')^{-1}(-\cot \theta)$. So it suffices to find a $y$ for which $(f')^{-1}(y) > (g')^{-1}(y)$. 

To do this, we make the following observation: since $f(b) - f(a) \geq g(b) - g(a)$, $\int_{a}^{b} f'(x)dx \geq \int_{a}^{b} g'(x)dx$. This means there must be a point $c \in (a, b)$ where $f'(c) > g'(c)$. If not, then we must have $f'(x) \leq g'(x)$ for all $x \in (a, b)$; but the only way we can simultaneously have $f'(x) \leq g'(x)$ for all $x \in (a, b)$ and $\int_{a}^{b}f'(x)dx \geq \int_{a}^{b}g'(x)dx$ is if $f'(x) = g'(x)$ for almost all $x \in (a, b)$ -- but this would contradict the fact that $f$ and $g$ are distinct concave functions. 

Now, take a point $c \in (a, b)$ where $f'(c) > g'(c)$ and choose a $y$ in $f'(c)$. Since $g'$ is a decreasing function, there must exist a $c' < c$ such that $y \in g'(c')$, and so $(f')^{-1}(y) > (g')^{-1}(y)$. 
\end{proof}

We can now prove Lemma \ref{lem:non-dominance}. \jon{this proof might be a good candidate for a diagram}

\begin{proof}[Proof of Lemma~\ref{lem:non-dominance}]
Since $\M_1$ and $\M_2$ are distinct asymptotic menus, there must be an extreme point $\csp$ in one menu that does not belong to the other. In particular, there must exist an optimizer payoff $u_{O}$ where $u_{O}(\csp) > u_{O}(\csp')$ for any $\csp'$ in the other menu. Denote this specific optimizer payoff by $u_{O}^{0}$.

We will show that there exists a $u_{O} \in \mathrm{span}(u_L, u_{O}^{0})$ where $V_{L}(\M_1, u_O) > V_{L}(\M_2, u_O)$. To do this, we will project $\M_1$ and $\M_2$ to two-dimensional sets $S_1$ and $S_{2}$ by letting $S_{1} = \{(u_L(\csp), u_{O}^{0}(\csp)) \mid \csp \in \M_1 \}$ (and defining $S_{2}$ symmetrically). By our construction of $u_{O}^{0}$, these two convex sets $S_{1}$ and $S_{2}$ are distinct. Also, note that if $u_O = \lambda_{1}u_L + \lambda_{2}u_{O}^{0}$, we can interpret $V_{L}(\M_1, u_O)$ as the maximum value of $z_1$ for any point in $\arg\max_{(z_1, z_2) \in S_1} (\lambda_1z_1 + \lambda_2z_2)$. We can interpret $V_{L}(\M_2, u_O)$ similarly.

Let us now consider the geometry of $S_1$ and $S_2$. Let $u^{-}$ denote the common value of $\Um(\M_1)$ and $\Um(\M_2)$, and similarly, let $u^{+}$ denote the common value of $\Up(\M_1)$ and $\Up(\M_2)$. Both $S_1$ and $S_2$ are contained in the ``vertical'' strip $u^{-} \leq z_1 \leq u^{+}$. We can therefore write $S_1$ as the region between the concave curve $f_{\text{up}}:[u^{-}, u^{+}]$ (representing the upper convex hull of $S_1$) and $f_{\text{down}}$ (representing the lower convex hull of $S_1$; define $g_{\text{up}}$ and $g_{\text{down}}$ analogously for $S_2$. Since $S_1$ and $S_2$ are distinct, either $f_{\text{up}} \neq g_{\text{up}}$ or $f_{\text{down}} \neq g_{\text{down}}$; without loss of generality, assume $f_{\text{up}} \neq g_{\text{up}}$ (we can switch the upper and lower curves by changing $u_{O}^{0}$ to $-u_{O}^{0}$).

Note also that since $\M^{+}_1 = \M^{+}_2$ and $\M^{-}_1 \subseteq \M^{-}_2$, we have $f_{\text{up}}(u^{+}) = g_{\text{up}}(u^{+})$ and $f_{\text{up}}(u^{-}) \leq g_{\text{up}}(u^{-})$ (since $[f_{\text{down}}(u^{-}), f_{\text{up}}(u^{-})] \subseteq [g_{\text{down}}(u^{-}), g_{\text{up}}(u^{-})]$). By Lemma \ref{lem:geometry}, there exists a $\theta \in [0, 2\pi]$ for which $\hat{f}_{\text{up}}(\theta) > \hat{g}_{\text{up}}(\theta)$. But by the definition of $\hat{f}$ and $\hat{g}$, this implies that for $u_{O} = \cos(\theta) u_L + \sin(\theta) u^{0}_{O}$, $V_{L}(\M_1, u_{O}) > V_{L}(\M_2, u_O)$, as desired. 
\end{proof}

Lemma \ref{lem:non-dominance} will be important for proving that menus satisfying the characterization of Theorem \ref{thm:characterization} are all Pareto-optimal. To prove that menus violating the characterization are Pareto-dominated, we will need the following lemma.

\begin{lemma}\label{lem:min-set-dominance}
Let $\M_1$ be an asymptotic menu, and let $\M_2 = \conv(\M_1, Z)$, where $Z$ is a convex set of CSPs with the property that every $\csp \in Z$ satisfies $u_L(\csp) = \Um(\M_1)$. Then if $\M_2 \neq \M_1$, $\M_2$ is Pareto-dominated by $\M_1$. 
\end{lemma}
\begin{proof}
\jon{Insert. this probably exists in some form somewhere already?}
\end{proof}

We can now prove our main characterization theorem.

\begin{proof}[Proof of Theorem~\ref{thm:characterization}]
We will start by showing that any no-regret menu that does not satisfy these two constraints must be Pareto-dominated. Any menu that violates the first constraint is Pareto-dominated as a consequence of Lemma \ref{lem:has_max_point}. Any menu that violates the second constraint is Pareto-dominated as a direct consequence of Lemma \ref{lem:min-set-dominance}.

We now must show that all other no-regret menus are Pareto-optimal. We will begin by showing that all menus with $\M^{-} = \M_{NSR}^{-}$ and $\M^{+} = \{\csp^{+}\}$ are Pareto-optimal. To see that these menus satisfy the conditions of the characterization, note that for every no-regret menu $\M$, $\M^{-}$ must contain $\M_{NSR}^{-}$ (Lemma \ref{lem:menu-min-set}). In particular, if $\M^{-} = \M_{NSR}^{-}$, then there is no way to write $\M$ in the form $\conv(\M', Z)$ for a no-regret $\M' \subset \M$ and $Z \subseteq u_{L}^{-1}(\Uzs)$. 

Now, consider such a menu $\M$ and assume to the contrary it is Pareto-dominated by some other asymptotic menu $\M'$. Without loss of generality, it suffices to only consider Pareto-optimal $\M'$, so we can assume $(\M')^{+} = \{\csp^{+}\}$. If $\Um(\M') < \Uzs$, then $\M$ cannot be Pareto-dominated by $\M'$ (since $V_{L}(\M, -u_L) = \Uzs > V_{L}(\M', -u_L)$). By Lemma \ref{lem:menu-min-value}, we must therefore have that $\Um(\M') = \Uzs$. By Lemma \ref{lem:menu-min-set}, this implies that $\M^{-} = \M_{NSR}^{-} \subseteq (\M')^{-}$. But now, by Lemma \ref{lem:non-dominance}, $\M'$ does not Pareto-dominate $\M$, establishing a contradiction.

\jon{todo: handle the removable case (might be annoying)}
\end{proof}

\subsection{Other Pareto-optimal algorithms}
\label{sec:other-pareto}

The previous sections have been concerned with Pareto-optimal \emph{no-regret} menus. This raises the obvious question: do there exist learning algorithms that incur high regret and yet are still Pareto-optimal? The following lemma shows this is the case.

\begin{lemma}
The learner algorithm which always plays the move $l$ associated with $L+ = (l, o)$ is Pareto-optimal. \jon{restate this lemma so it is about a menu}
\end{lemma}
\begin{proof}
\jon{todo: update proof}
Call the algorithm described above $A$. Consider any algorithm $B$ which outperforms $A$ on some game $G = (\mu_{\mathcal{L}},\mu_{\mathcal{O}})$. This must mean that $B$ induces a different menu given $\mu_{\mathcal{L}}$. Note that the extreme points of the menu of $A$, $M_{A}$, are $m$ unit vectors, corresponding to the move pair dimensions $(l,k)$ $\forall k \in [m]$. $M_{B}$ is not a strict subset of $M_A$. Assume for contradiction that it is a strict subset. Then one of the extreme points of $M_{A}$ is not present in $M_{B}$, w.l.o.g. the point that just consists of the move $(l,k)$. Then if the optimizer chooses to just play $k$ against $B$, the learner cannot only play $l$. So there must be some extreme point with some fraction of the move pair $(r,k)$ for some other learner move $r$. But this extreme point is not within $M_{A}$, leading to a contradiction. Thus $M_{B}$ is not a strict subset of $M_{A}$. Since it must be different from $M_{A}$, there must be an extreme point in $M_{B}$ which is not anywhere in $M_{A}$. Call this point $x$.   \\

Now, we will construct a game $G'$ where $A$ outperforms $B$. Let $\mu'_{\mathcal{L}} = \mu_{\mathcal{L}}$, so that $A$ and $B$ still induce the same menus. Now, consider $x$. Select the move pair dimension in $x$ which is the most frequent, and which does not involve $l$. Call this move pair $(i,j)$, $i \neq l$, and let $\frac{1}{c}$ be the fraction of the time that $(i,j)$ is played in $x$. This fraction must exist, as $x$ is not in the convex hull of $M_{A}$'s extreme points. Now, set $\mu'_{\mathcal{O}}(i,j) = 2$. Set $\mu'_{\mathcal{O}}(l, o) = \frac{1}{c}$ (or something below this that is above 0, or really 0 if we are ok with tiebreaking in learner's favor). The rest of $\mu'_{\mathcal{O}}$ will be set to $0$. \\

Now, consider how $A$ and $B$ will perform on this game. Recall that their menus will be unchanged on $G'$ from $G$. In $M_{A}$, there are no points involving $(i,j)$ at all. Thus the optimizer must choose between getting $\frac{1}{c}$ with $L+$ or getting $0$. They will choose to play $L+$ and the learner gets their max value. \\

In $M_{B}$, $x$ is in the menu. The payoff of $x$ for the optimizer is at least $\frac{1}{c} \cdot 2 = \frac{2}{c}$. This is a larger payoff for the optimizer than playing $L+$. Therefore $L+$ is not the max-payoff point for the optimizer in the menu, so the learner will not get $L+$. Thus, this is a game where algorithm $A$ is strictly better for the learner than algorithm $B$. 
\end{proof}

\begin{corollary}
There exists a learning algorithm $\cA$ that is not no-regret, but whose asymptotic menu $\M(\cA)$ is Pareto-optimal.
\end{corollary}


% \subsection{OLD}

% \jon{Do we want to include this other example? Not sure if they are useful for our story.}
% \nat{Might be worth putting in appendix--I think it works for the story, because we're saying, no regret algorithms aren't necessarily pareto optimal and pareto optimal algorithms aren't necessarily no regret. But there are algorithms that are both.}

% \begin{lemma}
% The learner algorithm which tries the move $l$ associated with $L+ = (l, o)$ and otherwise plays another constant move $k$ forever is pareto-optimal. 
% \end{lemma}
% \begin{proof} (informal)
% Call the algorithm described above $A$. Consider any algorithm $B$ which outperforms $A$ on some game $G = (\mu_{\mathcal{L}},\mu_{\mathcal{O}})$. This must mean that $B$ induces a different menu given $\mu_{\mathcal{L}}$. Note that the extreme points of the menu of $A$, $M_{A}$, are $m$ unit vectors, corresponding to the move pair dimensions $(k,j)$ $\forall j \in [m]$, and also the unit vector with only the move pair $(l,o)$. $M_{B}$ is not a strict subset of $M_A$. If it were, then by Lemma~\ref{lem:minimal}, it must not contain $L+$, and in this case it certainly cannot pareto-dominate $A$.

% So there must be some extreme point in $M_{B}$ which is not anywhere in $M_{A}$. Call this point $x$.   \\

% Now, we will construct a game $G'$ where $A$ outperforms $B$. Let $\mu'_{\mathcal{L}} = \mu_{\mathcal{L}}$, so that $A$ and $B$ still induce the same menus. Now, consider $x$. Select the move pair dimension in $x$ which is the most frequent, and which does not involve either the learner playing $k$ or the move pair $(l,o)$. Call this move pair $(i,j)$. Let $\frac{1}{c}$ be the fraction of the time that $(i,j)$ is played in $x$. This fraction must exist, as $x$ is not in the convex hull of $M_{A}$'s extreme points. Now, set $\mu'_{\mathcal{O}}(i,j) = 2$. Set $\mu'_{\mathcal{O}}(l, o) = \frac{1}{c}$ (or something below this that is above 0, or really 0 if we are ok with tiebreaking in learner's favor). The rest of $\mu'_{\mathcal{O}}$ will be set to $0$. \\

% Now, consider how $A$ and $B$ will perform on this game. Recall that their menus will be unchanged on $G'$ from $G$. In $M_{A}$, there are no points involving $(i,j)$ at all. Thus the optimizer must choose between getting $\frac{1}{c}$ with $L+$ or getting $0$. They will choose to play $L+$ and the learner gets their max value. \\

% In $M_{B}$, $x$ is in the menu. The payoff of $x$ for the optimizer is at least $\frac{1}{c} \cdot 2 = \frac{2}{c}$. This is a larger payoff for the optimizer than playing $L+$. Therefore $L+$ is not the max-payoff point for the optimizer in the menu, so the learner will not get $L+$. Thus, this is a game where algorithm $A$ is strictly better for the learner than algorithm $B$. 
% \end{proof}

% \begin{lemma}
% \label{lem:Lplus}
%     Consider any algorithm, which on some learner payoff $\mu_{\mathcal{L}}$, does not have $L+$ in its menu. Then this algorithm is pareto-dominated.
% \end{lemma}

% \begin{lemma}
% Given an algorithm generating a family $\{M(\mu_{\mathcal{L}})\}$ of menus (over leader payoffs), 
% \begin{enumerate}
%     \item There exists an algorithm that generates menus $\text{Conv}(\mu_{\mathcal{L}} \cup L_+(\mu_{\mathcal{L}}))$
%     \item There may not always exist an algorithm generating menus  $\{M(\mu_{\mathcal{L}})\} \cup \text{minimax}(\{M(\mu_{\mathcal{L}})\})$ where $\text{minimax}(\{M(\mu_{\mathcal{L}})\})$ refers to all distributions over action pairs achieving at least the minimax value.
% \end{enumerate}
% \end{lemma}

% \noindent
% \begin{lemma}
% \begin{enumerate}
% Consider any two algorithms $A$ and $B$ where, on all $\mu_{\mathcal{L}}$, $M_{A} \subseteq M_{B}$,
%     \item  If on at least one $\mu_{\mathcal{L}}$, $M_{A} \subsetneq M_{B}$ and $M_{B} \backslash M_{A}$ contains only points with learner value less than the min learner value in $M_{A}$; Then, $M_{B}$ is pareto dominated by $M_{A}$.
%     \item   If on at least one $\mu_{\mathcal{L}}$, $M_{A} \subsetneq M_{B}$ and $M_{B} \backslash M_{A}$ contains only points with learner value greater than the max learner value in $M_{A}$; Then, $M_{A}$ is pareto dominated by $M_{B}$.
% \end{enumerate}
% \end{lemma}



% \begin{lemma}
% \label{lem:minmin}
%     Consider any two algorithms $A$ and $B$ where, on some $\mu_{\mathcal{L}}$, the min learner value of $M_{B}$ is less than the min learner value of $M_{A}$. Then, $M_{B}$ does not dominate $M_{A}$.
% \end{lemma}

% \begin{lemma}
% \label{lem:maxmax}
%     Consider any two algorithms $A$ and $B$ where, on some $\mu_{\mathcal{L}}$, the max learner value of $M_{B}$ is greater than the max learner value of $M_{A}$. Then, $M_{A}$ does not dominate $M_{B}$.
% \end{lemma}


% \esh{------------------------------------------------------------------x-------------------------------------------------}

% \esh{The critical path begins here}
% \begin{definition}
%     Consider some polytope with a set $T$ of extreme points. For any $x \in T$, let $y$ be a neighbor to $x$ if there exists a direction such that $x$ and $y$ are the sole maximizers in $T$. Equivalently, $x,y \in T$ are said to be neighbours if $Conv(x,y)$ is a $1$-face of the polytope.  We use the notation $N(x)$ to denote the set of neighbors of the extreme point $x$.
% \end{definition}



% \begin{lemma}
% \label{lem:path}
% Consider some polytope with a set $T$ of extreme points, and some vector $v$. For any $x \in T$, if $<x,v>$ is no larger than $ <p,v>$ for all $p \in N(x)$, then $<x,v>$ is no larger than $<t,v>$ for all $t \in T$. Furthermore, if $<x,v>$ is no smaller than $<p,v>$ for all $p \in N(x)$, then $<x,v>$ is no smaller than $<t,v>$ for all $t \in T$.  
% \end{lemma}


% \begin{proof}
%     \esh{A polytope is spanned by the neighbouring edges of any vertex}

%     \esh{https://math.stackexchange.com/questions/3807208/how-to-show-that-any-polytope-p-is-spanned-by-the-neighboring-edges-of-any-ver}
% \end{proof}

% \esh{I think this result with the proof below works for non-polytope menus as well}
% \begin{lemma}
% \label{lemma:unique_points_preserved}
%     Consider two algorithms $A$ and $B$ that induce %polytope 
%     menus $M_A$ and $M_B$ respectively for some leader payoff $\mu_{\mathcal{L}}$ with menu $M_A$ containing an extreme point $X$ that is not a part of $M_B$. Let $C$ be the convex hull of the union of $A$ and $B$. Then, either $X$ is an 
%  extreme point of $C$ or $C$ contains two extreme points $X'$ and $Y'$ such that $X' \in M_A \setminus M_B$ and $Y' \in M_B\setminus M_A $ (note that they would automatically be extreme points of $M_A$ and $M_B$ respectively). 
% \end{lemma}  

% \begin{proof}
%    Let $T_A$ ($T_B$) denote the set of extreme points of $M_A$ ($M_B$) that are not a point of $M_B$ ($M_A$). Thus, $X \in T_A$. Let $T$ denote the extreme points of $C$. Either $X \in T$ or $X \notin T$. We only need to consider the second case. In this case, $X$ can be written as a convex combination of extreme points of $C$ - let $T' \subset T$ be a minimal set of extreme points of $C$ such that $X$ can be written as a convex combination of points in $T'$. Since $X$ is not an extreme point of $C$, $X \notin T'$.  It suffices to prove that $T' \cap T_A \ne \phi$ and $T' \cap T_B \ne \phi$, since these results would directly imply a point each from $T_A$ and $T_B$ among the extreme points of $C$ (since $T' \subseteq T$). 
   
%    First, to show $T' \cap T_A \ne \phi$, we assume otherwise, which would imply that all the points in $T'$ are extreme points of $M_B$ (since each extreme point of $C$ is either an extreme point of $M_A$ or $M_B$ or both). Thus, $X$ can be written as a convex combination of extreme points of $M_B$, implying that $ X \in M_B$, which is a contradiction, therefore invalidating the assumption.

%    For the proof of $T' \cap T_B \ne \phi$, we again attempt to find a contradiction by assuming that this is not true. This implies that $X$ can be written as a convex combination of extreme points of $M_A$ excluding $X$ (since $X \notin T'$). This is a contradiction, since we started with $X$ being an extreme point of $M_A$.
% \end{proof}


% \begin{lemma}
% \label{Abetter}
% Consider two algorithms $A$ and $B$ producing polytope menus $M_{A}$ and $M_{B}$ accordingly, and the convex hull of their extreme points $C$. If there are two neighboring extreme points $a$ and $b$ in $C$ such that $a$ is not contained within $M_{B}$, $b$ is an extreme point of $M_{B}$, and $\langle b, \mu_{\mathcal{L}} \rangle < \langle a, \mu_{\mathcal{L}} \rangle$, then $A$ outperforms $B$ on a positive measure set of optimizer payoffs.%games.  
% \end{lemma}

% \begin{proof}
% %\esh{Add reasoning for +ve measure}

% As $a$ and $b$ are neighboring points, there is some direction $d$ for which they are both maximizers in $C$ and no other extreme point is a maximizer. Note that this means that $b$ is the unique maximizing point under $d$ in $M_{B}$ and $(a,b)$ is the unique pair of maximizing points under $d$ in $M_{A}$. Let $\epsilon$ be the smallest difference between $\langle b,d \rangle $ and $\langle x,d \rangle$, where $x$ is any extreme point in $M_{B}$ or $M_{A}$ other than $b$ or $a$ (note that this may include points that are not extreme points of $C$). This quantity $\varepsilon$ is well defined and positive since the polytope menus have a finite set of extreme points. Furthermore, let $R$ be the highest absolute value learner value achievable in $\mu_{\mathcal{L}}$. Then, let us consider the direction $d' = d + \frac{\epsilon}{4R} \cdot \mu_{\mathcal{L}}$. 

% Note that for any extreme point $p$ in $M_{A}$ or $M_{B}$, we can upper bound the change in their value between $d'$ and $d$:

% \begin{align*}
% |\langle p,d' \rangle - \langle p,d \rangle | &= |\langle p,d'-d \rangle| = |\langle p,\frac{\epsilon}{4 R} \cdot \mu_{\mathcal{L}} \rangle|\\  &= \frac{\epsilon}{4 R} \cdot |\langle p,\mu_{\mathcal{L}} \rangle | 
% \leq \frac{\epsilon}{4 R} \cdot R = \frac{\epsilon}{4}
% \end{align*}

% Thus, when going from $d$ to $d'$, every extreme point's value can change by at most $\frac{\epsilon}{4}$. Since all extreme points in $M_{A}$ and $M_{B}$ are $\epsilon$-separated from $a$ and $b$ under $d$, they are still all $\frac{\epsilon}{2}$-separated from them under $d'$. So in $M_{A}$ and $M_{B}$, the only candidates left to consider for maximizing points under $d'$ are $a$ and $b$. In $M_{B}$, there is no $a$, so the maximizing point is $b$.

% However, in $M_{A}$, the maximizing point is $a$. Note that $\langle a,d' \rangle > \langle b,d' \rangle $, because 

% \begin{align*}
% \langle a,d' \rangle - \langle b,d' \rangle  = 
% \frac{\epsilon}{4 R} (\langle a, \mu_{\mathcal{L}} \rangle - \langle b,\mu_{\mathcal{L}} \rangle) 
% > 0 \tag{By $\langle a, \mu_{\mathcal{L}} \rangle > \langle b, \mu_{\mathcal{L}} \rangle$}
% \end{align*}


% This means that, under the optimizer payoff vector $\mu_{\mathcal{O}} = d'$, the optimizer would pick the point $a$ under $M_{A}$ and $b$ under $M_{B}$. As the $\mu_{\mathcal{L}}$ value of $a$ is greater than that of $b$, $M_{A}$ performs better under $d'$ than $M_{B}$.  A similar construction can be used for any smaller, positive value of $\varepsilon$, giving us a positive measure set of optimizer payoffs that satisfy where $A$ outperforms $B$.

% \end{proof}

% \esh{Verified upto here}
% \begin{lemma}
% \label{Bbetterconvex}

% \nat{new approach: pick the max-valued blue extreme point. if this is well defined, use the edge argument. if iut's not well-defined, you can just wiggle around the uL value by epsilon.}
% Consider two algorithms $A$ and $B$ producing menus $M_{A}$ and $M_{B}$ accordingly, where $M_{B}$ is a polytope, and the convex hull of the menus is $C$. If there exists a point $b$ on $C$ such that $b$ is an extreme point of $M_{B}$, and some direction $j$ and value $\epsilon$ such that for all maximizing points on the convex hull
% $a$ is not contained within $M_{B}$, $\langle b, \mu_{\mathcal{L}} \rangle > \langle a, \mu_{\mathcal{L}} \rangle$, and there exists a path along the surface of $C$ from $a$ to $b$ such that $\mu_{\mathcal{L}}$ strictly increases, then $B$ outperforms $A$ on some games.  
% \end{lemma}

% \begin{proof}
% As $a$ and $b$ are neighboring points, there is some direction $d$ for which they are both maximizers in $C$ and no other extreme point is a maximizer. Note that this means that $b$ is the unique maximizing point under $d$ in $M_{B}$ and $(a,b)$ is the unique pair of maximizing points under $d$ in $M_{A}$. Let $\epsilon$ be the smallest difference between $\langle b,d \rangle $ and $\langle a,d \rangle$, where $x$ is any extreme point in $M_{B}$ or $M_{A}$ other than $b$ or $a$ (note that this may include points that are not extreme points of $C$). Furthermore, let $R$ be the highest absolute value learner value achievable in $\mu_{\mathcal{L}}$. 

% Then, let us consider the direction $d' = d - \frac{\epsilon}{4R} \cdot \mu_{\mathcal{L}}$. 

% Note that for any extreme point $p$ in $M_{A}$ or $M_{B}$, we can upper bound the change in their value between $d'$ and $d$:

% \begin{align*}
% |\langle p,d' \rangle - \langle p,d \rangle | = |\langle p,d'-d \rangle| \\
% = |\langle p,\frac{-\epsilon}{4 R} \cdot \mu_{\mathcal{L}} \rangle|\\  = \frac{\epsilon}{4 R} \cdot |\langle p,\mu_{\mathcal{L}} \rangle | \\
% \leq \frac{\epsilon}{4 R} \cdot R = \frac{\epsilon}{4}
% \end{align*}

% Thus, when going from $d$ to $d'$, every extreme point's value can change by at most $\frac{\epsilon}{4}$. Since all extreme points in $M_{A}$ and $M_{B}$ are $\epsilon$-separated from $a$ and $b$ under $d$, they are still all $\frac{\epsilon}{2}$-separated from them under $d'$. So in $M_{A}$ and $M_{B}$, the only candidates left to consider for maximizing points under $d'$ are $a$ and $b$. In $M_{B}$, there is no $a$, so the maximizing point is $b$.

% However, in $M_{A}$, the maximizing point is $a$. 
% Note that $\langle a,d' \rangle < \langle b,d' \rangle $, because 

% \begin{align*}
% \langle a,d' \rangle - \langle b,d' \rangle \\ = 
% -\frac{\epsilon}{4 R} (\langle a, \mu_{\mathcal{L}} \rangle - \langle b,\mu_{\mathcal{L}} \rangle) \\
% = 
% \frac{\epsilon}{4 R} (\langle b, \mu_{\mathcal{L}} \rangle - \langle a,\mu_{\mathcal{L}} \rangle) \\
% < 0 \tag{By $\langle a, \mu_{\mathcal{L}} \rangle > \langle b, \mu_{\mathcal{L}} \rangle$}
% \end{align*}

% This means that, under the optimizer payoff vector $\mu_{\mathcal{O}} = d'$, the optimizer would pick the point $a$ under $M_{A}$ and $b$ under $M_{B}$. As the $\mu_{\mathcal{L}}$ value of $a$ is less than that of $b$, $M_{A}$ performs worse under $d'$ than $M_{B}$. 

% \end{proof}


% \begin{lemma}
% \label{Bbetter}
% Consider two algorithms $A$ and $B$ producing polytope menus $M_{A}$ and $M_{B}$ accordingly, and the convex hull of their extreme points $C$. If there are two neighboring extreme points $a$ and $b$ in $C$ such that $a$ is not contained within $M_{B}$, $b$ is an extreme point of $M_{B}$, and $\langle b, \mu_{\mathcal{L}} \rangle > \langle a, \mu_{\mathcal{L}} \rangle$, then $B$ outperforms $A$ on some games.  
% \end{lemma}

% \begin{proof}
% As $a$ and $b$ are neighboring points, there is some direction $d$ for which they are both maximizers in $C$ and no other extreme point is a maximizer. Note that this means that $b$ is the unique maximizing point under $d$ in $M_{B}$ and $(a,b)$ is the unique pair of maximizing points under $d$ in $M_{A}$. Let $\epsilon$ be the smallest difference between $\langle b,d \rangle $ and $\langle a,d \rangle$, where $x$ is any extreme point in $M_{B}$ or $M_{A}$ other than $b$ or $a$ (note that this may include points that are not extreme points of $C$). Furthermore, let $R$ be the highest absolute value learner value achievable in $\mu_{\mathcal{L}}$. 

% Then, let us consider the direction $d' = d - \frac{\epsilon}{4R} \cdot \mu_{\mathcal{L}}$. 

% Note that for any extreme point $p$ in $M_{A}$ or $M_{B}$, we can upper bound the change in their value between $d'$ and $d$:

% \begin{align*}
% |\langle p,d' \rangle - \langle p,d \rangle | = |\langle p,d'-d \rangle| \\
% = |\langle p,\frac{-\epsilon}{4 R} \cdot \mu_{\mathcal{L}} \rangle|\\  = \frac{\epsilon}{4 R} \cdot |\langle p,\mu_{\mathcal{L}} \rangle | \\
% \leq \frac{\epsilon}{4 R} \cdot R = \frac{\epsilon}{4}
% \end{align*}

% Thus, when going from $d$ to $d'$, every extreme point's value can change by at most $\frac{\epsilon}{4}$. Since all extreme points in $M_{A}$ and $M_{B}$ are $\epsilon$-separated from $a$ and $b$ under $d$, they are still all $\frac{\epsilon}{2}$-separated from them under $d'$. So in $M_{A}$ and $M_{B}$, the only candidates left to consider for maximizing points under $d'$ are $a$ and $b$. In $M_{B}$, there is no $a$, so the maximizing point is $b$.

% However, in $M_{A}$, the maximizing point is $a$. 
% Note that $\langle a,d' \rangle < \langle b,d' \rangle $, because 

% \begin{align*}
% \langle a,d' \rangle - \langle b,d' \rangle \\ = 
% -\frac{\epsilon}{4 R} (\langle a, \mu_{\mathcal{L}} \rangle - \langle b,\mu_{\mathcal{L}} \rangle) \\
% = 
% \frac{\epsilon}{4 R} (\langle b, \mu_{\mathcal{L}} \rangle - \langle a,\mu_{\mathcal{L}} \rangle) \\
% < 0 \tag{By $\langle a, \mu_{\mathcal{L}} \rangle > \langle b, \mu_{\mathcal{L}} \rangle$}
% \end{align*}

% This means that, under the optimizer payoff vector $\mu_{\mathcal{O}} = d'$, the optimizer would pick the point $a$ under $M_{A}$ and $b$ under $M_{B}$. As the $\mu_{\mathcal{L}}$ value of $a$ is less than that of $b$, $M_{A}$ performs worse under $d'$ than $M_{B}$. 

% \end{proof}


% \begin{lemma}
% \label{lem:incomp}
%     Consider any two algorithms $A$ and $B$ which, on some $\mu_{\mathcal{L}}$, have polytope menus $M_{A}$ and $M_{B}$ with all max and min learner value points shared. If $M_{A}$ and $M_{B}$ differ on at least one extreme point, $A$ and $B$ are incomparable.
% \end{lemma}

% \begin{proof}
% As $M_{A}$ and $M_{B}$ differ on at least one extreme point and they share all their max and min learner valued points, there must be some extreme point in either $M_{A}$ or $M_{B}$ which gets the learner strictly between their max and min value and is not contained within the other menu. w.l.o.g. let $M_{A}$ contain an extreme point of this form.% , and call this extreme point $a^{*}$.

% Let the polytope $C$ be the convex hull of the union of the extreme points of $M_{A}$ and $M_{B}$. Thus, every extreme point in $C$ must be an extreme point of either $M_{A}$ or $M_{B}$. Let us label the extreme points of $C$ according to which menu they were originally from. If the extreme point is an extreme point in $M_{A}$ but not $M_{B}$, color it red. If it is an extreme point of both menus, or just an extreme point of $M_{B}$, color it blue.  

% Combining our assumption about $M_A$ containing a unique extreme point with Lemma~\ref{lemma:unique_points_preserved}, there must be at least one red point in $C$, $a^{*}$. We claim there is a path through neighboring points from $a^{*}$ to a min-valued learner point such that at each step, the $\mu_{\mathcal{L}}$ value strictly decreases. To see this, note that by Lemma~\ref{lem:path}, as long as the current point is not a minimizing point in the $\mu_{\mathcal{L}}$ direction, there is a way to pick a neighboring point with strictly smaller $\mu_{\mathcal{L}}$. Thus if we continue this process until it is impossible to pick a valid neighbor, we have reached a minimizing point, and the path we took from $a^{*}$ to this point always has strictly decreasing $\mu_{\mathcal{L}}$ value. Call this path $\mathcal{P}$.

% Note that all minimizing points are blue, and $a^{*}$ is red. Thus, when walking from $a^{*}$ to any minimizing point through $\mathcal{P}$, there must be some point of the path where we travel from a red point to a neighboring blue point. Let us call the red point here $r^{*}$ and the blue point $b^{*}$. By our construction of $\mathcal{P}$, it must be the case that $r^{*}$ has a strictly higher $\mu_{\mathcal{L}}$ value than $b^{*}$. Furthermore $r^{*}$ and $b^{*}$ are neighboring points where $r^{*}$ is not contained within $M_{B}$ and $b^{*}$ is an extreme point of $M_{B}$. Thus, by lemma~\ref{Abetter}, there are games where $A$ performs better than $B$.

% Now, we must prove there is a game where $M_{B}$ performs better. 

% We claim there is a path in $C$ through neighboring points from $a^{*}$ to a max-valued learner point such that at each step, the $\mu_{\mathcal{L}}$ value strictly increases. We can again use~\ref{lem:path} to prove this. Call this path $\mathcal{P}$.

% Note that all maximizing points are blue, and $a^{*}$ is red. Thus, when walking from $a^{*}$ to any maximizing point through $\mathcal{P}$, there must be some point of the path where we travel from a red point to a neighboring blue point. Let us call the red point here $r^{*}$ and the blue point $b^{*}$. By our construction of $\mathcal{P}$, it must be the case that $r^{*}$ has a strictly lower $\mu_{\mathcal{L}}$ value than $b^{*}$. Furthermore $r^{*}$ and $b^{*}$ are neighboring points where $r^{*}$ is not contained within $M_{B}$ and $b^{*}$ is an extreme point of $M_{B}$.. Thus, by lemma~\ref{Bbetter}, there are games where $B$ performs better than $A$. 

% As $A$ sometimes performs better than $B$ and $B$ sometimes performs better than $A$, the two algorithms are incomparable. 


% \end{proof}



 
 
 
 
 \begin{lemma}
 \label{lem:incomp}
     Consider any two algorithms $A$ and $B$ which, on some $\mu_{\mathcal{L}}$, have menus $M_{A}$ and $M_{B}$ where $M_{A}$ has some 
     extreme point which is not in $M_{B}$, and $M_{B}$ is a polytope menu. Furthermore, assume that $M_{A}$ and $M_{B}$ share all max learner value points. Then there exists a game $G = (\mu_{\mathcal{L}}, \mu_{\mathcal{O}})$ in which $B$ strictly outperforms $A$.
 \end{lemma}

 %\esh{Issue to be dealt with : Does either menu having a unique min value point translate to there being a unique min value point from the menu in the set of extreme points of the convex hull of the union? -- this is implictly assumed in the current version of the proof}

 %\esh{Fix found - to be added -- if a unique extreme point of a menu is not an extreme point of the convex hull of the union, then there are in fact unique extreme points from both menus that are extreme points of the convex hull of the union}

 \begin{proof}

 Consider some extreme point $b$ of $M_{B}$. It has some maximizing direction $d_{b}$. Let $\epsilon_{b}$ be the smallest difference between $\langle b, d_{b} \rangle$ and $\langle \hat b, d_{b} \rangle$ for any $\hat b \neq b \in M_{B}$. Note that, by the fact that $M_{B}$ is a polytope, $\epsilon_{b}$ must be strictly greater than $0$. Furthermore, let $$\epsilon_{B} : =\min_{b \in M_{B}}\epsilon_{b}$$
 Intuitively, $\epsilon_{B}$ is the smallest amount of "wiggle room" that any extreme point in $M_{B}$ has in its optimizing direction, before another extreme point becomes optimal. 



Now, let us consider any pair of red and blue point such that the red point has strictly lower $\mu_{\mathcal{L}}$ value and they have closer optimizing directions to each other than to anyone else (or is within epsilon). We are also ok with ties.

This must exist. If not, then if we made every red point have an arrow to the higher value point of closest optimizing direction, and same for blue, none of these lines can go towards each other. This graph has 2n nodes which each have an edge, so there has to be a cycle. If that cycle has two blues in a row or two reds in a row, that's a contradiction. If that cycle is of length more than $2$, then we have like, B1 R1 B2 R2 B1. This means that B1 is closer to R1, but R1 is closer to B2, but B2 is closer to R2, but R2 is closer to B1. The distance of these edges has to like strictly decrease every time you don't loop back to the one before, but then this means when you get back to the start you have a contradiciton. So a pair like this exists.

NOW, you can just pick the perpendicular angle to their tangent line. this will be a convex combo of both of them. Plus a tiny bit towards red. There should not be any points in this direction--

This means they obviously both are picked, unless there were ties for UL on the red and blue points. 
But if there were ties, the point still has to be different, so there has to be some direction separating them. Mix in a tiny bit of that for each. Now, if you have two different ties, you do have to be a bit careful. 



%Ask every blue for the extreme point from R or B which has lower UL value but has closest maximizing direction among those points. If it's red, and it's within wiggle room, just pick any. At least one of these blue extreme points must return a red point. If within epsion, we done. If not, if we pick the maximizing direction halfway between the points, the red one is picked in MR and the blue in MB.  

 %Let $C$ be the convex hull of the union of the extreme points of $M_{A}$ and $M_{B}$. Note that $C$ may not be a polytope if $M_{A}$ is not a polytope, and thus may have an infinite number of extreme points. Regardless, every extreme point in $C$ must be an extreme point of either $M_{A}$ or $M_{B}$. Let us color the extreme points of $C$ according to which menu they were originally from. If the extreme point is an extreme point in $M_{A}$ but not $M_{B}$, color it red. If it is an extreme point of both menus, or just an extreme point of $M_{B}$, color it blue. Note that all blue points are extreme points, i.e., vertices, of $M_B$, and there are only a finite number of them.



 %Call the max learner value of $M_{A}$ and $M_{B}$ $\L_{max}$. 
%Combining our assumption with Lemma~\ref{lemma:unique_points_preserved}, there is at least one red-colored extreme point in $C$ which is separated from any blue-colored points by some value $ > 0$ (as otherwise in the limit, $M_{B} = M_{A}$).  Since $C$ is convex, there are no local maxima. Therefore there is a path $P$ of (extreme points of) strictly increasing $\mu_{\mathcal{L}}$ value from any point on the surface of $C$ to a max-valued $\mu_{\mathcal{L}}$ point such that all adjacent extreme points on the path are either connected by an edge or are infinitely close to each other. By our assumption that all the max-valued $\mu_{\mathcal{L}}$ points are blue, there is therefore a (potentially continuous) path along the surface of $C$ of strictly increasing $\mu_{\mathcal{L}}$ value from any red point to some blue point. 


%Consider the minimal blue point for which this is true; that is, the blue point such that it has a path to a red point of smaller value, and it's the shortest such path. So it shouldn't have more than one blue point in it. 
 %There are two cases: 

% \begin{itemize}

% \item There is a red extreme point which has an optimizing direction within $\frac{\epsilon_{B}}{2}$ of it, where the red point has strictly lower $\mu_{\mathcal{L}}$ value. Then, pick this point. Boom.

 %\item There is no red extreme point which has an optimizing direction within $\frac{\epsilon_{B}}{2}$ of it in which the red point has strictly lower $\mu_{\mathcal{L}}$ value. Then, this blue point isn't infinitely close to any red points, so the thing between this blue point and a red point has to be an edge.

  %Boom.
 %\end{itemize}


% %To show that these are the only two possible cases, assume for contradiction that there is no direction $d$ such that some $r$ and $b$ are uniquely optimal, where the red point has strictly lower $\mu_{\mathcal{L}}$ value. Then, pick any two arbitrary $r$ and $b$ points where the red point has strictly lower $\mu_{\mathcal{L}}$ value (this must be possible to do). By our assumption, the direction in which these points have equal value has some other point which has higher value. Furthermore, this point must have $\mu_{\mathcal{L}}$ value between $r$ and $b$.



% %Then, consider some red extreme point $r$ and some blue extreme point $b$ of larger $\mu_{\mathcal{L}}$ value. If there is no red extreme point closer to $b$ than $r$ with $\mu_{\mathcal{L}}$ value between $b$ and $r$, and there is no edge between $b$ and $r$, then there must be a blue extreme point $b_{2}$ closer to $b$ than $r$ with $\mu_{\mathcal{L}}$ value between $b$ and $r$. Continue picking $b$ until



% %(1) there are no edges between a red extreme point and a blue extreme point of increasing $\mu_{L}$ value, and (2) there is a blue extreme point $b$ that has some red point $r$ of lower $\mu_{\mathcal{L}}$ value which is closer to $b$ than to any other blue extreme point, and there is no infinite sequence of red extreme points of lower $\mu_{L}$ value than $b$ which converge to $b$. Since there is no such infinite sequence, $b$ must 


% %there is no well-defined red-colored extreme point of largest $\mu_{L}$ value, and furthermore there is not an infinite sequence of red extreme points that approach any point $p$ which is not a red extreme point, where $p$ has larger $\mu_{\mathcal{L}}$ value than any of these points. By our first assumption there is an infinite sequence of red-colored extreme points of increasing  $\mu_{\mathcal{L}}$ value. Let the limit value of this sequence be $\mu_{\mathcal{L}}^{*} < L+$. There is some point $x$ on $C$ which is not a red extreme point, with $\mu_{\mathcal{L}}(x) =  \mu_{\mathcal{L}}^{*}$. We know by our second assumption that for any point $p$ on $C$ that is not a red extreme point, there is a well-defined red-colored extreme point which is closest to it while having strictly less $\mu_{\mathcal{L}}$ value by some $\epsilon$ (or this set is empty). So $x$ must have a well-defined red extreme point of this type. But this point has strictly less $\mu_{\mathcal{L}}$ value by some $\epsilon$, and there is no closer point to $x$.

% %$p$ might not be an extreme point. If it is not an extreme point, it is on some face of $C$ (this should be true by definition). Pick an extreme point $p'$ on this same face with larger  $\mu_{\mathcal{L}}$ value than $p$ (should also always be possible). This point is maximized 




% %Then for every blue extreme point $b$, there is a well-defined red extreme point which is closest to $b$, given that it has strictly lower $\mu_{\mathcal{L}}$ than $b$. Now, let us iterate through all extreme blue points in decreasing over of $\mu_{\mathcal{L}}$ value. 


% %Now, consider all such red points of this form. If the red extreme point maximizing $\mu_{\mathcal{L}}$ over this set is a well-defined red extreme point in $C$, we are done. Otherwise, there is some red colored extreme point $r$ with larger $\mu_{\mathcal{L}}$ which is not in the set. This point is not the closest point to any 

% %Now, consider $b = L+$ (as we know the extreme point of $C$ maximizing $\mu_{\mathcal{L}}$ is blue). There is a well-defined red extreme point which is closest given that it has strictly lower $\mu_{\mathcal{L}}$ than $b$. 


% %As $M_{A}$ contains the unique point achieving $\L_{max}$, this implies that $\mu_{\mathcal{L}}(a^{*}) < L_{max}$). Consider the red extreme point $x$ with maximum $\mu_{\mathcal{L}}$ value. If this point is well defined, then by lemma~\ref{lem:path} there must be an edge from $x$ to a higher-value $\mu_{\mathcal{L}}$ point. By the way we chose $x$, the higher value point must be blue. 

% %From this point, by lemma~\ref{lem:path} \nat{this needs to work for paths on arbitrary convex sets, does it?}, there is a path along the convex hull $C$ ending at the max-value point of $C$ such that $\mu_{\mathcal{L}}$ is strictly increasing at each step. Since the max-valued point is blue (shared), this means that there is a path along the convex hull that crosses from red to blue which strictly increases in $\mu_{\mathcal{L}}$. Therefore, there must be a point on this path such that for any $\epsilon$, of neighboring extreme points $(r^{*},b^{*})$ such that $\langle r^{*}, \mu_{\mathcal{L}} \rangle < \langle b^{*}, \mu_{\mathcal{L}} \rangle$. Note that $r^{*}$ is not contained within $M_{B}$ and $b^{*}$ is an extreme point of $M_{B}$, so by Lemma~\ref{Bbetter}, there are games where $B$ outperforms $A$.

 \end{proof}


% \begin{observation}
%     The last case left to consider is when $M_A$ has a strict superset of min points as well as of non min/max points - clearly, $A$ can do worse on some games, but are there games where $A$ can do better?
% \end{observation}


% %Below lemma superseded by the above
% \begin{comment}
    

% \begin{lemma}[Informal]
% Foe some leader payoff, if two algorithms $A$ and $B$ induce menus that a have the same min value and the same shared unique max value point, and $A$ has a strict superset of min value points, then $A$ cannot dominate $B$.
    
% \end{lemma}
% \end{comment}




% \begin{lemma}
%     \label{lemma:maximin_plus_nr}
%     Let the learner payoff be some fixed $\mu_L$.
%     Consider an empirical distribution over action pairs $X \in \mathbb{R}^{m\times n}$. Let $\beta'$ be the marginal distribution for the learner associated with the point $X$. If $X$ simultaneously satisfies the no-regret condition and provides exactly the maximin value for the learner, then $\beta$ must be a minimax distribution for the optimizer, i.e., $\beta' \in \argmin_{\beta \in \Delta^m} \max_{a \in [m]} \mu_L(a,\beta)$.
% \end{lemma}

% \begin{proof}
%     Since the point $X$ satisfies the no-regret property, it must be the case that $\mu_L(X) \ge \max_{a\in [m]} \mu_L(a,\beta')$. By definition (and using the minimax theorem), the maximin value $V(\mu_L)$ equals $ \min_{\beta \in \Delta^m} \max_{a \in [m]} \mu_L(a,\beta)$. Putting together these inequalities, we get $\mu_L(X) \ge V(\mu_L)$. However, we know that $\mu_L(X) = V(\mu_L)$ implying that the inequalities are in fact equalities, which gives us the desired result. 
% \end{proof}


% \subsection{Beyond Polytopes}
% \label{sec:polytopes_limits}
% \input{polytopes_limits}



% \begin{comment}
    

% \begin{note}
%     Although we believe the lemma statement is correct, the current proof outline works only when all the min value points are shared.
% \end{note}

% {\bf Outline of Proof : }

% Two menus - A and B (both are polytopes!)

% \begin{itemize}
%     \item Draw the convex hull $C$ of the the union of the two menus - Note : All extreme points are A-points, B-points and AB-points (all are originally extreme points). Special case - all AB points (implies A=B). Otherwise, at least one A-point or one B-point
%     \item WLOG, consider at least one B-point extreme point of $C$. Can show that there is one extreme point with larger $u_L$ value and one with smaller $u_L$ value compared to any $B$-point extreme point (this might just be a premise of the lemma).
%     \item Pick the $B$-point $b_{\text{better}}$ that minimizes $u_L$ value. Draw the boundary hyperplane of the convex hull of all extreme points of $C$ except $\bebetter$ that is closest to $\bebetter$. Call this hyperplane $S$ and all the extreme points of $C$ on $S$ as $T$. Let $u$ be the perpendicular direction connecting $\bebetter$ to $S$. 
%     \item First, we show that there are points $c,d \in T$ such that $u_L(c) < u_L (\bebetter) < u_l(d)$ - this can be done by drawing lines from $\bebetter$ to the max and min leader value points in $C$. Now, consider the direction $u - \varepsilon u_L$ (for the optimizer payoff). All points in $S$ are tied for $u$, this tiebreaks in favor of pointss with smaller $u_L$ value, at least one has smaller value than $\bebetter$. By the choice of $\bebetter$, any such point is an A-point or an AB-point. Thus, for small enough $\varepsilon$, a point with smaller $u_L$ value is picked in $A$ and $\bebetter$ is picked in B. A similar proof is used for the other direction.
%     \end{itemize}

% \end{comment}


%\begin{theorem}
%Every algorithm which includes $L+$ in its menu and does not include any point below the learner maximin value is pareto optimal. Notably, this includes all no-regret algorithms.
%\end{theorem}

%\begin{proof}
%(informal): Assume for contradiction that some algorithm $A$ of the sort above exists, but some other algorithm $B$ pareto dominates it. By lemma~\ref{lem:minmin}, the min learner value of $B$ must be no lower than the min learner value of $A$, which is the maximin value. But the min learner value of $B$ cannot be higher than this, so the min learner value of $B$ must be the same as the min learner value of $A$. 

%Furthermore, by lemma~\ref{lem:maxmax}, the max learner value of $B$ cannot be lower than the max learner value of $A$, which is $L+$. Therefore, $B$ has a min learner and max learner value which is the same as $A$. Furthermore, since the payoffs in the matrix are unique, they must actually have the same max point. 

%Since $M_{A}$ and $M_{B}$ have the same min value and max value, then, by lemma~\ref{lem:incomp}, they must not differ on any extreme points that are not at the min or max values. 

%Finally, $M_{A}$ and $M_{B}$ must have at least one point extreme point at which they differ, otherwise neither can dominate the other. So, $M_{B}$ must have all the same extreme points as $M_{A}$, except that either $M_{A}$ has an extreme point with learner value $V$ (maximin) that $M_{B}$ does not have, or vice-versa. So the only thing that could possibly dominate $A$ is something that is just like $A$ but with different maximin-valued extreme points. We need to handle this case. 
%\end{proof}


==> old/sec3_old.tex <==

\subsection{OLD}

\begin{observation}
    Menus are closed under union (in the limit) but not under intersection.
\end{observation}
\begin{proof}
    Any two menus with a single point of intersection will suffice. The existence of such a pair can be shown by construction - by first constructing menus that do not intersect, by having the respective learning algorithms use disjoint subsets of actions, and then constructively adding a single point to both menus (again corresponding to a disjoint subset of learner actions).
\end{proof}



\begin{observation}
    There exists a menu such that if it were truncated by removing all points that achieve less than the maxmin, does not continue to remain a menu.
\end{observation}
\begin{proof}
    Such a menu is achieved by the following algorithm. Play the learner side of $L^+$ until the optimizer plays their side of it. At the first defection by the optimizer, switch to playing the constant algorithm.
\end{proof}


\begin{lemma}
The union of any valid menu and any finite set of points is a valid menu.  \label{lem:union}
\end{lemma}

\begin{proof}
Consider any valid menu $A$, it set of  extreme points $M_{A}$, and any finite set of points $P$. 
Our goal is to show an algorithm which produces the limit-object menu which is a convex hull of $M_A \bigcup P$. 

Let the algorithm $A'$ be defined as follows: define an injection $m$ from ordered sequences of optimizer moves of length $\lceil{log_{m}(|P|)} \rceil$ to elements in $P$. Play any moves during the first $log_{m}(|P|)$ rounds. Then, observe the ordered sequence $S$ played so far by the optimizer. If it does not map to a valid element in $P$, default to playing $A$ (with an empty history) for the rest of the game. If it does map to some valid element $p \in P$, play the learner's side of $p$ until the opponent ever does not play their side of $p$. If the opponent ever does not play their side of $p$, default to playing $A$ (with an empty history) for the rest of the game.  

We claim that in the limit, this algorithm's extreme points $M_{A'}$ are exactly $M_A \bigcup P$. To see this, first note that any point in $M_{A}$ is in $M_{A'}$. For any such point $x$, consider the (infinitely long) optimizer sequence $r$ that achieves it against $A$. Then, against $A'$, the optimizer can do the following: play arbitrarily for the first $\lceil{log_{m}(|P|)} \rceil$ rounds, then play anything other than the expected side of $p$ in the next round. The learner will then begin playing according to $A$. Now, the optimizer can play $r$. In the limit, this point will approach $x$. 
\end{proof}


%\section{Results for General Algorithms}

\begin{definition}[Minimal Menu]
A minimal menu is a menu for which there is no other valid menu strictly contained within it. 
\end{definition}

\begin{definition}[Minimal L+ Menu]
A minimal L+ menu is a menu that contains L+, and for which there is no other valid menu strictly contained within it that also contains L+.
\end{definition}

\begin{theorem}
\label{thm:L+_minimal_po}
An algorithm is pareto-optimal if for all $\mu_{\mathcal{L}}$, (all )its asymptotic menu(s) is a polytope and is a minimal $L+$ menu. 
\label{thm:L+minimal}
\end{theorem}

\esh{Big change here !! -- Let's weaken this to the following statement (something that can be proved with the current machinery) -- An algorithm is pareto-optimal if its menu is a polytope and is L+-minimal  for all $\mu_{\mathcal{L}}$. }

\nat{Are all L+-minimal menus polytopes? Probably not, but worth thinking about}

\nat{Does the strictly increasing path argument still work for general convex sets?}

\begin{proof}
Call the algorithm described above $B$. 
To prove that $B$ is pareto-optimal over all games, it is sufficient for us to prove the stronger statement that it is pareto-optimal over every fixed $\mu_{\mathcal{L}}$. Consider any $\mu_{\mathcal{L}}$, and the induced menu $M_{B}$. 


Let us assume for contradiction that some algorithm $A$ (whose menu might not necessarily be a polytope) pareto-dominates $B$. Then $A$ must outperform $B$ on some game $G = (\mu_{\mathcal{L}},\mu_{\mathcal{O}})$. This means that $M_{B}$ and $M_{A}$ cannot be the exact same menu. 

We claim that $M_{A}$ is not a strict subset of $M_B$. If it were, then by Lemma~\ref{lem:minimal}, it must not contain $L+$, and in this case it cannot pareto-dominate $B$, as $B$ would outperform $A$ when $\mu_{\mathcal{O}} = \mu_{\mathcal{L}}$. Since $M_{A}$ is not a strict subset of $M_{B}$ and is not the same menu as $M_{B}$, there must be some extreme point in $M_{A}$ which is not contained within $M_{B}$. Recall also that $M_{A}$ and $M_{B}$ share the same max learner value point. Thus by lemma~\ref{lem:incomp}, $B$ outperforms $A$ on some games. Therefore $A$ does not pareto dominate $B$. As we have selected $A$ to be any algorithm that outperforms $B$ on some game, and shown that all $A$ of this form do not pareto-dominate $B$, there is no algorithm that pareto-dominates $B$. 
\end{proof}



\begin{lemma}
\label{lem:minimal}
The menu which has the extreme points $(b_{l},b_{o})$ and also $(a,j)$ $\forall j \in [m]$ is a minimal $L+$-containing menu.
\end{lemma}

\begin{proof}
Assume for contradiction that it is not $L+$-minimal. Then there exists a menu containing $L+$ which is strictly contained within this menu. Let us call the original menu $M$ and the new menu $M'$. First, note that $M'$ must contain the extreme point $(b_{l},b_{o})$ be definition. In addition it must contain the extreme point $(a,j)$ $\forall j \neq b_{o}$. This is because for all $j \neq b_{o}$, the only move pair containing $j$ present anywhere in the menu is $(a, j)$. So whatever menu point is created by the optimizer always playing $j$ is either $(a,j)$ or a new extreme point. Furthermore, the menu cannot contain any points in which the leader plays any moves other than $b_{l}$ or $a$ (other than a vanishing fraction of the time). 

This leaves us with only one extreme point we may be able to remove: $(a,b_{o})$. Thus, $M'$ has all extreme points in $M$ except for this point. Now, let the extreme point in $M'$ which includes the move pair $(a,b_{o})$ most frequently be called $X$, and let $1 - \epsilon$ be the fraction of the time that $(a,b_{o})$ is played in $X$. Note that $\epsilon$ is a constant between $0$ and $1$ independent of $T$, as otherwise by our assumptions on menus, $M'$ would be the same menu as $M$. 

 Because $M'$ is a valid menu, there must exist some algorithm $A'$ which induces it. Now, let the optimizer play the following strategy against $A'$: on rounds where $A'$ will play $a$ w.p. $\geq 1 - \frac{\epsilon}{100}$, play $b_{o}$. On rounds where $A'$ will play $b_{l}$ w.p. $> \frac{\epsilon}{100}$, play some other specific move $k$. If neither of these cases is true, they will play any arbitrary move. Note that $A'$ cannot play another move other than $a$ or $b_{l}$ for a constant number of rounds, as there are no extreme points in $M'$ involving any other moves for the learner, so we will disregard those move pairs in the sequence. (Have to clean this up a little bit to make sure they don't just have a sublinear probability of a random additional move every time to go to the arbitrary case but that's easy). 

Now, consider what distribution this will create. If $A'$ plays $a$ w.p. $\geq 1 - \frac{\epsilon}{100}$ on a $1 - \frac{\epsilon}{100}$ fraction of rounds, then there will be a point in the menu that has the move pair $(a,o)$ appearing at least a $(1 - \frac{\epsilon}{100})(1 - \frac{\epsilon}{100})$ fraction the time. This would lead to a contradiction, as this is greater than $1 - \epsilon$:

\begin{align*}
(1 - \frac{\epsilon}{100})(1 - \frac{\epsilon}{100}) = 1 - \frac{\epsilon}{50} + \frac{\epsilon^{2}}{10,000} \\
= 1 - \epsilon (\frac{\epsilon}{10000} - \frac{1}{50})
\geq 1 - \frac{\epsilon}{10000} + \frac{1}{50} \\
\geq 1 - \frac{\epsilon}{10000} \geq 1 - \epsilon
\end{align*} \\


Otherwise, $A'$ most plays $l$ w.p. $\geq \frac{\epsilon}{100}$ on a $ \geq \frac{\epsilon}{100}$ fraction of rounds. On those rounds the optimizer will play $k$. But this means that the move pair $(l,k)$ must appear in an extreme point $\geq \frac{\epsilon}{100} \cdot \frac{\epsilon}{100}$ fraction of the time, which is also a constant, leading to a contradiction. Thus, every scenario leads to a contradiction, so $M'$ is not a valid menu and $M$ is a minimal $L+$-containing menu. 


\end{proof}


%\subsection{Results about No-Swap Regret Algorithms - Proof of Theorem~\ref{theorem:all_about_nsr}}
%\label{sec:all_about_nsr}

%\input{NSR_NR}

==> pareto_optimal_menus_old.tex <==
\section{Characterizing Pareto-Optimal Menus}
\label{sec:pareto-optimal-menus}

In this section we shift our attention to understanding which asymptotic menus are Pareto-optimal and which are Pareto-dominated by other asymptotic menus. The ideal result would be a characterization of all Pareto-optimal asymptotic menus; we will stop a little short of this and instead provide a full characterization of all Pareto-optimal \emph{no-regret} menus that are also \emph{polytopal} -- i.e., can be written as the intersection of a finite number of half-spaces. This characterization will be sufficient for proving our main results that the no-swap-regret menu $\M_{NSR}$ is Pareto-optimal, but that the menu corresponding to multiplicative weights is sometimes Pareto-dominated. 

Before we introduce the characterization, we introduce a little bit of additional notation. For any menu $\M$, let $\Up(\M) = \max_{\csp \in \M} u_{L}(\csp)$ denote the maximum learner payoff of any CSP in $\M$; likewise, define $\Um(\M) = \min_{\csp \in \M} u_{L}(\csp)$. We will also let $\M^{+} = \argmax_{\csp \in \M} u_{L}(\csp)$ and $\M^{-} = \argmin_{\csp \in \M} u_{L}(\csp)$ be the subsets of $\M$ that attain this maximum and minimum (we will call these the \emph{maximum-value} and \emph{minimum-value sets} of $\M$).

Our characterization can now be simply stated as follows.

\begin{theorem}\label{thm:pareto-optimal-characterization}
Let $\M$ be a polytopal no-regret menu. Then $\M$ is Pareto-optimal iff $\M^{-} = \M^{-}_{NSR}$. That is, $\M$ must share the same minimum-value set as the no-swap-regret menu $\M_{NSR}$.
\end{theorem}

Note that while this characterization only allows us to reason about the Pareto-optimality of polytopal no-regret menus, in stating that these menus are Pareto-optimal, we are comparing them to all possible asymptotic menus. That is, we show that they are not Pareto-dominated by any possible asymptotic menu, even one which may have high regret and/or be an arbitrary convex set. We conjecture that this characterization holds for all no-regret menus (even ones that are not polytopal).

The remainder of this section will be dedicated to proving Theorem \ref{thm:pareto-optimal-characterization}. We will begin in Section \ref{sec:learner-utilities} by establishing some basic properties about $\M^{+}$, $\M^{-}$, $\Um(\M)$, and $\Up(\M)$ for no-regret and Pareto-optimal menus. Then in Section \ref{sec:minimal-lemma} we prove our main technical lemma (Lemma \ref{lem:non-dominance}), which shows that a menu cannot be Pareto-dominated by a menu with a larger minimal set. Finally, we complete the proof of Theorem \ref{thm:pareto-optimal-characterization} in Section \ref{sec:completing-the-proof}, and discuss some implications for the Pareto-optimality of the no-regret and no-swap-regret menus in Section \ref{sec:regret-implications}.



% (which will set up the framework for proving that multiplicative weights is sometimes Pareto-dominated in Section \ref{sec:mean_based_pareto_dominated}). 


% In this section we shift our attention to understanding which asymptotic menus are Pareto-optimal and which are Pareto-dominated by other asymptotic menus. Our main goal will be the establishment of key technical tools for establishing pareto-domination or incomparability of pairs of menus This will set up the framework for proving that multiplicative weights is sometimes Pareto-dominated in Section~\ref{sec:mean_based_pareto_dominated} and the framework for proving that all no swap regret algorithms are pareto-optimal in section~\ref{sec:all_about_nsr}. 


\subsection{Constraints on learner utilities}
\label{sec:learner-utilities}

We begin with some simple observations on the possible utilities of the learner under Pareto-optimal menus and no-regret menus. We first consider $\M^{+}$. Recall that (by assumption) there is a unique pure strategy profile $\csp^{+} = (i^{*}) \otimes (j^{*})$ that maximizes the learner's reward. We claim that any Pareto-optimal menu must contain $\csp^{+}$.

\begin{lemma}\label{lem:has_max_point}
If $\M$ is a Pareto-optimal asymptotic menu, then $\M^{+} = \{\csp^{+}\}$.
\end{lemma}
\begin{proof}
Assume $\M$ is a Pareto-optimal asymptotic menu that does not contain $\csp^{+}$. By Lemma \ref{lem:char_upwards_closed}, the set $\M' = \conv(\M, \csp^{+})$ is also a valid asympotic menu. We claim $\M'$ Pareto-dominates $\M$.

To see this, first note that when $u_O = u_L$, $V_L(\M', u_O) = u_L(\csp^{+}) > V_{L}(\M, u_O)$, since $\csp^{+}$ is the unique CSP in $\Delta_{mn}$ maximizing $u_L$. On other hand, for any other $u_O$, the maximizer of $u_O$ over $\M'$ is either equal to the maximizer of $u_O$ over $\M$, or equal to $\csp^{+}$. In either case, the learner's utility is at least as large, so $V_L(\M', u_O) \geq V_L(\M, u_O)$ for all $u_O$. It follows that $\M'$ Pareto-dominates $\M$.  
\end{proof}

Note also that $\csp^{+}$ belongs to $\M_{NSR}$ (since it a best-response CSP of the same form as in Lemma \ref{lem:nsr_characterization}), so $\M^{+}_{NSR} = \csp^{+}$. Since $\M_{NSR}$ is also contained in every no-regret menu, this also means that for any (not necessarily Pareto-optimal) no-regret menu $\M$, $\M^{+} = \M^{+}_{NSR} = \csp^{+}$.

We now consider the minimum-value set $\M^{-}$. Unlike for $\M^{+}$, it is no longer the case that all Pareto-optimal menus share the same set $\M^{-}$. It is not even the case (as we shall see in Section \ref{sec:other-pareto-optimal}), that all Pareto-optimal menus have the same minimum learner utility $\Um(\M)$. 

% However, it is the case that all \emph{no-regret} algorithms share the same value for the minimum learner utility $\Um(\M)$, namely $\Uzs = \Um(\M_{NR})$. The reason for this is that $\Uzs$ is also the largest utility the learner can guarantee when playing a zero-sum game (i.e., when the optimizer has payoffs $u_{O} = -u_{L}$), and thus it is impossible to obtain a higher value of $\Um(\M)$. We will prove this in Section~\ref{sec:all_about_nsr}, after introducing no-regret and no-swap-regret menus. 


However, it is the case that all \emph{no-regret} algorithms share the same value for the minimum learner utility $\Um(\M)$, namely the ``zero-sum'' utility $\Uzs = \min_{x \in \Delta_{m}} \max_{y \in \Delta_{n}} u_L(x, y)$. The reason for this is that $\Uzs$ is the largest utility the learner can guarantee when playing a zero-sum game (i.e., when the optimizer has payoffs $u_{O} = -u_{L}$), and thus it is impossible to obtain a higher value of $\Um(\M)$. This is formalized in the following lemma.

\begin{lemma}\label{lem:menu-min-value}
Every asymptotic menu must have $\Um(\M) \leq \Uzs$. Moreover, if $\M$ is a no-regret asymptotic menu, then $\Um(\M) = \Uzs$, and $\M_{NSR}^{-} \subseteq \M^{-}$.
\end{lemma}
\begin{proof}
Let $(x_{ZS}, y_{ZS})$ be the solution to the minimax problem $\min_{x \in \Delta_{m}} \max_{y \in \Delta_{n}} u_L(x, y)$ (i.e., the Nash equilibrium of the corresponding zero-sum game). By Theorem \ref{thm:characterization}, any asymptotic menu $\M$ must contain a point of the form $x_{ZS} \otimes y$. By construction, $u_L(x_{ZS} \otimes y) \leq U_{ZS}$, so $\Um(\M) \leq U_{ZS}$.

To see that every no-regret asymptotic menu satisfies $\Um(\M) = \Uzs$, assume that $\M$ is a no-regret menu, and $\csp \in \M$ satisfies $u_L(\csp) < \Uzs$. Since $\csp$ has no-regret (satisfies the conditions of \eqref{eq:no-regret-constraint}), we must also have $u_L(\csp) \geq \max_{y \in \Delta_{n}} \min_{x \in \Delta_{m}} u_L(x, y)$, since this holds for whatever marginal distribution $x$ is played by the optimizer under $\csp$. But by the minimax theorem, $\max_{y \in \Delta_{n}} \min_{x \in \Delta_{m}} u_L(x, y) = U_{ZS}$, and so we have a contradiction.

Finally, note that since $\M$ is no-regret, $\M_{NSR} \subseteq \M$ and so $\M_{NSR}^{-} \subseteq \M^{-}$ (since they share the same minimum value). 
% \jon{Theorem \ref{thm:nr_nsr_containment} shows one direction; thinking about the NE of the ZSG shows the other.}
\end{proof}

What can we say in place of Lemma \ref{lem:menu-min-value} for the case of \emph{high-regret} algorithms (algorithms which are not no-regret?). As mentioned earlier, there exist Pareto-optimal high-regret algorithms which do not satisfy the conditions of Lemma \ref{lem:menu-min-value} \jon{consider moving the theorem in section 6 here (and removing section 6)}. However, the following lemma shows that high-regret algorithms can never Pareto-dominate no-regret algorithms, and hence are safe to ignore for the purpose of determining which no-regret menus are Pareto-optimal.

\begin{lemma}\label{lem:high-regret-cannot-dominate}
Let $\cA$ be a high-regret learning algorithm, and let $\cA'$ be a no-regret learning algorithm. Then $\M(\cA)$ cannot Pareto-dominate $\M(\cA')$.
\end{lemma}
\begin{proof}
Without loss of generality, assume $\M(\cA)^{+} = \{\csp^{+}\}$; if not, then apply Lemma \ref{lem:has_max_point} to construct a menu that Pareto-dominates $\M(\cA)$ and use that in place of $\cA$. Since $\cA'$ is no-regret, note that $\M(\cA')^{+}$ also equals $\{\csp^{+}\}$.

Now, if $\cA$ is a high-regret learning algorithm, there is some CSP $\csp \in \M(\cA)$ which has high regret with respect to some fixed action. That is, there exists some $j^* \in [n]$ such that

\begin{equation}\label{eq:high-regret}
\sum_{i\in[m]}\sum_{j\in[n]} \csp_{ij}(u_{L}(i, j^*) - u_{L}(i, j)) > 0.
\end{equation}

\jon{todo: finish (right now I think I can get things to work if the algorithm has high regret wrt the same $j^*$ as in $\csp^{+}$, but I'm hoping it works in general)}
% Consider the payoff $u_O$ defined via $u_O(i, j) = u_L(i, j^*) - u_L(i, j)$. By \eqref{eq:high-regret}, there exists a CSP $\csp \in \M(\cA)$ where $u_O(\csp) > 0$. This CSP cannot be $\csp^{+}$, since $\csp^{+}$ has no regret 
\end{proof}

% Unlike $\M^{+}$ which is always equal to $\{\csp^{+}\}$ for Pareto-optimal menus, the minimizing set $\M^{-}$ is not uniquely defined and may contain many CSPs. However, there is a ``minimal'' minimizing set $\M^{-}$ for no-regret menus: any such menu $\M^{-}$ must contain $\M_{NSR}^{-}$.



%In fact, this is true for the slightly larger class of menus with $\Um(\M) = \Uzs$. 

% \begin{lemma}\label{lem:menu-min-set}
% Let $\M$ be an asymptotic menu with $\Um(\M) = \Uzs$. Then $\M_{NSR}^{-} \subseteq \M^{-}$. \jon{Actually, is this theorem true? What about e.g. the learner strategy that always plays their nash eq?}
% \end{lemma}
% \begin{proof}
% By Lemma~\ref{lem:nsr_characterization}, $\M_{NSR}^{-}$ can also be written as the convex combination of extreme points of the form $x \otimes y$, with $x \in \Delta_{m}$ and $y \in \BR_{L}(x)$. We will show that any such point must also belong to $\M^{-}$, thus implying the theorem statement.

% Assume, for sake of contradiction, that some such point $x \otimes y$ does not belong to $\M$. Furthermore, assume to start that $y$ is the unique best-response to $x$, so $\BR_{L}(x) = \{y\}$ (we will describe how to lift this assumption later). By our characterization of valid asymptotic menus, there must be some $y' \in \Delta_{n}$ such that $x \otimes y'$ does belong to $\M$. By assumption, $y'$ is not a best response to $x$, so $u_L(x \otimes y') < u_L(x \otimes y) = \Uzs$. But this contradicts the fact that $\Um(\M) = \Uzs$.

% To handle the situation where $y$ is not the unique best response to $x$, recall that by 

% \jon{old proof:}

% Then there is some menu $\M$ with a point $X =  x \otimes y$ such that $y \in \BR_{L}(x)$ that is not present in $\M$. %Since $\M$ is convex, without loss of generality, $y$ is a pure strategy of the learner. 

% Note that for all points in $M^{-}$ of the form $x \otimes y$, with $x \in \Delta_{m}$, $y \in \BR_{L}(x)$, $x$ must be a minmax distribution. Therefore, it is sufficient to prove that all menus with $U^{-}(M) = U_{ZS}$ must contain all points of the form $x_{mm} \otimes y$, where $x_{mm}$ is a minmax distribution and $y \in \BR_{L}(x)$.

% By the fact that $U^{-}(M) = U_{ZS}$, if $x_{mm}$ is a minmax distribution, then any point of the form $x_{mm} \otimes y$ in $\M$ must have that $y$ is a best response to $x_{mm}$. By Lemma~\ref{lem:farkas}, for all such $x_{mm}$, $\M$ must include all points of the form $x_{mm} \otimes y$, with $y \in \BR_{L}(x_{mm})$. \nat{this lemma got deconstructed and put into other lemmas now it seems, so we need to correct this pointer}

% Thus, at least one such point is not in $\M$, in which case we can use the previous case's argument to derive a contradiction, completing the proof.

% \end{proof}


\subsection{Pareto-domination and minimum-value sets}
\label{sec:minimal-lemma}
%\begin{theorem}\label{thm:characterization_polytope}
%A no-regret polytopal menu $\M$ is Pareto-optimal iff $\M^{+} = \M_{NSR}^{+}$ ($= \{\csp^{+}\}$) and $\M^{-} = \M^{-}_{NSR}$.
%\end{theorem}

%Note that while this result only allows us to reason about the pareto-optimalily of no-regret polytopal menus, the pareto-optimality condition is still measured by comparing to all other menus, which may have high regret and/or be arbitrary convex sets. 

% We will show a sequence of lemmas describing the conditions under which a menu $\M_1$ can Pareto-dominate a menu $\M_2$. The significant lemma we build towards is Lemma~\ref{lem:non-dominance}, which states a necessary condition for any menu to be pareto-dominated. This will be used to show that every no swap regret algorithm is pareto optimal and, conversely, leveraged to show that all strictly mean-based algorithms are pareto-dominated.

We now present our main lemma in the proof of Theorem \ref{thm:pareto-optimal-characterization}, which shows that if one menu has a larger minimum-value set than another menu (and both menus share the same maximum-value set), then the first menu cannot possibly Pareto-dominate the second menu.
 
\begin{lemma}\label{lem:non-dominance}
Let $\M_1$ and $\M_2$ be two distinct asymptotic menus where $\M_{1}^{+} = \M_{2}^{+}$, and $\M_{1}^{-} \subseteq \M_{2}^{-}$. Then there exists a $u_O$ for which $V_{L}(\M_1, u_O) > V_{L}(\M_2, u_O)$ (i.e., $\M_2$ does not Pareto-dominate $\M_1$).
\end{lemma}

\esh{Sanity check - do we really need $\M_{1}^{+} = \M_{2}^{+}$ or is $U^+(\M_1) = U^+(\M_2)$ sufficient? - I guess with our assumption about learner payoffs - they are equivalent.}

Note that Lemma \ref{lem:non-dominance} holds even in the case where $\M_{1}^{-} = \M_{2}^{-}$. One important consequence of this is that all menus with the same value of $\M^{-}$ and $\M^{+}$ are incomparable to each other under the Pareto-dominance order.~\esh{This statement is a bit confusing - can we replace it with the phrase "same value of" with "identical min and max value sets"?}

We introduce one more lemma, which covers the case 


\begin{lemma}\label{lem:minimal_non-dominance}
Let $\M_1$ and $\M_2$ be two distinct asymptotic menus where $\M_{1}^{+} = \M_{2}^{+}$, and $\M_2 \setminus \M_1 \ne \phi$. Then there exists a $u_O$ for which $V_{L}(\M_1, u_O) > V_{L}(\M_2, u_O)$ (i.e., $\M_2$ does not Pareto-dominate $\M_1$).
\end{lemma}

\esh{I think the previous lemma becomes a corollary - we can split the analysis into two cases - $\M_{1}^{-} = \M_{2}^{-}$ and $\M_{1}^{-} \subsetneq \M_{2}^{-}$}

The key technical ingredient for proving Lemma \ref{lem:non-dominance} is the following lemma, which establishes a ``two-dimensional'' variant of the above claim.

\begin{lemma}\label{lem:geometry}
Let $f, g: [a, b] \rightarrow \mathbb{R}$ be two distinct concave functions satisfying $f(a) \leq g(a)$ and $f(b) = g(b)$. For $\theta \in [0, \pi]$, let $\hat{f}(\theta) = \argmax_{x \in [a, b]} (x\cos\theta + f(x)\sin\theta)$ (if the argmax is not unique, then $\hat{f}(\theta)$ is undefined). Define $\hat{g}(\theta)$ symmetrically. Then there exists a $\theta$ for which $\hat{f}(\theta) > \hat{g}(\theta)$. %\nat{Should it be $x \in [a,b]$?}
\end{lemma}
\begin{proof}
Since $f(x)$ is a concave curve, it has a (weakly) monotonically decreasing derivative $f'(x)$. This derivative is not necessarily defined for all $x \in [a, b]$, but since $f$ is concave it is defined almost everywhere. At points $c$ where it is not defined, $f$ still has a well-defined left derivative $f'_L(x) = \lim_{h \rightarrow 0} (f(x) - f(x - h))/h$ and right derivative $f'_R(x) = \lim_{h \rightarrow 0} (f(x + h) - f(x))/h$. We will abuse notation and let $f'(x)$ denote the interval $[f'_L(x), f'_R(x)]$ (at the boundaries defining $f'(a) = (-\infty, f_{R}(a)]$ and $f'(b) = [f_{L}(b), \infty)$. Similarly, the interval-valued inverse function $(f')^{-1}(y)$ is also well-defined, decreasing in $y$, and uniquely-defined for almost all values of $y$ in $(-\infty, \infty)$. 

Note that since $\hat{f}(\theta)$ is the $x$ coordinate of the point on the curve $f(x)$ that maximizes the inner product with the unit vector $(\cos\theta, \sin\theta)$, $f'(\hat{f}(\theta))$ must contain the value $-\cos\theta / \sin\theta = -\cot \theta$. In particular, if $\hat{f}(\theta)$ is uniquely defined, $\hat{f}(\theta) = (f')^{-1}(-\cot \theta)$. So it suffices to find a $y$ for which $(f')^{-1}(y) > (g')^{-1}(y)$. 

To do this, we make the following observation: since $f(b) - f(a) \geq g(b) - g(a)$, $\int_{a}^{b} f'(x)dx \geq \int_{a}^{b} g'(x)dx$~\footnote{These integrals are well defined because the first derivatives of $f$ and $g$ exist almost everywhere.}. This means there must be a point $c \in (a, b)$ where $f'(c) > g'(c)$. If not, then we must have $f'(x) \leq g'(x)$ for all $x \in (a, b)$; but the only way we can simultaneously have $f'(x) \leq g'(x)$ for all $x \in (a, b)$ and $\int_{a}^{b}f'(x)dx \geq \int_{a}^{b}g'(x)dx$ is if $f'(x) = g'(x)$ for almost all $x \in (a, b)$ -- but this would contradict the fact that $f$ and $g$ are distinct concave functions.

Now, take a point $c \in (a, b)$ where $f'(c) > g'(c)$ and choose a $y$ in $f'(c)$. Since $g'$ is a decreasing function, there must exist a $c' < c$ such that $y \in g'(c')$, and so $(f')^{-1}(y) > (g')^{-1}(y)$. 


% \nat{Comment below about generalization}\jon{commented out for now (I think we don't need this given Appendix \ref{app:pareto-dominance-eq}).}



% Working on a generalization to multiple different $u_{0}$ but it might not work: To do this, we make the following observation: since $f(b) - f(a) \geq g(b) - g(a)$, $\int_{a}^{b} f'(x)dx \geq \int_{a}^{b} g'(x)dx$~\footnote{These integrals are well defined because the first derivatives of $f$ and $g$ exist almost everywhere}. This means there must be an interval $C = (c^{-},c^{+}) \in (a,b)$ where $f'(c) > g'(c), \forall c \in C$, $c^{+} - c^{-}  = \epsilon > 0$, $f'(c^{-}) = g'(c^{-})$, and $f'(c^{+}) = g'(c^{+})$. If not, then we must have $f'(x) \leq g'(x)$ for all but a zero-measure set of $x \in (a, b)$; but the only way we can simultaneously have $f'(x) \leq g'(x)$ for all but a zero-measure set of $x \in (a, b)$ and $\int_{a}^{b}f'(x)dx \geq \int_{a}^{b}g'(x)dx$ is if $f'(x) = g'(x)$ for almost all $x \in (a, b)$ -- but this would contradict the fact that $f$ and $g$ are distinct concave functions. 

% Now, choose $y^{+}$ in $f'(c^{+}-\alpha)$ for some constant $\alpha < \frac{\epsilon}{4}$. Since $g'$ is a decreasing function, there must exist a $x^{+} < c^{+} - \alpha$ such that $y^{+} \in g'(x^{+})$, and so $(f')^{-1}(y^{+}) > (g')^{-1}(y^{+})$. Next, choose $y^{-}$ in $f'(c^{-} + \alpha)$. Again, there must exist a $x^{-} < c^{-} + \alpha$ such that $y^{-} \in g'(x^{-})$, and so $(f')^{-1}(y^{-}) > (g')^{-1}(y^{-})$. We claim that for some choice of $\alpha$, $y^{-}$ and $y^{+}$ must be different. Assume for contradiction that they are not. Then, $f'(c^{+} - \alpha) = f'(c^{-} + \alpha)$ for all $\alpha > 0$. For this to be the case, it must be that $f'(c^{+}) = f'(c^{-})$. But then, we have that $g'(c^{+}) = f'(c^{-})$ and $g'(c^{-}) = f'(c^{+})$. So we have that 

% \begin{align*}
% & g'(c^{-} + \epsilon) < f'(c^{-} + \epsilon) \\ &
% < f'(c^{-}) \tag{As $f'$ is nonincreasing} \\
% & = g'(c^{+})
% \end{align*}

% But this means that $g'(c^{-} + \epsilon) < g'(c^{+})$. Recall that $c^{-} + \epsilon < c^{+}$. Therefore, this is a contradiction, as $g'$ is also nonincreasing.  

% Let $\beta = y^{-} - y^{+}$. Now, consider any $y$ such that $y^{-} \leq y \leq y^{+}$. By the fact that $f'$ is nonincreasing, if $f'(c) = y$, then $c^{-} \leq c \leq c^{+}$. Therefore, $f(y^{-}) < f(y) < f(y^{+})$.  


% Therefore, $y^{-}$ and $y^{+}$ are separated for some choice of $\alpha$. This means that $f(y^{+}) > g(y^{+})$ and $f(y^{-}) > g(y^{-})$ for two distinct values. 


% Now, take a point $c \in (a, b)$ where $f'(c) > g'(c)$ and choose a $y$ in $f'(c)$. Since $g'$ is a decreasing function, there must exist a $c' < c$ such that $y \in g'(c')$, and so $(f')^{-1}(y) > (g')^{-1}(y)$. 



% \nat{end comment}
\end{proof}

We can now prove Lemma \ref{lem:non-dominance}. \jon{this proof might be a good candidate for a diagram}

\begin{proof}[Proof of Lemma~\ref{lem:non-dominance}]
Since $\M_1$ and $\M_2$ are distinct asymptotic menus, there must be an extreme point $\csp$ in one menu that does not belong to the other. In particular, there must exist an optimizer payoff $u_{O}$ where $u_{O}(\csp) > u_{O}(\csp')$ for any $\csp'$ in the other menu. Denote this specific optimizer payoff by $u_{O}^{0}$.
% \esh{This is intuitive, but should we offer a proof? We wrote something along these lines for an older sequence of ideas - we wrote this because not every distinct extreme point of $M_1$ necessarily does better on its unique max direction within $M_1$ when compared to points in $M_2$}\jon{I think this fact is well-known enough that we don't need to prove it separately (it's a consequence of the separating hyperplane theorem).}

We will show that there exists a $u_{O} \in \mathrm{span}(u_L, u_{O}^{0})$ where $V_{L}(\M_1, u_O) > V_{L}(\M_2, u_O)$. To do this, we will project $\M_1$ and $\M_2$ to two-dimensional sets $S_1$ and $S_{2}$ by letting $S_{1} = \{(u_L(\csp), u_{O}^{0}(\csp)) \mid \csp \in \M_1 \}$ (and defining $S_{2}$ symmetrically). By our construction of $u_{O}^{0}$, these two convex sets $S_{1}$ and $S_{2}$ are distinct. Also, note that if $u_O = \lambda_{1}u_L + \lambda_{2}u_{O}^{0}$, we can interpret $V_{L}(\M_1, u_O)$ as the maximum value of $z_1$ for any point in $\arg\max_{(z_1, z_2) \in S_1} (\lambda_1z_1 + \lambda_2z_2)$. We can interpret $V_{L}(\M_2, u_O)$ similarly.
% \nat{This is true but needs a proof using the convex hull argument, not super obvious off the bat I think}\esh{Lemma~\ref{lemma:unique_points_preserved} does this job for us if we don't have a direct proof}\jon{doesn't this follow directly from the construction of $u_{O}^0$? one of these two sets has a larger extreme point in one direction}\nat{We meant the proof of the existence of $u_{O}^0$ itself--see new comment above.}

Let us now consider the geometry of $S_1$ and $S_2$. Let $u^{-}$ denote the common value of $\Um(\M_1)$ and $\Um(\M_2)$, and similarly, let $u^{+}$ denote the common value of $\Up(\M_1)$ and $\Up(\M_2)$. Both $S_1$ and $S_2$ are contained in the ``vertical'' strip $u^{-} \leq z_1 \leq u^{+}$. We can therefore write $S_1$ as the region between the concave curve $f_{\text{up}}:[u^{-}, u^{+}]$ (representing the upper convex hull of $S_1$) and $f_{\text{down}}$ (representing the lower convex hull of $S_1$; define $g_{\text{up}}$ and $g_{\text{down}}$ analogously for $S_2$. Since $S_1$ and $S_2$ are distinct, either $f_{\text{up}} \neq g_{\text{up}}$ or $f_{\text{down}} \neq g_{\text{down}}$; without loss of generality, assume $f_{\text{up}} \neq g_{\text{up}}$ (we can switch the upper and lower curves by changing $u_{O}^{0}$ to $-u_{O}^{0}$).



Note also that since $\M^{+}_1 = \M^{+}_2$ and $\M^{-}_1 \subseteq \M^{-}_2$, we have $f_{\text{up}}(u^{+}) = g_{\text{up}}(u^{+})$ and $f_{\text{up}}(u^{-}) \leq g_{\text{up}}(u^{-})$ (since $[f_{\text{down}}(u^{-}), f_{\text{up}}(u^{-})] \subseteq [g_{\text{down}}(u^{-}), g_{\text{up}}(u^{-})]$). By Lemma \ref{lem:geometry}, there exists a $\theta \in [0, \pi]$ for which $\hat{f}_{\text{up}}(\theta) > \hat{g}_{\text{up}}(\theta)$. But by the definition of $\hat{f}$ and $\hat{g}$, this implies that for $u_{O} = \cos(\theta) u_L + \sin(\theta) u^{0}_{O}$, $V_{L}(\M_1, u_{O}) > V_{L}(\M_2, u_O)$, as desired.%~\esh{Should likely be $[0,\pi]$ for this to make sense} 
% \nat{need to add in explanation for why we can split $\theta$ into two values for the two cases.} 
% \jon{changed the range to $[0, \pi]$, agree that makes sense. I'm not sure what ``split $\theta$ into two values for the two cases'' means.} 
% ~\nat{My confusion was about the fact that you consider two cases, where the upper and lower convex hulls have the property we want, and then focus entirely on that case. And whether we have to show that we can ignore the other part of the convex hull when considering the optimizing direction. But as I write this I realize it doesn't really makes sense so don't worry about it :)}
\end{proof}


% \begin{lemma} For any two polytopal asymptotic menus $\M_{1}$ and $\M_{2}$, if there is some $u_{O}$ such that $V_{L}(\M_{1},u_{O}) > V_{L}(\M_{2},u_{O})$, then there is some constant measure set of  $u'_{O}$ such that $V_{L}(\M_{1},u'_{O}) > V_{L}(\M_{2},u'_{O})$.
% \end{lemma}
% \begin{proof}
% Let $x_{1}$ be the extreme point in $\M_{1}$ in the direction $u_{O}$, and let $x_{2}$ be the extreme point in $\M_{2}$ in the direction $u_{0}$. By assumption, $V_{L}(x_{1}) > V_{L}(x_{2})$.

% Now, consider the set of $\bar{u}_{O}$ under which $x_{1}$ is a best response in $\M_{1}$, and the set of $\hat{u}_{O}$ under which $x_{2}$ is a best response in $\M_{2}$. If there is a constant measure set of overlap, we are done (everything here has the property we want). If not, then these sets only intersect at a single point. As both menus are polytopes, the sets themselves must be of constant measure set. But since they only overlap in a single place, $u_{O}$ is a tiebreak point for both menus. But for this to be the case, both menus have to have parallel faces. And in this case, there's no angle that distinguishes between 

% \end{proof}









% \begin{lemma}\label{lem:menu-min-value}
% If $\M$ is a no-regret asymptotic menu, then $\Um(\M) = \Uzs$.
% \end{lemma}
% \begin{proof}
% \nat{Theorem \ref{thm:nr_nsr_containment} shows one direction; Lemma~\ref{lem:menu-min-UB} shows the other}
% \end{proof}


% Unlike $\M^{+}$ which is always equal to $\{\csp^{+}\}$ for Pareto-optimal menus, the minimizing set $\M^{-}$ is not uniquely defined and may contain many CSPs. However, there is a ``minimal'' minimizing set $\M^{-}$ for no-regret menus: for any such menu $\M^{-}$ must contain $\M_{NSR}^{-}$. In fact, this is true for the slightly larger class of menus with $\Um(\M) = \Uzs$. 

% \begin{lemma}\label{lem:menu-min-set}
% Let $\M$ be an asymptotic menu with $\Um(\M) = \Uzs$. Then $\M_{NSR}^{-} \subseteq \M^{-}$.
% \end{lemma}
% \begin{proof}


% By Lemma~\ref{lem:nsr_characterization}, all extreme points of $\M_{NSR}^{-}$ must be of the form $x \otimes y$, with $x \in \Delta_{m}$ and $y \in \BR_{L}(x)$. Furthermore, by definition, for all points in $\M^{-}$, $u_{L}(x \otimes y) = \Uzs$. By Lemma~\ref{lem:minimal_min}, $\M^{-}$ must also contain all these points. Therefore, $\M_{NSR}^{-} \subseteq \M^{-}$.



% \end{proof}



% %\begin{lemma}
% %If $\M$ is an asymptotic menu of a no-regret learning algorithm, then $\cM \subseteq \cM_{NR}$. If $\M$ is an asymptotic menu of a no-swap-regret learning algorithm, then $\cM \subseteq \cM_{NSR}$.
% %\end{lemma}












% A careful reading of the first part of the proof of Lemma~\ref{lem:nsr_characterization} highlights that we only the no-regret property in showing that all CSPs of the form $x \otimes y$, with $x \in \Delta_{m}$ and $y \in \BR_{L}(x)$ are contained in $\M_{NSR}$, thus; all such points are contained in $\M_{NR}$. We show below that a more fine grained result is true, where $\M_{NR}$ is replaced by the menu of any no-regret algorithm.




\subsection{Completing the proof}
\label{sec:completing-the-proof}

We can now finish the proof of Theorem~\ref{thm:pareto-optimal-characterization}.
\begin{proof}[Proof of Theorem~\ref{thm:pareto-optimal-characterization}]
We will first prove that if a no-regret menu $\M$ satisfies $\M^{-} = \M_{NSR}^{-}$, then it is Pareto-optimal. To do so, we will consider any other menu $\M'$ and show that $\M'$ does not Pareto-dominate $\M$. There are three cases to consider:

% To see this, note that if $U^{-}(\M') < U^{-}(\M)$, then $\M'$ cannot dominate $\M$ since $V_{L}(\M, -u_L) > V_{L}(\M', -u_L)$ (that is, if the optimizer's utility is aligned completely against the learner's utility, the learner does worse under $\M'$). But also, by Lemma \ref{lem:menu-min-value}, we cannot have $U^{-}(\M') > U^{-}(\M) = U_{ZS}$. So we must have $U^{-}(\M') = U^{-}(\M)$.

% By Lemma \ref{lem}
% First, we will prove that every no-regret menu $\M$ that has the same set of minimum value points as $P_{NSR}$ is pareto-optimal. To do so, we will consider any other menu $\bar{\M}$ and show that $\bar{\M}$ does not pareto-dominate $\M$, considering three cases:

\begin{itemize}
\item \textbf{Case 1}: $U^{-}(\M') < U^{-}(\M)$. In this case, $\M'$ cannot dominate $\M$ since $V_{L}(\M, -u_L) > V_{L}(\M', -u_L)$ (note that $U^{-}(\M) = V_{L}(\M, -u_L)$, since if $u_O = -u_L$, the optimizer picks the utility-minimizing point for the learner).

\item \textbf{Case 2}: $U^{-}(\M') > U^{-}(\M)$. By Lemma \ref{lem:menu-min-value}, this is not possible.

\item \textbf{Case 3}: $U^{-}(\M') = U^{-}(\M)$. Then, by Lemma~\ref{lem:menu-min-set}, $\M^{-} \subseteq (\M')^{-}$. Also, by Lemma \ref{lem:has_max_point}, we can assume without loss of generality that $(\M')^{+} = \{\csp^{+}\} = \M^{+}$ (if $\M'$ does not contain $\csp^{+}$, replace it with the Pareto-dominating menu that contains it). Now, by Lemma~\ref{lem:non-dominance}, $\M'$ does not dominate $\M$.
\end{itemize}

We now must show that if $\M^{-} \neq \M_{NSR}^{-}$, then it is Pareto-dominated by some other menu. Since $\M$ is (by assumption) a no-regret menu, we must have $U^{-}(\M) = U^{-}(\M_{NSR}) = U_{ZS}$, and $\M^{-} \supset \M^{-}_{NSR}$ (Lemmas \ref{lem:menu-min-value} and \ref{lem:menu-min-set}). Consider an extreme point $\csp_0$ that belongs to $\M^{-}$ but not to $\M_{NSR}^{-}$. Construct the menu $\M'$ as follows: it is the convex hull of $\M_{NSR}$ and all the extreme points in $\M$ \emph{except for} $\csp_0$. By Lemma \ref{lem:char_upwards_closed}, this is a valid menu (it is formed by adding some points to the valid menu $\M_{NSR}$). Note also that $\M'$ has all the same extreme points of $\M$ except for $\csp_0$ (since $\M$ is a polytope, we add a finite number of extreme points to $\M'$, all of which are well-separated from $\csp_0$), and in particular is distinct from $\M$.

We will show that $\M'$ Pareto-dominates $\M$. To see this, note first that, by Lemma~\ref{lem:non-dominance}, there is some $u_{O}$ such that $V_{L}(U_{\M},u_{O}) < V_{L}(U_{\M'},u_{O})$. Furthermore, for all other values of $u_{O}$, $V_{L}(U_{\M},u_{O}) \leq V_{L}(U_{\M'},u_{O})$. This is since the maximizer of $u_O$ over $\M$ is either the minimal-utility point $\csp_0$ (which cannot be strictly better than the maximizer of $u_O$ over $\M'$), or exactly the same point as the maximizer of $u_O$ over $\M'$. It follows that $\M'$ Pareto-dominates $\M$.
\end{proof}

Note that in the Proof of Theorem \ref{thm:pareto-optimal-characterization}, we only rely on the fact that the menu $\cM$ is polytopal in precisely one spot, when we construct a menu $\M'$ that Pareto-dominates $\M$ by ``removing'' an extreme point from $\M^{-}$. As stated, this removal operation requires $\M$ to be a polytope: in general, it is possible that any extreme point $\csp_0$ that belongs to $\M^{-}$ is a limit of other extreme points in $\M$, and so when attempting to construct $\M'$ per the procedure above, we would just perfectly recover the original $\M$ when taking the convex closure of the remaining points. 

That said, it is not clear whether the characterization of non-polytopal Pareto-optimal menus is any different than the characterization in Theorem \ref{thm:pareto-optimal-characterization}. In fact, by the argument in the proof of Theorem \ref{thm:pareto-optimal-characterization}, one direction of the characterization still holds (if a non-polytopal no-regret menu satisfies $\M^{-} = \M^{-}_{NSR}$, then it is Pareto-optimal). We conjecture that this characterization holds for non-polytopal menus (and leave it as an interesting open problem). 

\begin{conjecture}
Any no-regret menu $\M$ is Pareto-optimal iff $\M^{-} = \M_{NSR}$.
\end{conjecture}

On the other hand, the restriction to no-regret menus is necessary for the characterization of Theorem \ref{thm:pareto-optimal-characterization} to hold. In Section \ref{sec:other-pareto-optimal} we provide an example of a (high-regret) Pareto-optimal menu which does not satisfy $\M^{-} = \M^{-}_{NSR}$. We also leave it as an interesting open question to provide a full characterization of all Pareto-optimal asymptotic menus.

\subsection{Implications for no-regret and no-swap-regret menus}
\label{sec:regret-implications}

Already Theorem \ref{thm:pareto-optimal-characterization} has a number of immediate consequences for understanding the no-regret menu $\M_{NR}$ and the no-swap-regret menu $\M_{NSR}$, both of which are polytopal no-regret menus by their definitions in \eqref{eq:no-regret-constraint} and \eqref{eq:no-swap-regret-constraint} respectively. As an immediate consequence of our characterization, we can see that the no-swap-regret menu (and hence any no-swap-regret learning algorithm) is Pareto-optimal.

\begin{corollary}
The no-swap-regret menu $\M_{NSR}$ is a Pareto-optimal asymptotic menu.
\end{corollary}

It would perhaps be ideal if $\M_{NSR}$ was the unique Pareto-optimal no-regret menu, as it would provide a somewhat clear answer as to which learning algorithm one should use in a repeated game. Unfortunately, this is not the case -- although $\M_{NSR}$ is the minimal Pareto-optimal no-regret menu, Theorem \ref{thm:pareto-optimal-characterization} implies there exist infinitely many distinct Pareto-optimal menus. %\nat{minimal amongst all no regret menus at least}

On the more positive side, Theorem \ref{thm:pareto-optimal-characterization} (combined with Lemma \ref{lem:char_upwards_closed}) gives a recipe for how to construct a generic Pareto-optimal learning algorithm: start with a no-swap-regret learning algorithm (the menu $\M_{NSR}$) and augment it with any set of additional CSPs that the learner and optimizer can agree to reach. This can be any set of CSPs as long as i. each CSP $\csp$ has no regret, and ii. each CSP has learner utility $u_L(\csp)$ strictly larger than the minimax value $U_{ZS}$. 

\begin{corollary}
There exist infinitely many Pareto-optimal asymptotic menus.
\end{corollary}

Finally, perhaps the most interesting consequence of Theorem \ref{thm:pareto-optimal-characterization} is that, despite this apparent wealth of Pareto-optimal menus and learning algorithms, the no-regret menu $\M_{NR}$ is very often \emph{Pareto-dominated}. In particular, there are large sets of learner payoffs $u_L$ for which $\M^{-}_{NR} \neq \M^{-}_{NSR}$, as we show below.

\begin{corollary}
There is a positive measure set of learner payoffs $u_L$ for which the no-regret $\M_{NR}$ is \emph{not} a Pareto-optimal asymptotic menu.
\end{corollary}
\begin{proof}

\end{proof}
% Theorem~\ref{theorem:all_about_nsr} follows directly from Theorem~\ref{thm:pareto_optimal_nr_char}. 



==> polytopes_limits.tex <==
The below results form an outline for the tools we need to generalize our results about polytope menus to the limit menus.

\esh{This section is, as things stand, redundant. It might be worth mentioning Lemma~\ref{lemma:finite_time_horizon_polytope} though.}

\begin{lemma}
\label{lemma:finite_time_horizon_polytope}
    For a finite time horizon, the menu of every algorithm $\A$ on every learner payoff is a polytope. \esh{Add Caveat : the optimizer actions have finite information}
\end{lemma}


\begin{proof}
    Intuition : Induction on the $\#$ of time steps

    We show that this statement is true for the base case of $T=1$. For $T=1$, any algorithm $A$ is characterized entirely by the play $x_1 \in \Delta^m$ that it makes in the first round. Similarly, the behaviour of the optimizer is entirely determined by $y_1 \in \Delta^n$ chosen for the first round. Thus, the menu $\M(A)$ is exactly the set $\{x_1 \otimes y_1: y_1 \in \Delta^n\} \subseteq \Delta^{mn}$. This menu is a polytope because it can be written as the convex hull of the finite set $\{x_1 \otimes \mathbbm{1}_j \}_{j\in [n]}$. For a proof by induction, we assume the hypothesis that for all algorithms $A$ for threshold $T$, the menu $\M(A)$ is a polytope. Now, consider some algorithm $A$ for threshold $T+1$. This algorithm always picks $x_1 \in \Delta^m$ in the first round regardless of the optimizer's behavior since it has no history to observe yet. Let us consider any optimizer sequence $y_1, y_2 \cdots y_{T+1}$. Depending on $y_1$, the algorithm $A$ changes its state after the first round onward and we can think of it as using some algorithm $(B_{y_1})$ for rounds $2$ to $T$ where $A_t(y_1, y_2 \cdots y_{t-1}) = (B_{y_1})_{t-1}(y_2, y_3, y_4 \cdots y_{t-1}) $.

    Let $P(y_1, y_2 ,\cdots y_{T+1}) := \frac{1}{T }\sum_{t=1}^T x_t \otimes y_t$ where $x_t  = A_t(y_1,y_2,\cdots y_{t-1}) $. The menu $\M(A)$ is the convex hull of the set $X: = \{ P(y_1, y_2 ,\cdots y_{T+1})\}_{y_1, y_2 ,\cdots y_{T+1}}$. Let $Z(y_1): = \{ Q(y_1,y_2, y_3 ,\cdots y_{T+1})\}_{y_2, y_3 ,\cdots y_{T+1}}$ where $Q(y_1, y_2, y_3 ,\cdots y_{T+1}) :=   \frac{1}{T+1}\sum_{t=2}^{T+1} x_t \otimes y_t$ where $x_t  = (B_{y_1})_t(y_2,\cdots y_{t-1}) $ and let $Z' = \{z + \frac{1}{T+1} x_1 \otimes y_1\}_{y_1 \in \Delta^n, z \in Z(y_1)}$. Using the induction hypothesis, Conv($Z'$) is a polytope because the induction hypothesis shows that each $Z(y_1)$ is a polytope since it is just the menu induced by a $T-1$ threshold algorithm $(B_{y_1})$ 
    \esh{This proof is running into issues at this point due to the infinite choices for $y_1$ -- one possible fix is to discretize the set of distributions avaliable to a threshold $T$- algorithm and the corresponding optimizer using some granularity bounded by a function of $T$ -- this has its issues}
    \esh{This is sort of linked to the observation that we had that an action of the learner/ optimizer is infinitely informative}
\end{proof}


%\esh{Is it WLOG to assume that consecutive polytopes in this sequence become increasingly closer under the Haussdorff distance? ( equivalence between different notions of convergence under the Haussdorff metric) This seems like a reasonable assumption under the notion of time-consistency of algorithms in case it buys us something extra.}
\begin{lemma}
    Let $P_1, P_2 \cdots $ be a sequence of polytopes in $\mathbb{R}^d$ that converges under the Hausdorff metric to some limit set $P$. Let $u_L \in \mathbb{R}^d$ be a direction for linear maximization and let $v_1, v_2 \cdots $ be the sequence of obejctive values for $u_L$ in this sequence of polytopes. Then this latter sequence converges to a value $v$. Additionally, $ v = \max_{x\in P} u_L(x)$.
\end{lemma}


Why do we care about the limit object?

Isn't it as good to make the same statements with sublinear approximation about all time steps beyond a threshold?

\nat{In order to add a point to a menu, you do need to make sublinear changes to the extreme points of the original menu. This means nothing in the limit, but in the actual game, it could completely change what extreme point should be selected. Thinking about limit objects solves this problem, but doesn't the fact that the limit object behavior is so different than the actual finite time game suggest that the limit object isn't that meaningful? }

